Deciding Asynchronous Hyperproperties for Recursive Programs

We introduce a novel logic for asynchronous hyperproperties with a new mechanism to identify relevant positions on traces. While the new logic is more expressive than a related logic presented recently by Bozzelli et al., we obtain the same complexity of the model checking problem for finite state models. Beyond this, we study the model checking problem of our logic for pushdown models. We argue that the combination of asynchronicity and a non-regular model class studied in this paper constitutes the first suitable approach for hyperproperty model checking against recursive programs.

==> math/constructions/formulatranslation.tex <==
For the translation of $\varphi := Q_n \pi_n \dots Q_1 \pi_1 . \psi$, we obtain $\varphi'$ by  transforming $\psi$ into a formula $\psi'$, where every test $[\delta]_\pi$ is replaced by $[\at(\delta)]_\pi$ and successor assignments $\Delta$ 
%with $\Delta(\pi_i) = \delta_i$ 
are replaced by $\Delta'$ where $\Delta'(\pi) = \at(\Delta(\pi))$. % if $\Delta(\pi) = \delta$.
%The translation $\varphi'$ is then given as $Q_n \pi_n \dots Q_1 \pi_1 . \psi'$.

==> math/constructions/vpformulatranslation.tex <==
\tbd{Formula translation}

==> math/constructions/vpmodelcheckinglemma.tex <==
We extend the construction from \autoref{subsec:singleassignmentmodelchecking} to also handle abstract and caller successors.
The main difference is that instead of constructing an APA with the desired properties, we construct a 2-AJA.
However, since any APA can also be considered a 2-AJA that only uses global successors, the construction from \autoref{subsec:singleassignmentmodelchecking} can be kept as is.
Thus, we only have to add cases for $\bigcirc^{a} \delta$ and $\bigcirc^{-} \delta$ foramulae to the construction of the transition function and obtain a lemma similar to \autoref{cor:modelcheckinglemma} for $\delta$ formulae with all kinds of next operators.
The constructions are given as follows:
\begin{align*}
	\rho_{\delta}(q_{\bigcirc^a \theta}, A \cup N) &= (a,q_{\theta},\false)\\
	\rho_{\delta}(q_{\bigcirc^- \theta}, A \cup N) &= (c,q_{\theta},\false).
\end{align*}
The priority assignment is done as previously.

==> math/constructions/vpproductstructure.tex <==
\tbd{Structure translation}

==> math/defs/semantics.tex <==
\begin{definition}[Quantifier semantics of stuttering $H_\mu$]
	For quantified stuttering $H_\mu$ formulae $\varphi$, the semantics is defined in the following way:
	\begin{align*}
		\Pi &\models_\mathcal{K} \exists \pi . \varphi &&\qquad \text{ iff } \Pi[\pi \mapsto p] \models_\mathcal{K} \varphi \text{ for some } p \in Paths(\mathcal{K}) \\
		\Pi &\models_\mathcal{K} \forall \pi . \varphi &&\qquad \text{ iff } \Pi[\pi \mapsto p] \models_\mathcal{K} \varphi \text{ for all } p \in Paths(\mathcal{K}) \\
		\Pi &\models_\mathcal{K} \psi &&\qquad \text{ iff } (0,...,0) \in \llbracket \psi \rrbracket_{\mathcal{W}_0}^\Pi
	\end{align*}
\end{definition}
\begin{definition}[Path assignment semantics of stuttering $H_\mu$]
	For multi-path stuttering $H_\mu$ formulae $\psi$, the semantics is defined in the following way:
	\begin{align*}
		\llbracket [\delta]_{\pi_i} \rrbracket_{\mathcal{W}}^\Pi &:= \{(v_1,...,v_n) \in \mathbb{N}_0^n \mid v_i \in \llbracket \delta \rrbracket_{\mathcal{V}_0}^{\Pi(\pi_i)} \}  \\
		\llbracket X \rrbracket_{\mathcal{W}}^\Pi &:= \mathcal{W}(X)  \\
		\llbracket \psi_1 \lor \psi_2 \rrbracket_{\mathcal{W}}^\Pi &:= \llbracket \psi_1 \rrbracket_{\mathcal{W}}^\Pi \cup \llbracket \psi_1 \rrbracket_{\mathcal{W}}^\Pi \\
		\llbracket \lnot \psi \rrbracket_{\mathcal{W}}^\Pi &:= \mathbb{N}_0 \setminus \llbracket \psi \rrbracket_{\mathcal{W}}^\Pi  \\
		\llbracket \bigcirc^\Delta \psi \rrbracket_{\mathcal{W}}^\Pi &:= \{ v \in \mathbb{N}_0^n \mid succ_\Delta(\Pi,v) \in \llbracket \psi \rrbracket_{\mathcal{W}}^{\Pi} \}  \\
		\llbracket \mu X . \psi \rrbracket_{\mathcal{W}}^\Pi &:= \bigsqcap\{ V \subseteq \mathbb{N}_0^n \mid \llbracket \psi \rrbracket_{\mathcal{W}[X \mapsto V]}^\Pi \subseteq V\} 
	\end{align*}
\end{definition}
\begin{definition}[Path semantics of stuttering $H_\mu$]
	For path stuttering $H_\mu$ formulae $\delta$, the semantics is defined in the following way:
	\begin{align*}
		\llbracket a \rrbracket_\mathcal{V}^p  &:= \{ i \in \mathbb{N} \mid a \in L(p[i])\} \\
		\llbracket X \rrbracket_\mathcal{V}^p  &:= \mathcal{V}(X) \\
		\llbracket \delta_1 \lor \delta_2 \rrbracket_\mathcal{V}^p  &:= \llbracket \delta_1 \rrbracket_{\mathcal{V}}^p \cup \llbracket \delta_2 \rrbracket_{\mathcal{V}}^p \\
		\llbracket \lnot \delta \rrbracket_\mathcal{V}^p  &:= \mathbb{N}_0 \setminus \llbracket \delta \rrbracket_{\mathcal{V}}^p \\
		\llbracket \bigcirc^f \delta \rrbracket_\mathcal{V}^p  &:= \{ i \in \mathbb{N} \mid succ_f(p,i) \in \llbracket \delta \rrbracket_{\mathcal{V}}^p\} \\
		\llbracket \mu X . \delta \rrbracket_\mathcal{V}^p  &:= \bigsqcap\{ I \subseteq \mathbb{N}_0 \mid \llbracket \delta \rrbracket_{\mathcal{V}[X \mapsto I]}^p \subseteq I\} 
	\end{align*}
\end{definition}

==> math/defs/stutteringkequivalence.tex <==
\begin{definition}
	Given a Kripke Structure $\mathcal{K} = (S,s_0,R,L)$, a formula $\psi$ over $\{\pi_1,\dots,\pi_n\}$ with successor assignment $\Delta$ and Alternating Parity Automaton $\mathcal{A}$, we call $\mathcal{A}$ $\mathcal{K}$-equivalent to $\psi$ with respect to $\Delta$, iff the following condition holds:
	for all path assignments $\Pi$ and offsets $i$, we have $(i,\dots,i) \in \llbracket \psi^{s} \rrbracket^{\Pi^\Delta}$ iff $w_{\Pi^{\Delta}}[(i,\dots,i)] \in \mathcal{L}(\mathcal{A})$.
\end{definition}

==> math/proofs/alignmentlemma.tex <==
\begin{proof}(of \cref{lem:alignmentlemma})
	We choose $k$ as the difference between the starting stack level and the lowest stack level encountered during the subtraces.
	$l$ is chosen as the difference between the final stack level and the lowest stack level.
	It is easy to see the subtraces can be divided into three subsections according to $(\abs^* \ret)^k$, $(\abs^* \call)^l$ and $\abs^*$.
	The first subsection ends when the lowest stack level is encountered for the first time and the second subsection ends when the finial stack level is entered for the first time with the additional condition that the stack level never drops below this level after that.
\end{proof}

==> math/proofs/deltastrictexpressiveness.tex <==
\begin{proof}(of \cref{thm:deltastrictexpressiveness})
	Follows immediately from \cref{lem:deltastrictexpressivenesslemma1} and \cref{lem:deltastrictexpressivenesslemma2}.
\end{proof}

\begin{comment}
	\begin{proof}(of \cref{thm:deltastrictexpressiveness})
		The hyperproperty $\mathcal{H}$ is given by the set of all $\mathcal{T} \subseteq (2^\AP)^\omega$ such that for all $tr \in \mathcal{T}$ we have $p \in tr(0)$ and all $tr \in \mathcal{T}$ have the same finite number of positions $i$ with  $p \in tr(i)$.
		In $\Delta$-stuttering $H_\mu$, this can be expressed as $\forall \pi_1 . \forall \pi_2 . [p]_{\pi_1} \land [p]_{\pi_2} \land (([p]_{\pi_1} \land [p]_{\pi_2}) \mathcal{U}^{\Delta} (\lnot[p]_{\pi_1} \land \lnot[p]_{\pi_2}))$ where $\Delta(\pi_1) = \Delta(\pi_2) = p$.
		
		In order to show that $\Gamma$-stuttering $H_\mu$ with basis $LTL$ cannot express this property, we first inductively define $nd(\delta)$ as the nesting depth of $\bigcirc$ modalities in $\delta$:
		$nd(a) = 0$, $nd(\lnot \delta) = nd(\delta)$, $nd(\delta \lor \delta') = nd(\delta \mathcal{U} \delta') = \max \{nd(\delta),nd(\delta')\}$ and $nd(\bigcirc \delta) = nd(\delta) + 1$.
		Furthermore, for $n \geq 1$ let $tr_n$ be the trace $\{p\}^n\emptyset^\omega$.
		Next, we show:
		
		\textbf{Claim $1$:} for all formulae $\delta \in LTL$ with $nd(\delta) = n$, we have $tr_i \models \delta$ iff $tr_j \models \delta$ for all $i,j > n$.
		
		In this claim, we write $tr \models \delta$ for $0 \in \llbracket \delta \rrbracket^{tr}$ in order to improve readability in the proof.
		The proof is by structural induction:
		\begin{description}
			\item[Case $\delta = a$:] Straightforward due to $tr_i(0) = tr_j(0) = \{p\}$.
			
			\item[Case $\delta = \lnot \delta'$:] Directly from the induction hypothesis.
			
			\item[Case $\delta = \delta' \lor \delta''$:] Directly from the induction hypothesis.
			
			\item[Case $\delta = \bigcirc \delta'$:] From the definition of $nd$, we have $i-1,j-1 > nd(\delta')$ for $i,j > nd(\delta)$.
			Hence, we have $tr_i \models \delta$ iff $tr_{i-1} \models \delta'$ iff $tr_{j-1} \models \delta'$ iff $tr_j \models \delta$ where the first and last equivalence are due to the semantics of $\delta$ and the second equivalence follows from the induction hypothesis.
			
			\item[Case $\delta = \delta' \mathcal{U} \delta''$:] From the definition of $nd$, we have $i,j > nd(\delta')$ and $i,j > nd(\delta'')$ for all $i,j > nd(\delta)$.
			Assume w.l.o.g. that $i \leq j$.
			We show both directions of the equivalence separately.
			Assume first that $tr_j \models \delta$.
			If $tr_j \models \delta''$, then $tr_i \models \delta''$ by the induction hypothesis and we have $tr_i \models \delta$.
			If $tr_j \not\models \delta''$, then by the induction hypothesis ($\ast$) $tr_l \not\models \delta''$ for all $j \geq l \geq i$.
			As $tr_j \models \delta$, there is a $k$ such that $tr_k \models \delta''$ and for all $l$ with $j \geq l > k$ we have $tr_l \models \delta'$ and $tr_l \not\models \delta''$.
			By ($\ast$) we have $i > k$.
			By the semantics of $\mathcal{U}$, we get $tr_i \models \delta$.
			The other direction is similar.
			%We discriminate cases based on what formulae $tr_j$ satisfies.
			%If $tr_j \models \delta''$, then $tr_i \models \delta''$ by the induction hypothesis and we have $tr_j \models \delta$ and $tr_i \models \delta$.
			%If $tr_j \not\models \delta''$, then by the induction hypothesis ($\ast$) $tr_l \not\models \delta''$ for all $j \geq l \geq i$.
			%If additionally, $tr_j \models \delta$, then there is a $k$ such that $tr_k \models \delta''$ and for all $j \geq l > k$ we have $tr_j \models \delta'$ and $tr_l \not\models \delta''$.
			%By ($\ast$) we have $i > k$.
			%By the semantics of $\mathcal{U}$, we get $tr_i \models \delta$.
		\end{description}
		
		Next, we use Claim $1$ to show:
		
		\begin{sloppypar}
			\textbf{Claim $2$:} for all trace assignments $\Pi$, we have $(0,\dots,0) \in \llbracket \psi \rrbracket^{\Pi[\pi \mapsto tr_i]}$ iff $(0,\dots,0) \in \llbracket \psi \rrbracket^{\Pi[\pi \mapsto tr_j]}$ for all $i,j >\max\{nd(\delta) \mid \delta \in \sub(\psi)\}$.
		\end{sloppypar}
		
		By unrolling every fixpoint once, we can bring every closed formula $\psi$ into a form $\rho$ described by the following grammar:
		\begin{align*}
			\rho := \quad [\delta]_\pi  \mid \rho \lor \rho \mid \lnot \rho \mid \bigcirc^{\Delta} \psi
		\end{align*}
		The proof is by structural induction on $\rho$.
		\begin{description}
			\item[Case $\rho = [\delta{]}_\pi$:] Immediate by Claim $1$
			\item[Case $\rho = \lnot\rho'$:] Directly from the induction hypothesis
			\item[Case $\rho = \rho' \lor \rho''$:] Directly from the induction hypothesis
			\item[Case $\rho = \bigcirc^\Gamma \psi$:] The formula $\psi$ is evaluated on index vectors, namely the $\Gamma$-successors of $(0,\dots,0)$ in $\Pi[\pi \mapsto tr_i]$ and $\Pi[\pi \mapsto tr_j]$.
			By Claim $1$, it follows that on $tr_i$ and $tr_j$, the suffixes starting from the $\Gamma$-successors of $(0,\dots,0)$ are the same.
			For all other traces in $\Pi[\pi \mapsto tr_i]$ and $\Pi[\pi \mapsto tr_j]$, the suffixes are the same for trivial reasons.
			Since the evaluation of $\psi$ only depends on these suffixes, the results are the same.
		\end{description}
		Assume now that $\varphi = Q_1 \pi_1  \dots Q_m \pi_m . \psi$ is a formula that expresses the above hyperproperty $\mathcal{H}$.
		Let $n = \max\{nd(\delta) \mid \delta \in \sub(\psi)\}$.
		Then, let $\mathcal{T}_1 = \{t_{n+1}\}$ and $\mathcal{T}_2 = \{t_{n+1},t_{n+2}\}$.
		Obviously $\mathcal{T}_1 \in \mathcal{H}$ whereas $\mathcal{T}_2 \not\in \mathcal{H}$.
		Consequently $\mathcal{T}_1 \models \varphi$ and $\mathcal{T}_2 \not\models \varphi$.
		However, using Claim 2, it is easy to see that $\mathcal{T}_1 \models \varphi$ implies $\mathcal{T}_2 \models \varphi$, a contradiction.
	\end{proof}
\end{comment}

==> math/proofs/deltastrictexpressivenessfix.tex <==
\subsection*{Fix to proof of \cref{thm:deltastrictexpressiveness}}

Let $\mathcal{H} = \{\mathcal{T} \subseteq (2^\AP)^\omega \mid \exists n \in \mathbb{N}.\forall tr \in \mathcal{T}. p \in tr(i) \text{ for exactly } n \text{ positions } i \}$.
We write $tr \models \delta$ for $0 \in \llbracket \delta \rrbracket^{tr}$ for single trace formulae $\delta$ in order to improve readability.

\input{math/theorems/ltlclaim}
\input{math/proofs/ltlclaim}

\input{math/theorems/deltastrictexpressivenesslemma1}
\input{math/proofs/deltastrictexpressivenesslemma1}

\input{math/theorems/deltastrictexpressivenesslemma2}
\input{math/proofs/deltastrictexpressivenesslemma2}


\begin{comment}
	Let $\mathcal{H} = \{\mathcal{T} \subseteq (2^\AP)^\omega \mid \exists n \in \mathbb{N}.\forall tr \in \mathcal{T}. p \in tr(0), p \in tr(i) \text{ for exactly } n \text{ positions } i \}$.
	%We say that $\varphi$ expresses $\mathcal{H}$ when for all sets of traces $\mathcal{T} \subseteq (2^\AP)^\omega$ and trace assignments $\Pi$ over $\mathcal{T}$, $\Pi \models_{\mathcal{T}} \varphi$ iff $\mathcal{T} \in \mathcal{H}$.
	We say that $\varphi$ expresses $\mathcal{H}$ when for all sets of traces $\mathcal{T} \subseteq (2^\AP)^\omega$ the following two statements are equivalent:
	\begin{itemize}
		\item For all trace assignments $\Pi$ over $\mathcal{T}$ binding the variables in $\varphi$, we have  $\Pi \models_{\mathcal{T}} \varphi$
		\item $\mathcal{T} \in \mathcal{H}$
	\end{itemize}
	
	
	\begin{lemma}\label{lem:deltrastrictexpressivenessfix1}
		In the decidable fragment, there is no quantifier-free $\Gamma$-stuttuering $H_\mu$ formula $\psi$ over variables $\pi_1,\dots,\pi_n$ such that the following statements are equivalent: (i) for all trace assignments $\Pi$, $(0,\dots,0) \in \llbracket \psi \rrbracket^\Pi$ and (ii) $\{\Pi(\pi_1),\dots,\Pi(\pi_n)\} \in \mathcal{H}$.
		% is a path assignment over some $\mathcal{T} \in \mathcal{H}$.
	\end{lemma}
	\begin{proof}
		We show the claim for formulae over two variables $\pi_1,\pi_2$, the proof for formulae with more free variables works the same.
		
		Assume towards contradiction that there is a formula $\psi$ with the desired semantics.
		Let $\Gamma$ be the unique stuttering-assignment in $\psi$.
		Let $\mathcal{A}_{\psi^s}$ be the automaton given by \cref{thm:synchronousautomaton} for $\psi^s$, i.e. the synchronous variant of $\psi$. 
		Furthermore, let $l = nd(\psi) + 1$ and let $m = 2 \cdot l + |\mathcal{A}_{\psi^s}| + 1$.
		Consider $tr_1 := \{p\}^{l+1} \emptyset^m \{p\}^{m-l} \emptyset^\omega$ and $tr_2 := \{p\} \emptyset^l \{p\}^m \emptyset^\omega$.
		It is easy to see that $\{tr_1,tr_2\} \in \mathcal{H}$ and thus we have $(0,0) \in \llbracket \psi \rrbracket^\Pi$ for a trace assignment $\Pi$ with $\Pi(\pi_1) = tr_1$ and $\Pi(\pi_2) = tr_2$.
		
		We say that a stuttering criterion $\gamma \in 2^\delta$ makes a type one step on $tr$ at position $i$ if $\Succ_\gamma(tr,i)$ is given by the first case in the definition of $\Succ_\gamma$.
		Similarly, we say that $\gamma$ makes a type two step on $tr$ at position $i$ if $\Succ_\gamma(tr,i)$ is given by the second case.
		We distinguish three cases based on where the criteria in $\Gamma$ make type one and type two steps on $tr_1$ and $tr_2$ respectively.
		
		In the first case, $\Gamma(\pi_1)$ makes a type one step on $tr_1$ at position $0$.
		Let $tr_1' := \{p\} tr_1$, i.e. a variant of $tr_1$ with an additional $p$-position at the front.
		By Claim 1, we know that $tr_1'(0)$ and $tr_1'(1)$ have the same valuations for all formulae in $\Gamma(\pi_1)$.
		Thus, $\strf_{\Gamma(\pi_1)}(tr_1) = \strf_{\Gamma(\pi_1)}(tr_1')$.
		Let $\Pi' := \Pi[\pi_1 \mapsto tr_1']$ be a variant of $\Pi$ where $tr_1$ is replaced with $tr_1'$.
		Since $tr_1'$ and $tr_2$ do not have the same number of $p$-positions, $\Pi'$ does not fulfill the desired property.
		Using \cref{lem:synchronousconnection} and the fact that $\Pi^\Gamma = \Pi'^\Gamma$, we obtain that $(0,0) \in \llbracket \psi \rrbracket^{\Pi'}$, a contradiction.
		
		In the second case, $\Gamma(\pi_1)$ makes a type two step on $tr_1$ at position $0$ and $\Gamma(\pi_2)$ makes a type one step on $tr_2$ at position $l+2$.
		This case works similar to the first one, but a $p$-position is added to the $\{p\}^m$ subword of $tr_2$ this time.
		
		In the third case, $\Gamma(\pi_1)$ makes a type two step on $tr_1$ at position $0$ and $\Gamma(\pi_2)$ makes a type two step on $tr_2$ at position $l+2$.
		In particular, this means that $\strf_1 := \strf_{\Gamma(\pi_1)}(tr_1)$ conicides with $tr_1$ and $\strf_2 := \strf_{\Gamma(\pi_2)}(tr_2)$ coincides with a version of $tr_2$ that has less positions in its $\emptyset^l$ subword and is otherwise the same.
		By \cref{lem:synchronousconnection} we know that $(0,0) \in \llbracket \psi^s \rrbracket^{\Pi^\Gamma}$ from which we obtain $w_{\Pi^\Gamma} \in \mathcal{L}(\mathcal{A}_{\psi^s})$.
		We inspect the run of $\mathcal{A}_{\psi^s}$ on $w_{\Pi^\Gamma}$ more closely.
		Due to our observation of the form of $\strf_1$ and $\strf_2$, we know that after $l+2$ steps, $\mathcal{A}_{\psi^s}$ is at a position where it reads at least $m+1$ $(\emptyset,\{p\})$ symbols, i.e. $\emptyset$ on $\strf_1$ and $\{p\}$ on $\strf_2$.
		This means that some state $q$ of $\mathcal{A}_{\psi^s}$ is visited twice while reading these symbols.
		The subrun between the two visits of $q$ can be repeated by adding an appropriate number of $(\emptyset,\{p\})$ symbols to $w_{\Pi^\Gamma}$ without changing the acceptance of $\mathcal{A}_{\psi^s}$.
		We thus obtain $w' \in \mathcal{L}(\mathcal{A}_{\psi^s})$ for a variant $w'$ of $w_{\Pi^\Gamma}$ where $\strf_1$ is replaced with some $tr_1'$ and $\strf_2$ is replaced with some $tr_2'$.
		In particular, $tr_1'$ and $tr_2'$ do not have the same number of $p$-positions.
		After the second visit to $q$ there are still at least $l$ $(\emptyset,\{p\})$ symbols left.
		By a slight variation of Claim 1, we thus know that the additional positions in $tr_1'$ and $tr_2'$ have the same valuations as the positions directly behind them for all formulae from $\Gamma(\pi_1)$ and $\Gamma(\pi_2)$ respectively.
		Therefore $\strf_{\Gamma(\pi_1)}(tr_1') = tr_1'$ and $\strf_{\Gamma(\pi_2)}(tr_2') = tr_2'$ and $\Pi' = \Pi'^\Gamma$ for $\Pi'$ with $\Pi'(\pi_1) = tr_1'$ and $\Pi'(\pi_2) = tr_2'$.
		With an additional use of \cref{lem:synchronousconnection}, we conclude that $(0,0) \in \llbracket \psi \rrbracket^{\Pi'}$, a contradicition.
	\end{proof}
	
	\tbd{The Lemma can also be extended to quantified formulae over at least two free variables.
		$|\mathcal{A}_{\varphi}|$ can now only exist for regular sets of traces.
		It also depends on the size of the Kripke Structure representing $\mathcal{T}$.
		We construct a set $\mathcal{T}$ such that $\mathcal{A}_{\varphi}$ is $\mathcal{T}$-equivalent to $\varphi$.
		Since $m$ has to be greater than the size of $|\mathcal{A}_{\varphi}|$, for the exact construction of $tr_1$ and $tr_2$, we have to find a regular representation that is smaller but still contains $tr_1$ and $tr_2$.
		We can instead use the sets where $m$ is replaced with $*$.
		This also has the effect that the additional trace from case 2 and the pumped traces from case 3 are in the set.
		We also add the additional trace from case 1 so all traces used here are in the trace set.
		
		The case discrimination is still done on $tr_1$ and $tr_2$ and works the same way since if $\Pi$ only maps to $tr_1$ and $tr_2$, then it is a trace assignment over $\{tr_1,tr_2\} \in \mathcal{H}$ as well, while in the other cases, it cannot be a trace assignment over some $\mathcal{T} \in \mathcal{H}$ as it has two traces with different amounts of $p$-positions.
		\textcolor{red}{This does not show that $\varphi$ expresses $\mathcal{H}$ since the trace set $\mathcal{T}$ on the left and right side of the equivalence can/have to be different sets.}}
	
	\begin{lemma}
		In the decidable fragment, there is no quantified $\Gamma$-stuttering $H_\mu$ formula $\varphi$ that expresses $\mathcal{H}$.
	\end{lemma}
	\begin{proof}
		The main part of the proof considers formulae over at least two variables.
		The claim for one variable can be reduced to the claim for two variables by adding a conjunct $[\true]_{\pi}$ for a fresh trace variable $\pi$ to the formula.
		The proof is by induction on the length of the quantifier-prefix of $\varphi$.
		
		The base case follows immediately from \cref{lem:deltrastrictexpressivenessfix1}.
		
		In the inductive step, assume towards contradiction, that there is a formula $\varphi$ with the desired semantics.
		There are two cases, $\varphi= \forall \pi. \varphi'$ or $\varphi = \exists \pi. \varphi'$.
		
		Case 1: $\varphi = \forall \pi. \varphi'$.
		We show that $\varphi'$ also expresses $\mathcal{H}$.
		Let $\mathcal{T} \subseteq (2^\AP)^\omega$ be an arbitrary set of traces.
		There are two possibilities, $\mathcal{T} = \emptyset$ and $\mathcal{T} \neq \emptyset$.
		For the first one, both directions of the equivalence are trivial since $\emptyset \in \mathcal{H}$ and there are no trace assignments $\Pi$ over $\mathcal{T}$ binding any variables.
		Thus, both claims hold for $\mathcal{T} = \emptyset$.
		For the second, $\mathcal{T} \neq \emptyset$, we show the two directions of the equivalence in more detail.
		
		Direction 1: $\Rightarrow$\\
		%Let $\mathcal{T}$ be a set of traces and $\Pi$ be a trace assignment over $\mathcal{T}$ with $\Pi \models_{\mathcal{T}} \varphi'$.
		%\textcolor{red}{This means that $\Pi' \models_{\mathcal{T}} \varphi$ for $\Pi' = \Pi \setminus \{\pi\}$ .}
		%In particular, $\Pi'$ is also a trace assignment over $\mathcal{T}$.
		%From our assumption, we get $\mathcal{T} \in \mathcal{H}$.
		%\textcolor{blue}{
			Assume that for all trace assignments $\Pi$ over $\mathcal{T}$, we have $\Pi \models_{\mathcal{T}} \varphi$'.
			From this, we know that also $\Pi \models_{\mathcal{T}} \forall \pi. \varphi'$ for all trace assignments $\Pi$ over $\mathcal{T}$ since for a trace assignment $\Pi$ over $\mathcal{T}$ and a trace $tr \in \mathcal{T}$, $\Pi[\pi \mapsto tr]$ is also a trace assignment over $\mathcal{T}$.
			From our assumption, we get $\mathcal{T} \in \mathcal{H}$.
			%}
		
		Direction 2: $\Leftarrow$\\
		%Let $\mathcal{T} \in \mathcal{H}$ be a set of traces and $\Pi$ be a trace assignment over $\mathcal{T}$.
		%$\Pi' = \Pi \setminus \{\pi\}$ is also a trace assignment over $\mathcal{T}$.
		%From our assumption, we get that $\Pi' \models_{\mathcal{T}} \varphi$.
		%This means that for all $tr \in \mathcal{T}$, $\Pi'[\pi \mapsto tr] \models_{\mathcal{T}} \varphi'$.
		%In particular, since $\Pi = \Pi'[\pi \mapsto tr]$ for some $tr \in \mathcal{T}$, $\Pi \models_{\mathcal{T}} \varphi'$.
		%\textcolor{blue}{
			Assume that $\mathcal{T} \in \mathcal{H}$.
			From our assumption, we get that $\Pi \models_{\mathcal{T}} \forall \pi. \varphi'$ for all trace assignments $\Pi$ over $\mathcal{T}$.
			Let $\Pi$ be an arbitrary trace assignment $\Pi$ over $\mathcal{T}$.
			From $\Pi \models_{\mathcal{T}} \forall \pi. \varphi'$, we know that $\Pi [\pi \mapsto \Pi(\pi)] = \Pi \models_{\mathcal{T}} \varphi'$ since $\Pi(\pi) \in \mathcal{T}$.
			%}
		
		Case 2: $\varphi = \exists \pi. \varphi'$.
		Assume $\exists \pi. \varphi'$ expresses $\mathcal{H}$.
		Consider $\mathcal{T} = \emptyset$.
		It is easy to see that $\mathcal{T} \in \mathcal{H}$.
		\textcolor{red}{However, $\Pi \not\models_{\emptyset} \varphi$ for all trace assignments $\Pi$ and existentially quantified formulae $\varphi$.
			This leads to a contradiction.}
		
		\tbd{
			\textcolor{red}{We use the fact that there is a formula $\varphi_1$ expressing $\mathcal{H}$ iff there is a formula $\varphi_2$ expressing $\overline{\mathcal{H}} = \{ \mathcal{T} \subseteq (2^\AP)^\omega \mid \mathcal{T} \notin \mathcal{H} \}$ since one can be transformed into the other by negating it.}
			From our assumption, we get that $\forall \pi. \lnot \varphi'$ expresses $\overline{\mathcal{H}}$.
			We can show that $\lnot \varphi'$ expresses $\overline{\mathcal{H}}$ using the same arguments as in Case 1.
		}
		
		\tbd{
			Assume $\varphi = \exists \pi. \varphi'$ expresses $\mathcal{H}$.
			From the induction hypothesis we know that $\varphi'$ does not express $\mathcal{H}$.
			This means there is a set of traces $\mathcal{T} \subseteq (2^\AP)^\omega$ such that either (a) $\mathcal{T} \notin \mathcal{H}$ and for all trace assignments $\Pi$ over $\mathcal{T}$, $\Pi \models_{\mathcal{T}} \varphi'$ or (b) $\mathcal{T} \in \mathcal{H}$ and there is a trace assignment $\Pi$ over $\mathcal{T}$ such that $\Pi \not\models_{\mathcal{T}} \varphi'$.
			
			Case (a): From $\mathcal{T} \notin \mathcal{H}$ and the fact that $\varphi$ expresses $\mathcal{H}$, we know that there is a trace assignment $\Pi$ over $\mathcal{T}$ such that $\Pi \not\models_{\mathcal{T}} \varphi$.
			In particular, we have $\Pi[\pi \mapsto tr] \not\models \varphi'$ for all $tr \in \mathcal{T}$.
			However, since for $tr \in \mathcal{T}$, $\Pi[\pi \mapsto tr]$ is a trace assignment over $\mathcal{T}$, we have a contradiction.
			
			Case (b): Let $\mathcal{T}' = \Img(\Pi)$.
			Since $\Pi$ is a trace assignment over $\mathcal{T}$, we have $\mathcal{T}' \subseteq \mathcal{T}$.	
			From $\mathcal{T} \in \mathcal{H}$ and the fact that $\mathcal{H}$ is closed under taking subsets, we know that $\mathcal{T}' \in \mathcal{H}$.
			Since $\varphi$ expresses $\mathcal{H}$, we know that for all trace assignments $\Pi$ over $\mathcal{T}'$, $\Pi \models_{\mathcal{T}'} \varphi$.
			\textcolor{red}{\dots}
		}
	\end{proof}
	
	\tbd{
		In general:
		\begin{align*}
			&\forall x . P(x) \leftrightarrow R\\
			\equiv&\forall x. (P(x) \rightarrow R) \land (R \rightarrow P(x))\\
			\equiv&(\forall x. (P(x) \rightarrow R)) \land (\forall x. (R \rightarrow P(x)))\\
			\equiv&((\exists x. P(x)) \rightarrow R) \land (R \rightarrow (\forall x. P(x)))
		\end{align*}
		In our case:
		\begin{align*}
			&\forall \mathcal{T}. \forall \Pi. (\Pi \models_{\mathcal{T}} \varphi) \leftrightarrow \mathcal{T} \in \mathcal{H}\\
			\equiv&\forall \mathcal{T}. ((\exists \Pi. \Pi \models_{\mathcal{T}} \varphi) \rightarrow (\mathcal{T} \in \mathcal{H})) \land (\mathcal{T} \in \mathcal{H} \rightarrow (\forall \Pi. \Pi \models_{\mathcal{T}} \varphi))
		\end{align*}
	}
	
	\tbd{
		New proof idea:\\
		Let $\mathcal{T}^\gamma = \{\strf_{\gamma}(tr) \mid tr\in \mathcal{T} \}$ and $\mathcal{T}^\Gamma = (\mathcal{T}^{\Gamma(\pi_1)},\dots,\mathcal{T}^{\Gamma(\pi_n)})$.
		$\Pi$ is a trace assignment over $\mathcal{T}^\Gamma$ iff for all $\pi$, $\Pi(\pi) \in \mathcal{T}^{\Gamma(\pi)}$.
		We redefine the semantics for ordered trace sets $\mathcal{T}^\Gamma$ and trace assignments $\Pi$ over $\mathcal{T}^\Gamma$.
		We have:
		\begin{align*}
			&\Pi \models_{\mathcal{T}^\Gamma} \psi \text{ iff } (0,\dots,0) \in \llbracket \psi \rrbracket^{\Pi}\\
			&\Pi \models_{\mathcal{T}^\Gamma} \exists \pi. \varphi \text{ iff } \exists tr \in \mathcal{T}^{\Gamma(\pi)}. \Pi[\pi \mapsto tr] \models_{\mathcal{T}^\Gamma} \varphi \\
			&\Pi \models_{\mathcal{T}^\Gamma} \forall \pi. \varphi \text{ iff } \forall tr \in \mathcal{T}^{\Gamma(\pi)}. \Pi[\pi \mapsto tr] \models_{\mathcal{T}^\Gamma} \varphi
		\end{align*}
		Comment: first case as usual since $\Pi = \Pi^\Gamma$ when $\Pi$ is a trace assignment over $\mathcal{T}^\Gamma$.
		Lemma:
		\begin{align*}
			\Pi \models_{\mathcal{T}} \varphi \text{ iff } \Pi^\Gamma \models_{\mathcal{T}^\Gamma} \varphi
		\end{align*}
		Proof by induction using variant of \cref{lem:synchronousconnection} with $\psi$ istead of $\psi^s$ in the base case.
		
		Then proof of main theorem by normal case discrimination instead of induction.
		Base case is as before.
		Universal case can be reduced to existential case as sketched before.
		Existential case remains to show:
		
		Assume $\varphi = \exists \pi. \varphi'$ expresses $\mathcal{H}$.
		Let $n = \max\{nd(\gamma) \mid \gamma \in \Gamma\}$ and $\gamma_{\pi} = \Gamma(\pi)$.
		Let $\mathcal{T}_1 = \{t_{n+1}\}$, $\mathcal{T}_2 = \{t_{n+1},t_{n+2}\}$ and $\Pi$ be a trace assignment over $\mathcal{T}_1$.
		\textcolor{red}{We know that $\strf_{\gamma}(t_{n+1}) = \strf_{\gamma}(t_{n+2})$ for all $\gamma \in \Gamma$, so $\mathcal{T}_1^{\Gamma} = \mathcal{T}_2^{\Gamma}$ and $\mathcal{T}_1^{\gamma_\pi} = \mathcal{T}_2^{\gamma_\pi}$.}
		We have:
		\begin{align*}
			&\mathcal{T}_1 \in \mathcal{H} \\
			\text{implies } &\Pi \models_{\mathcal{T}_1} \varphi\\
			\text{implies } &\Pi^\Gamma \models_{\mathcal{T}_1^\Gamma} \varphi\\
			\text{implies } &\exists tr \in \mathcal{T}_1^{\gamma_\pi}. \Pi^\Gamma[\pi \mapsto tr] \models_{\mathcal{T}_1^\Gamma} \varphi \\
			\text{implies } &\exists tr \in \mathcal{T}_2^{\gamma_\pi}. \Pi^\Gamma[\pi \mapsto tr] \models_{\mathcal{T}_2^\Gamma} \varphi \\
			\text{implies } &\Pi^\Gamma \models_{\mathcal{T}_2^\Gamma} \varphi\\
			\text{implies } &\Pi \models_{\mathcal{T}_2} \varphi\\
			\text{implies } &\mathcal{T}_2 \in \mathcal{H}
		\end{align*}
		The last step is since our equvalence requires only the existence of such a path assignment in this direction and leads to a contradiction.
	}
\end{comment}

\begin{comment}
	\begin{lemma}
		In the decidable fragment, there is no quantified $\Gamma$-stuttering $H_\mu$ formula $\varphi$ with $\pi_1,\pi_2 \in \free(\varphi)$ such that for all sets of traces $\mathcal{T} \subseteq (2^\AP)^\omega$ and trace assignments $\Pi$, $\Pi \models_{\mathcal{T}} \varphi$ iff $p \in \Pi(\pi_1)(0)$, $p \in \Pi(\pi_2)(0)$ and $\Pi(\pi_1)$ and $\Pi(\pi_2)$ have the same finite amount of $p$-positions.
	\end{lemma}
	\begin{proof}
		The proof is by induction on the size of the quantifier prefix of $\varphi$.
		In the base case, thre are no quantifiers, i.e.$\free(\varphi) = \{\pi_1,\pi_2\}$.
		\cref{lem:deltrastrictexpressivenessfix1} gives us the claim.
		
		In the inductive step, the induction hypothesis gives us the claim for formulae $\varphi$ with $k$ quantifiers.
		We now show that it holds for $k+1$ as well.
		Assume towards contradiction, that there is a formula $\varphi$ with $k + 1$ that has the desired semantics.
		It can have two forms, $\exists \pi. \varphi'$ or $\forall \pi. \varphi'$ for some $\pi \notin \{\pi_1,\pi_2\}$ and formula $\varphi'$ with $k$ quantifiers.
		\textcolor{red}{However, both cases imply that $\varphi'$ has the desired semantics for $k$, a contradiction.}
		\tbd{
			Case 1: $\varphi = \exists \pi. \varphi'$
			
			Direction 1: $\Rightarrow$\\
			Let $\Pi$ be a trace assignment with $\Pi \models_{\mathcal{T}} \varphi'$.
			This means that $\Pi' \models_{\mathcal{T}} \varphi$ for $\Pi' = \Pi \setminus \{\pi\}$ .
			From our assumption, we get that $p \in \Pi'(\pi_1)(0)$, $p \in \Pi'(\pi_2)(0)$ and $\Pi'(\pi_1)$ and $\Pi'(\pi_2)$ have the same finite amount of $p$-positions.
			Since $\Pi(\pi_1) = \Pi'(\pi_1)$ and $\Pi(\pi_2) = \Pi'(\pi_2)$, we get $p \in \Pi(\pi_1)(0)$, $p \in \Pi(\pi_2)(0)$ and $\Pi(\pi_1)$ and $\Pi(\pi_2)$ have the same finite amount of $p$-positions.
			
			Direction 2: $\Leftarrow$\\
			Let $\Pi$ be a trace assignment with $p \in \Pi(\pi_1)(0)$, $p \in \Pi(\pi_2)(0)$ and $\Pi(\pi_1)$ and $\Pi(\pi_2)$ have the same finite amount of $p$-positions.
			$\Pi' = \Pi \setminus \{\pi\}$ fulfills the same condition.
			From our assumption, we get that $\Pi' \models_{\mathcal{T}} \varphi$.
			\textcolor{red}{Now $\Pi \models_{\mathcal{T}} \varphi'$ might not follow since the existential quantifier in $\varphi$ might choose a different trace than $\Pi(\pi)$.}
		}
		
		\tbd{
			Case 2: $\varphi = \forall \pi. \varphi'$\\
			Direction 1: $\Rightarrow$\\
			Let $\Pi$ be a trace assignment with $\Pi \models_{\mathcal{T}} \varphi'$.
			This means that $\Pi' \models_{\mathcal{T}} \varphi$ for $\Pi' = \Pi \setminus \{\pi\}$ .
			From our assumption, we get that $p \in \Pi'(\pi_1)(0)$, $p \in \Pi'(\pi_2)(0)$ and $\Pi'(\pi_1)$ and $\Pi'(\pi_2)$ have the same finite amount of $p$-positions.
			Since $\Pi(\pi_1) = \Pi'(\pi_1)$ and $\Pi(\pi_2) = \Pi'(\pi_2)$, we get $p \in \Pi(\pi_1)(0)$, $p \in \Pi(\pi_2)(0)$ and $\Pi(\pi_1)$ and $\Pi(\pi_2)$ have the same finite amount of $p$-positions.
			
			Direction 2: $\Leftarrow$\\
			Let $\Pi$ be a trace assignment with $p \in \Pi(\pi_1)(0)$, $p \in \Pi(\pi_2)(0)$ and $\Pi(\pi_1)$ and $\Pi(\pi_2)$ have the same finite amount of $p$-positions.
			$\Pi' = \Pi \setminus \{\pi\}$ fulfills the same condition.
			From our assumption, we get that $\Pi' \models_{\mathcal{T}} \varphi$.
			\textcolor{red}{This case only follows if $\Pi$ is a trace assignment over $\mathcal{T}$ since otherwise $\Pi' \models_{\mathcal{T}} \varphi$ might not insure that the claim also holds for $\Pi$.}
		}
	\end{proof}
\end{comment}

==> math/proofs/deltatequivalence.tex <==
\begin{proof}
	Follows immediately from \cref{thm:synchronousautomaton} and \cref{lem:deltatequivalencecorollary}.
\end{proof}

==> math/proofs/gammaexpressiveness.tex <==
\begin{proof}
	\tbd{By making sure that between two states where $\Delta(\pi)$ holds, there is always a state where $\Delta(\pi)$ does not hold.
	Then, by choosing $\Gamma(\pi) = \{\Delta(\pi)\}$, $\bigcirc^{\Delta}$ can be simulated with $\bigcirc^{\Gamma}\bigcirc^{\Gamma}$.}
\end{proof}

==> math/proofs/modelcheckingreduction.tex <==
\begin{IEEEproof}(of )
	Transform a general formula $\varphi$ with successor assignment $\Delta$ and a fair Kripke Structure $(\mathcal{K},F)$ into $\varphi'$ and $(\mathcal{K}',F')$ as described above.
	$\varphi'$ has size $\mathcal{O}(|\varphi|)$ and $(\mathcal{K}',F')$ has size $\mathcal{O}(|\mathcal{K}| \cdot 2^{|\varphi| \cdot \log(|\varphi|)})$.
	By construction, we have $(\mathcal{K},F) \models \varphi$ iff $(\mathcal{K}',F') \models \varphi'$.\qed
\end{IEEEproof}

==> math/proofs/mumblingstrictexpressivenesslemma2.tex <==
\begin{proof}%(of \cref{lem:deltastrictexpressivenesslemma2})
	First of all, we adapt some of the theorems from \cref{sec:fsmodelchecking} to stuttering $H_\mu$.
	In particular, we define $(\Gamma,\mathcal{T})$-equivalence in the obvious way.
	Then, it is easy to see that the results of \cref{thm:deltatequivalence} carry over to this notion of equivalence.
	
	Assume towards contradiction that there is a hyperproperty formula $\varphi = Q_n \pi_n . \dots Q_1 \pi_1 . \psi$ from stuttering $H_\mu$ with unique stuttering expressing the property $\mathcal{H}$.
	Let $\varphi_i = Q_i \pi_i \dots Q_1 \pi_1 \psi$ for $i \leq n$, with $\varphi_0 = \psi$ and $\varphi_n = \varphi$.
	Let $\Gamma$ be the stuttering assignment used in $\varphi$ and $\Gamma(\pi_i) = \gamma_i$.
	We say that a jump criterion $\gamma \in 2^\delta$ makes a type one step on a trace $\tr$ at position $i$ if $\Succ_\gamma(tr,i)$ is given by the first case in the definition of $\Succ_\gamma$.
	Similarly, we say that $\gamma$ makes a type two step on $\tr$ at position $i$ if $\Succ_\gamma(tr,i)$ is given by the second case.
	Finally, we say that $\gamma$ makes a type one/two step (without specifying a position) if it makes a type one/two step at position $0$.
	
	We choose a trace $\tr$ from $(2^{\{p\}})^\omega$ with finitely many $p$-positions maximising
	\begin{align}\label{maxset}
		|\{ i \in \{1,\dots,n\} \mid \gamma_i \text{ makes a type one step on } \tr \}|.
	\end{align}
	Since $\tr$ has only finitely many $p$-positions, we can write it as $\tr = \tr_s \cdot \emptyset^\omega$.
	Let
	\begin{align*}
		&\mathit{TypeOnePos} = \\
		&\qquad\{ i \in \{1,\dots,n\} \mid \gamma_i \text{ makes a type one step on } \tr \} \text{ and}\\
		&\mathit{TypeTwoPos} = \\
		&\qquad\{ i \in \{1,\dots,n\} \mid \gamma_i \text{ makes a type two step on } \tr \}.
	\end{align*}
	For all $\hat{\tr} \in (2^{\{p\}})^*$, we have
	\begin{align}
		&\forall i \in \mathit{TypeOnePos}: \gamma_i \text{ makes a type one step on } \hat{\tr}\cdot \tr \label{typeone}\\
		&\forall i \in \mathit{TypeTwoPos}: \gamma_i \text{ makes a type two step on } \hat{\tr}\cdot \tr. \label{typetwo}
	\end{align}
	Here, Property~(\ref{typeone}) follows from the fact that when $\gamma$ makes a type one step at position $i$, then it also makes a type one step for all earlier positions $j \leq i$.
	Property~(\ref{typetwo}) follows from the fact that $\tr$ maximises the quantity in (\ref{maxset}): if Property~(\ref{typetwo}) would not hold for some $\hat{\tr}$, then $\hat{\tr} \cdot \tr$ would have more type one positions than $\tr$ given that (\ref{typeone}) holds.
	
	We transform $\psi$ in the same way as in the reduction presented in \cref{subsec:basis}.
	That is, for every $\gamma \in \base(\varphi)$, we introduce a fresh atomic proposition $\at(\gamma)$ and replace tests and stuttering criteria in $\psi$ with the respective atomic propositions.
	This yields a formula $\psi_\at$.
	It is straightforward to see that if we \textit{properly} label traces with these atomic propositions, i.e. extend each position $i$ on a trace $\tr_p \in (2^{\{p\}})^\omega$ with the set $\{\at(\gamma) \mid \tr_p[i] \models \gamma\}$ to obtain a trace $\tr_p^\at$, then 
	\begin{align}\label{atlabelling}
		(0,\dots,0) \in \llbracket \psi \rrbracket^{\Pi[\pi \mapsto \tr_p]} \text{ iff } (0,\dots,0) \in \llbracket \psi_\at \rrbracket^{\Pi[\pi \mapsto \tr_p^\at]}
	\end{align}
	for all traces $\tr_p \in (2^{\{p\}})^\omega$, trace assignments $\Pi$ and trace variables $\pi$.
	It is also clear that the $\Gamma$-variant of \cref{thm:deltatequivalence} is applicable to $\psi_\at$ since this formula has an atomic basis.
	
	Let $\mathcal{A}_{\psi}$ thus be the automaton for $\psi_\at$ according to \cref{thm:deltatequivalence} and let $|\mathcal{A}_\psi|$ be the number of states of $\mathcal{A}_\psi$.
	Let $l = |\tr_s| + 3\cdot \mathit{nd}(\psi) + |\mathcal{A}_{\psi}| + 3$.
	Consider the following two sets of traces $\mathcal{T} = \{\tr_0,\tr_1\}$ with $\tr_0 = \{p\}^l \cdot \emptyset^l \cdot \tr$ and $\tr_1 = \emptyset^l \cdot \{p\}^l \cdot \tr$ as well as $\mathcal{T}' = \{\tr_0',\tr_1'\}$ with $\tr_0' = \{p\}^{l + |\mathcal{A}_\psi|!} \cdot \emptyset^l \cdot \tr$ and $\tr_1' = \emptyset^{l + |\mathcal{A}_\psi|!} \cdot \{p\}^l \cdot \tr$.
	%\begin{align*}
	%	&\tr_0 = \{p\}^l \cdot \emptyset^l \cdot \tr &
	%	&\tr_1 = \emptyset^l \cdot \{p\}^l \cdot \tr \\
	%	&\tr_0' = \{p\}^{l + |\mathcal{A}_\psi|!} \cdot \emptyset^l \cdot \tr &
	%	&\tr_1' = \emptyset^{l + |\mathcal{A}_\psi|!} \cdot \{p\}^l \cdot \tr
	%\end{align*}
	\begin{comment}
	\begin{align*}
		tr_0 = \{p\}^l \cdot \emptyset^l \cdot tr &&
		tr_1 = \emptyset^l \cdot \{p\}^l \cdot tr
	\end{align*}
	and
	\begin{align*}
		tr_0' = \{p\}^{l + |\mathcal{A}_\psi|!} \cdot \emptyset^l \cdot tr &&
		tr_1' = \emptyset^{l + |\mathcal{A}_\psi|!} \cdot \{p\}^l \cdot tr
	\end{align*}
	\end{comment}
	%Also consider the trace sets $\mathcal{T} = \{\tr_0,\tr_1\}$ and $\mathcal{T}' = \{\tr_0',\tr_1'\}$.
	It is easy to see that $\mathcal{T} \in \mathcal{H}$ while $\mathcal{T}' \notin \mathcal{H}$.
	For any trace assignment $\Pi$ over $\mathcal{T}$, let $\Pi'$ be the trace assignment defined by
	\begin{align*}
		\Pi'(\pi_j) = \begin{cases}
			\tr_0' &\quad \text{if } \Pi(\pi_j) = \tr_0 \\
			\tr_1' &\quad \text{if } \Pi(\pi_j) = \tr_1.
		\end{cases}
	\end{align*}
	Additionally, let $\Pi_\at$ and $\Pi_\at'$ be the variants of $\Pi$ and $\Pi'$, where every trace $\tr_0,\tr_1,\tr_0'$ and $\tr_1'$ has been replaced with its properly labelled variant $\tr_0^\at,\tr_1^\at,\tr_0'^\at$ and $\tr_1'^\at$, respectively.
	The trace sets $\mathcal{T}_\at$ and $\mathcal{T}_\at'$ are defined analogously.
	Below, we show by induction over $j$ that for all trace assignments $\Pi$ over $\mathcal{T}$ and $j \in \{0,\dots,n\}$, $\Pi \models_{\mathcal{T}} \varphi_j$ implies $\Pi' \models_{\mathcal{T}'} \varphi_j$.
	For $j = n$, this would mean that $\mathcal{T} \in \mathcal{H}$, i.e. $\mathcal{T} \models \varphi_n$, implies $\mathcal{T}' \models \varphi_n$, i.e. $\mathcal{T}' \in \mathcal{H}$, a contradiction.
	
	\begin{figure}
		\resizebox{\columnwidth}{!}{
			\begin{tikzpicture}
				\node at (-5,0) {\strut Trace};
				\node at (-4,0) {\strut Type};
				
				\node at (-5,-0.5) {$\tr_0$};
				\node at (-4,-0.5) {$1$};
				\node at (-3,-0.5) {$p$};
				\node at (-2.5,-0.5) {$\dots$};
				\node at (-2,-0.5) {$p$};
				\node at (-1,-0.5) {$p$};
				\node at (-0.5,-0.5) {$\dots$};
				\node at (0,-0.5) {$p$};
				\node at (1,-0.5) {$p$};
				\node at (1.5,-0.5) {$\dots$};
				\node at (2,-0.5) {$p$};
				\node at (2.5,-0.5) {$\emptyset^l$};
				\node at (3,-0.5) {$\tr_s$};
				\node at (3.5,-0.5) {$\emptyset$};
				\node at (4,-0.5) {$\dots$};
				\node at (5,-0.5) {$\emptyset^\omega$};
				
				\node at (-5,-1) {$\tr_0$};
				\node at (-4,-1) {$2$};
				\node at (-3,-1) {$p$};
				\node at (-2.5,-1) {$\dots$};
				\node at (-2,-1) {$p$};
				\node at (-1,-1) {$p$};
				\node at (-0.5,-1) {$\dots$};
				\node at (0,-1) {$p$};
				\node at (1,-1) {$p$};
				\node at (1.5,-1) {$\dots$};
				\node at (2,-1) {$p$};
				\node at (2.5,-1) {$\emptyset^l$};
				\node at (3,-1) {$\tr_s$};
				\node at (3.5,-1) {$\emptyset$};
				\node at (4,-1) {$\dots$};
				\node at (5,-1) {$\emptyset^\omega$};
				
				\node at (-5,-1.5) {$\tr_1$};
				\node at (-4,-1.5) {$1$};
				\node at (-3,-1.5) {$\emptyset$};
				\node at (-2.5,-1.5) {$\dots$};
				\node at (-2,-1.5) {$\emptyset$};
				\node at (-1,-1.5) {$\emptyset$};
				\node at (-0.5,-1.5) {$\dots$};
				\node at (0,-1.5) {$\emptyset$};
				\node at (1,-1.5) {$\emptyset$};
				\node at (1.5,-1.5) {$\dots$};
				\node at (2,-1.5) {$\emptyset$};
				\node at (2.5,-1.5) {$p^l$};
				\node at (3,-1.5) {$\tr_s$};
				\node at (3.5,-1.5) {$\emptyset$};
				\node at (4,-1.5) {$\dots$};
				\node at (5,-1.5) {$\emptyset^\omega$};
				
				\node at (-5,-2) {$\tr_1$};
				\node at (-4,-2) {$2$};
				\node at (-3,-2) {$\emptyset$};
				\node at (-2.5,-2) {$\dots$};
				\node at (-2,-2) {$\emptyset$};
				\node at (-1,-2) {$\emptyset$};
				\node at (-0.5,-2) {$\dots$};
				\node at (0,-2) {$\emptyset$};
				\node at (1,-2) {$\emptyset$};
				\node at (1.5,-2) {$\dots$};
				\node at (2,-2) {$\emptyset$};
				\node at (2.5,-2) {$p^l$};
				\node at (3,-2) {$\tr_s$};
				\node at (3.5,-2) {$\emptyset$};
				\node at (4,-2) {$\dots$};
				\node at (5,-2) {$\emptyset^\omega$};
				
				\draw[ultra thick,color=red] (4.5,-0.3) -- (4.5,-0.7);
				\draw[ultra thick,color=red] (-1.5,-0.8) -- (-1.5,-1.2);
				
				\draw[ultra thick,color=red] (4.5,-1.3) -- (4.5,-1.7);
				\draw[ultra thick,color=red] (-1.5,-1.8) -- (-1.5,-2.2);
				
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (-3,-3) -- (-2,-3) node[left]{$|\tr_s| + 2 \cdot \mathit{nd}(\psi) + 1$};
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (-1,-3) -- (0,-3) node[midway]{$|\mathcal{A}_\psi| + 1$};
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (1,-3) -- (2,-3) node[midway]{$\mathit{nd}(\psi) + 1$};
			\end{tikzpicture}
		}
		\caption{Positions reached in component $i$ of the input word $w_{\Pi_\at^\Gamma}$ after $|\tr_s| + 2\cdot\mathit{nd}(\psi) + 1$ steps in an accepting run of $\mathcal{A}_\psi$.
		There are four cases where $\Pi(\pi_i) = \tr_0$ or $\Pi(\pi_i) = \tr_1$ and $i \in \mathit{TypeOnePos}$ or $i \in \mathit{TypeTwoPos}$.
		}
		\label{fig:acceptingrun}
	\end{figure}
	
	In the \textbf{base case}, assume that $\Pi \models_{\mathcal{T}} \psi$.
	By Property~(\ref{atlabelling}), we have $(0,\dots,0) \in \llbracket \psi_\at \rrbracket^{\Pi_\at}$.
	Since $\mathcal{A}_\psi$ is $(\Gamma,\mathcal{T}_\at)$-equivalent
	%\footnote{In fact, for unquantified formulae $\psi$, we have an automaton $\mathcal{A}_\psi$ that is $\hat{\mathcal{T}}$-equivalent for arbitrary sets of traces $\hat{\mathcal{T}}$.}
	 to $\psi_\at$ by the $\Gamma$-variant of \cref{thm:deltatequivalence}, we have an accepting run of $\mathcal{A}_\psi$ on $w_{\Pi_\at^\Gamma}$.
	%We have two cases, $|\mathit{TypeOnePos}| = n$ and $|\mathit{TypeOnePos}| \neq n$.
	%
	%In the first case, $\gamma_i$ makes a type one step on both $\tr_0$ and $\tr_1$ for all $i$ by Property~(\ref{typeone}).
	%With \cref{lem:ltlclaim}, we can see that we can add $\{p\}$-positions to the front of $\tr_0$ and $\emptyset$-positions to the front of $\tr_1$ while keeping their summarisation with respect to all $\gamma_i$ the same.
	%In particular, we can add $|\mathcal{A}_\psi|!$ such positions and obtain $\Pi^\Gamma = \Pi'^\Gamma$.
	%Thus, $w_{\Pi'^\Gamma} = w_{\Pi^\Gamma} \in \mathcal{L}(\mathcal{A}_\psi)$.
	%We conclude $\Pi' \models_{\mathcal{T}'} \psi$.
	%
	%In the second case,
	Consider the accepting run of $\mathcal{A}_\psi$ after $l - |\mathcal{A}_\psi| - \mathit{nd}(\psi) - 2 = |\tr_s| + 2\cdot\mathit{nd}(\psi) + 1$ steps.
	This situation is depicted in \Cref{fig:acceptingrun}.
	On the one hand, for all $i \in \mathit{TypeOnePos}$, the suffix left to read in component $i$ of $w_{\Pi_\at^\Gamma}$ is $\emptyset^\omega$.
	This is due to the fact that by \cref{lem:ltlclaim} and Property~(\ref{typeone}), it takes at most $\mathit{nd}(\psi)$ applications of $\Succ_{\gamma_i}$ to move over the prefix $\{p\}^l$ of $\tr_0^\at$, by the same argument it takes at most $\mathit{nd}(\psi)$ applications of $\Succ_{\gamma_i}$ to move over $\emptyset^l$ and finally, it takes at most $|\tr_s|$ applications of $\Succ_{\gamma_i}$ to move over $\tr_s$.
	The argumentation for $\tr_1^\at$ is analogous.
	This case is represented in line one and three in \Cref{fig:acceptingrun}.
	On the other hand, for all $i \in \mathit{TypeTwoPos}$, the suffix left to read in component $i$ of $w_{\Pi_\at^\Gamma}$ is either $\{p\}^{|\mathcal{A}_\psi|+\mathit{nd}(\psi)+2} \cdot \emptyset^l \cdot \tr$ if $\Pi(\pi_i) = \tr_0$ or $\emptyset^{|\mathcal{A}_\psi|+\mathit{nd}(\psi)+2} \cdot \{p\}^l \cdot \tr$ if $\Pi(\pi_i) = \tr_1$.
	This is due to the fact that by Property~(\ref{typetwo}), $\gamma_i$ makes only type two steps on $\tr_0$ and $\tr_1$.
	This case is represented in line two and four in \Cref{fig:acceptingrun}.
	Thus, during the next $|\mathcal{A}_\psi| + 1$ steps, the automaton reads the same symbols on all traces:
	For all $i \in \mathit{TypeOnePos}$, there are only $\emptyset$-symbols on $\tr_0$ in these positions, which by \cref{lem:ltlclaim} and the fact that the suffix is $\emptyset^\omega$ all have the same extended labelling in $\tr_0^\at$.
	For all $i \in \mathit{TypeTwoPos}$, there are only $\{p\}$-symbols on $\tr_1$ in these positions.
	By \cref{lem:ltlclaim} and the fact that the next $\mathit{nd}(\psi) + 1$ positions after these steps are also $\{p\}$-symbols on $\tr_1$, the extended labelling in $\tr_1^\at$ is the same for these steps as well.
	%Thus, during the next $|\mathcal{A}_\psi| + 1$ steps, the automaton reads only $\emptyset$-symbols for all $i \in \mathit{TypeOnePos}$ and either only $\{p\}$-symbols or only $\emptyset$-symbols for all $i \in \mathit{TypeTwoPos}$.
	During these steps where the same symbol is seen on each trace, at least one state $q$ of $\mathcal{A}_\psi$ is visited twice.
	Let $k$ be the number of steps between the two visits of $q$.
	By adding a multiple $m$ of $k$ $\{p\}$-positions to the front of $\tr_0$ and a multiple $m$ of $k$ $\emptyset$-positions to the front of $\tr_1$, we do not change the acceptance of $\mathcal{A}_\psi$ as the run can repeat the loop from $q$ to $q$ $m$ times and then proceed as before.
	This situation is depicted in \Cref{fig:pumpedrun}.
	This is for three reasons: (i) for $i \in \mathit{TypeTwoPos}$, the symbols are added where $\mathcal{A}_\psi$ loops from $q$ to $q$ (red positions in line two and four in \Cref{fig:pumpedrun}), (ii) for $i \in \mathit{TypeOnePos}$, still at most $\mathit{nd}(\psi)$ applications of $\Succ_{\gamma_i}$ are needed to skip over $\{p\}^{l + m \cdot k}$ or $\emptyset^{l + m \cdot k}$ due to \cref{lem:ltlclaim} (blue positions in line one and three in \Cref{fig:pumpedrun}) and $m \cdot k$ $\emptyset$-positions can be \textit{added} to the $\emptyset^\omega$ suffix of $\Pi(\pi_i)$ where $\mathcal{A}_\psi$ loops from $q$ to $q$ without changing the trace (red positions in line one and three in \Cref{fig:pumpedrun}), and (iii) by the same argument as before, the extended labelling on the added positions is the same as on the position directly after.
	By choosing $m = \frac{|\mathcal{A}_\psi|!}{k}$, we obtain $\tr_0'^\at$ from $\tr_0^\at$ and $\tr_1'^\at$ from $\tr_1^\at$.
	We thus have an accepting run of $\mathcal{A}_\psi$ on $w_{\Pi_\at'^\Gamma}$ and conclude $\Pi' \models_{\mathcal{T}'} \psi$ by again using Property~(\ref{atlabelling}) and the fact that $\mathcal{A}_\psi$ is also $(\Gamma,\mathcal{T}_\at')$-equivalent to $\psi_\at$.
	
	\begin{figure}
		\resizebox{\columnwidth}{!}{
			\begin{tikzpicture}
				\node at (-5,0) {\strut Trace};
				\node at (-4,0) {\strut Type};
				
				\node at (-5,-0.5) {$\tr_0'$};
				\node at (-4,-0.5) {$1$};
				\node at (-3,-0.5) {$p$};
				\node at (-2.5,-0.5) {$\dots$};
				\node at (-2,-0.5) {$p$};
				\node at (-1,-0.5) {$p$};
				\node at (-0.5,-0.5) {$\dots$};
				\node at (0,-0.5) {$p$};
				\node at (1,-0.5) {$p$};
				\node at (1.5,-0.5) {$\dots$};
				\node at (2,-0.5) {$p$};
				\node at (2.5,-0.5) {$\emptyset^l$};
				\node at (3,-0.5) {$\tr_s$};
				\node at (3.5,-0.5) {$\emptyset$};
				\node at (4,-0.5) {$\dots$};
				\node at (5,-0.5) {$\emptyset^\omega$};
				
				\node at (-5,-1) {$\tr_0'$};
				\node at (-4,-1) {$2$};
				\node at (-3,-1) {$p$};
				\node at (-2.5,-1) {$\dots$};
				\node at (-2,-1) {$p$};
				\node at (-1,-1) {$p$};
				\node at (-0.5,-1) {$\dots$};
				\node at (0,-1) {$p$};
				\node at (1,-1) {$p$};
				\node at (1.5,-1) {$\dots$};
				\node at (2,-1) {$p$};
				\node at (2.5,-1) {$\emptyset^l$};
				\node at (3,-1) {$\tr_s$};
				\node at (3.5,-1) {$\emptyset$};
				\node at (4,-1) {$\dots$};
				\node at (5,-1) {$\emptyset^\omega$};
				
				\node at (-5,-1.5) {$\tr_1'$};
				\node at (-4,-1.5) {$1$};
				\node at (-3,-1.5) {$\emptyset$};
				\node at (-2.5,-1.5) {$\dots$};
				\node at (-2,-1.5) {$\emptyset$};
				\node at (-1,-1.5) {$\emptyset$};
				\node at (-0.5,-1.5) {$\dots$};
				\node at (0,-1.5) {$\emptyset$};
				\node at (1,-1.5) {$\emptyset$};
				\node at (1.5,-1.5) {$\dots$};
				\node at (2,-1.5) {$\emptyset$};
				\node at (2.5,-1.5) {$p^l$};
				\node at (3,-1.5) {$\tr_s$};
				\node at (3.5,-1.5) {$\emptyset$};
				\node at (4,-1.5) {$\dots$};
				\node at (5,-1.5) {$\emptyset^\omega$};
				
				\node at (-5,-2) {$\tr_1'$};
				\node at (-4,-2) {$2$};
				\node at (-3,-2) {$\emptyset$};
				\node at (-2.5,-2) {$\dots$};
				\node at (-2,-2) {$\emptyset$};
				\node at (-1,-2) {$\emptyset$};
				\node at (-0.5,-2) {$\dots$};
				\node at (0,-2) {$\emptyset$};
				\node at (1,-2) {$\emptyset$};
				\node at (1.5,-2) {$\dots$};
				\node at (2,-2) {$\emptyset$};
				\node at (2.5,-2) {$p^l$};
				\node at (3,-2) {$\tr_s$};
				\node at (3.5,-2) {$\emptyset$};
				\node at (4,-2) {$\dots$};
				\node at (5,-2) {$\emptyset^\omega$};
				
				\draw[fill,color=blue,opacity=0.2] (-1.5,-0.3) -- (-1.5,-0.7) -- (0.5,-0.7) -- (0.5,-0.3) -- cycle;
				\draw[fill,color=red,opacity=0.2] (4.5,-0.3) -- (4.5,-0.7) -- (5.5,-0.7) -- (5.5,-0.3) -- cycle;
				\draw[fill,color=red,opacity=0.2] (-1.5,-0.8) -- (-1.5,-1.2) -- (0.5,-1.2) -- (0.5,-0.8) -- cycle;
				
				\draw[fill,color=blue,opacity=0.2] (-1.5,-1.3) -- (-1.5,-1.7) -- (0.5,-1.7) -- (0.5,-1.3) -- cycle;
				\draw[fill,color=red,opacity=0.2] (4.5,-1.3) -- (4.5,-1.7) -- (5.5,-1.7) -- (5.5,-1.3) -- cycle;
				\draw[fill,color=red,opacity=0.2] (-1.5,-1.8) -- (-1.5,-2.2) -- (0.5,-2.2) -- (0.5,-1.8) -- cycle;
				
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (-3,-3) -- (-2,-3) node[left]{$|\tr_s| + 2 \cdot \mathit{nd}(\psi) + 1$};
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (-1,-3) -- (0,-3) node[midway]{$|\mathcal{A}_\psi| + 1 + |\mathcal{A}_\psi|!$};
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (1,-3) -- (2,-3) node[pos = 1]{$\mathit{nd}(\psi) + 1$};
			\end{tikzpicture}
		}
		\caption{Accepting run of $\mathcal{A}_\psi$ on $w_{\Pi_\at'^\Gamma}$ after the application of the pumping argument.
		We have four cases for component $i$ of the input word where $\Pi(\pi_i) = \tr_0$ or $\Pi(\pi_i) = \tr_1$ and $i \in \mathit{TypeOnePos}$ or $i \in \mathit{TypeTwoPos}$.
		Loops in the automaton are added in the red positions.
		In the areas marked blue, positions are added as well, however these positions are skipped when the traces are progressed with type one steps.
		The valuations of tests in the additional positions are the same as in the position directly before them since there are at least $\mathit{nd}(\psi) + 1$ successive positions with the same symbol.}
		\label{fig:pumpedrun}
	\end{figure}
	
	The \textbf{inductive step} considers the quantifiers $Q_1,\dots,Q_n$ and follows straightforwardly from the semantics of quantifiers and the induction hypothesis.
	\begin{comment}
	In the \textbf{inductive step}, assume that the claim holds for $j$.
	We show the implication for $j+1$.
	There are two cases $Q_{j+1} = \exists$ and $Q_{j+1} = \forall$.
	
	In the first case, we have $\varphi_{j+1} = \exists \pi_{j+1}. \varphi_j$.
	We have:
	\begin{align*}
		&\Pi \models_{\mathcal{T}} \varphi_{j+1} \\
		\Rightarrow\quad& \exists \tr \in \mathcal{T}. \Pi[\pi_{j+1} \mapsto \tr] \models_{\mathcal{T}} \varphi_{j} \\
		\Rightarrow\quad& \Pi[\pi_{j+1} \mapsto \tr_0] \models_{\mathcal{T}} \varphi_j \text{ or } \Pi[\pi_{j+1} \mapsto \tr_1] \models_{\mathcal{T}} \varphi_j \\
		\Rightarrow\quad& \Pi'[\pi_{j+1} \mapsto \tr_0'] \models_{\mathcal{T}'} \varphi_j \text{ or } \Pi'[\pi_{j+1} \mapsto \tr_1'] \models_{\mathcal{T}'} \varphi_j \\
		\Rightarrow\quad& \exists \tr' \in \mathcal{T}'. \Pi'[\pi_{j+1} \mapsto \tr'] \models_{\mathcal{T}'} \varphi_{j} \\
		\Rightarrow\quad& \Pi' \models_{\mathcal{T}'} \varphi_{j+1}
	\end{align*}
	
	The second case, $Q_{j+1} = \forall$, is analogous.
	\end{comment}
\end{proof}

==> math/proofs/mumblingstrictltlexpressiveness.tex <==
\begin{proof}(of \cref{lem:mumblingstrictltlexpressiveness})
	Follows immediately from \cref{lem:mumblingstrictexpressivenesslemma1} and \cref{lem:mumblingstrictexpressivenesslemma2}.
\end{proof}

==> math/proofs/stutteringexpressiveness.tex <==
% !TeX spellcheck = en_US
\begin{proof}(of \cref{lem:stutteringexpressiveness})
	We show this claim by presenting a translation from a mumbling $H_\mu$ formula $\varphi$ with unique mumbling to an equivalent stuttering $H_\mu$ formula $\hat{\varphi}$ with unique stuttering.
	
	Let $\varphi = Q_n \pi_n . \dots Q_1 \pi_1 . \psi$ be a mumbling $H_\mu$ formula with unique mumbling using the successor assignment $\Delta$.
	We assume $\varphi$ is in positive form, i.e. negation occurs only in front of tests in $\psi$.
	As in other proofs, we define $\varphi_i = Q_i \pi_i . \dots Q_1 \pi_1 . \psi$ with $\varphi_0 = \psi$ and $\varphi_n = \varphi$.
	We assume w.l.o.g. that every test in $\psi$ is either only applied on the first position of a trace or only on later positions.
	This can be achieved by unrolling fixpoints so that all tests are either unguarded (and thus only apply to the first position) or in scope of at least one $\bigcirc^\Delta$ operator (and thus only apply to later positions).
	
	We first define a stuttering criterion $\Gamma$ by specifying $\Gamma(\pi)$ for each trace variable $\pi$.
	For this, let $\pi \in \{\pi_1,\dots,\pi_n\}$ be a trace variable with $\delta = \Delta(\pi)$ as well as $[\delta_1]_{\pi},\dots,[\delta_m]_{\pi}$ be the tests applied on $\pi$.
	We introduce $\bigcirc^{\delta} \delta'$ as an abbreviation for the trace formula $\bigcirc(\lnot \delta \mathcal{U} (\delta \land \delta'))$.
	Intuitively, $\bigcirc^{\delta} \delta'$ asserts that (i) there is a future position where $\delta$ holds and (ii) $\delta'$ holds at the next $\delta$ position.
	We define
	\begin{align*}
		\gamma_0 &= (\mathcal{F}\mathcal{G} \lnot \delta) \land \mu Y . ((\bigcirc^{\delta} \bigcirc \mathcal{G} \lnot \delta) \lor (\bigcirc^{\delta}\bigcirc^{\delta} Y)) \\
		\gamma_j &= (\mathcal{G}\mathcal{F} \delta) \land \mu Y . (\bigcirc^{\delta} \lnot \delta_j \lor \bigcirc^{\delta} (\delta_j \land \bigcirc^\delta (\delta_j \land Y))) \\
		\tilde{\gamma}_i &= (\mathcal{G}\mathcal{F} \delta) \land \mu Y . (\bigcirc^{\delta} \delta_j \lor \bigcirc^{\delta} (\lnot \delta_j \land \bigcirc^\delta (\lnot \delta_j \land Y)))
	\end{align*}
	for $j \in \{1,\dots,m\}$.
	We set 
	\begin{align*}
		\Gamma(\pi) = \{\gamma_0,\gamma_1,\dots,\gamma_m,\tilde{\gamma}_1,\dots,\tilde{\gamma}_m\}
	\end{align*}
	and replace every next operator $\bigcirc^\Delta$ in $\psi$ with $\bigcirc^\Gamma$.
	
	Next, we replace every test $[\delta_j]_\pi$ in scope of a $\bigcirc^\Delta$ operator by $[(\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)]_\pi$, obtaining a multitrace formula $\hat{\psi}$.
	$\hat{\varphi}$ is then given as $Q_n \pi_n . \dots Q_1 \pi_1 . \hat{\psi}$.
	We use the notation $\hat{\varphi}_i$ analogously defined as $\varphi_i$ and show by induction on $i$ that:
	
	\textbf{Main claim:} for all sets of traces $\mathcal{T}$ and trace assignments $\Pi$ over $\mathcal{T}$
	\begin{align*}
		\Pi \models_{\mathcal{T}} \varphi_i \text{ iff } \Pi \models_{\mathcal{T}} \hat{\varphi}_i.
	\end{align*}
	For $i = n$, this yields the equivalence of $\varphi$ and $\hat{\varphi}$.
	
	Before we perform the induction, let us explain the intuition of the translation.
	First, consider a trace where $\delta$ is true on a finite number of positions.
	This case is illustrated in \Cref{fig:intuition1}.
	On such traces, the formulae $\gamma_j$ or $\tilde{\gamma}_j$ never change their valuation since their first conjunct is not fulfilled.
	We thus use $\gamma_0$ to progress on such traces.
	Intuitively, the formula expresses that (i) there are only finitely many $\delta$-positions on the trace (expressed by $\mathcal{F}\mathcal{G}\lnot \delta$) and (ii) there is an odd number of $\delta$-positions after the current position (expressed by the fixpoint formula $\mu Y . ((\bigcirc^{\delta} \bigcirc \mathcal{G} \lnot \delta_i) \lor (\bigcirc^{\delta}\bigcirc^{\delta} Y))$).
	In the fixpoint formula, $\bigcirc^{\delta} \bigcirc \mathcal{G} \lnot \delta_i$ identifies the positions with exactly one $\delta$-position after them.
	Additionally, the use of $\bigcirc^{\delta}\bigcirc^{\delta} Y$ in each fixpoint iteration advances by two $\delta$-positions and thus expresses that a position satisfying the fixpoint is an even number of $\delta$-positions away from the base case.
	Since the number of $\delta$-positions left on the trace is decreased by one whenever a $\delta$-position is encountered, $\gamma_0$ changes its valuation exactly at the positions where $\delta$ holds.
	
	\begin{figure}
		%\resizebox{\columnwidth}{!}{
			\begin{tikzpicture}
				\node at (-6,1.5) {\#};
				\node at (-5,1.5) {4};
				\node at (-4,1.5) {4};
				\node at (-3,1.5) {3};
				\node at (-2,1.5) {3};
				\node at (-1,1.5) {2};
				\node at (0,1.5) {1};
				\node at (1,1.5) {1};
				\node at (2,1.5) {0};
				\node at (3,1.5) {0};
				\node at (4,1.5) {0};
				\node at (5,1.5) {0};
				
				\node at (-6,1) {$\models\gamma_0$};
				\node at (-5,1) {\xmark};
				\node at (-4,1) {\xmark};
				\node at (-3,1) {\cmark};
				\node at (-2,1) {\cmark};
				\node at (-1,1) {\xmark};
				\node at (0,1) {\cmark};
				\node at (1,1) {\cmark};
				\node at (2,1) {\xmark};
				\node at (3,1) {\xmark};
				\node at (4,1) {\xmark};
				\node at (5,1) {\xmark};
				
				\node at (-5,0) {$\delta$};
				\node at (-4,0) {$\lnot\delta$};
				\node at (-3,0) {$\delta$};
				\node at (-2,0) {$\lnot\delta$};
				\node at (-1,0) {$\delta$};
				\node at (0,0) {$\delta$};
				\node at (1,0) {$\lnot\delta$};
				\node at (2,0) {$\delta$};
				\node at (3,0) {$\lnot\delta$};
				\node at (4,0) {$\lnot\delta$};
				\node at (5,0) {$\lnot\delta$};
				\node at (6,0) {\dots};
				
				\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (3,-1) -- (6,-1) node[midway]{Suffix where $\delta$ does not hold};
				%\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (0,-1) -- (1,-1) node[midway]{Fixpoint base case};
				%\draw [decorate,decoration={brace,amplitude=8pt,mirror,raise=-4ex}] (-3,-1) -- (-2,-1) node[midway]{First Fixpoint iteration};
			\end{tikzpicture}
		%}
		\caption{Valuation of $\gamma_0$ on trace with finitely many $\delta$-positions.
		The numbers in the line labeled \# indicate the number of $\delta$-positions after the current position.}
		\label{fig:intuition1}
	\end{figure}
		
	Next, consider a trace where $\delta$ holds infinitely often.
	This case is illustrated in \Cref{fig:intuition2}.
	On such traces, the formulae $\gamma_0$ never changes its valuation since the first conjunct is not fulfilled.
	Here, we use formulae $\gamma_j$ and $\tilde{\gamma}_j$ to progress on the trace.
	For these formulae, the first conjunct $\mathcal{G}\mathcal{F} \delta$ is used to identify the case that there is an infinite number of $\delta$-positions.
	Additionally, we have:
	\begin{enumerate}
		\item $\gamma_j$ is satisfied on positions with an even number of positions that satisfy $\delta_j \land \delta$ after the current position and before the next position satisfying $\lnot \delta_j \land \delta$.
		The base case of the fixpoint formula ($\bigcirc^{\delta} \lnot \delta_j$) identifies positions with no further $\delta$-positions between them and the next position where $\lnot \delta_j \land \delta$ is true.
		Each fixpoint iteration (by $\bigcirc^{\delta} (\delta_j \land \bigcirc^\delta (\delta_j \land Y))$) advances by two $\delta$-positions where $\delta_j$ is true as well.
		\item Analogously, $\tilde{\gamma}_j$ is satisfied on positions with an even number of positions that satisfy $\lnot \delta_j \land \delta$ after the current position and before the next position satisfying $\delta_j \land \delta$.
	\end{enumerate}

	\begin{figure}
		%\resizebox{\columnwidth}{!}{
			\begin{tikzpicture}
				\node at (-6,1.5) {\#};
				\node at (-5,1.5) {0};
				\node at (-4,1.5) {0};
				\node at (-3,1.5) {3};
				\node at (-2,1.5) {3};
				\node at (-1,1.5) {2};
				\node at (0,1.5) {1};
				\node at (1,1.5) {1};
				\node at (2,1.5) {0};
				\node at (3,1.5) {0};
				\node at (4,1.5) {?};
				\node at (5,1.5) {?};
				
				\node at (-6,1) {$\models\gamma_j$};
				\node at (-5,1) {\cmark};
				\node at (-4,1) {\cmark};
				\node at (-3,1) {\xmark};
				\node at (-2,1) {\xmark};
				\node at (-1,1) {\cmark};
				\node at (0,1) {\xmark};
				\node at (1,1) {\xmark};
				\node at (2,1) {\cmark};
				\node at (3,1) {\cmark};
				\node at (4,1) {?};
				\node at (5,1) {?};
				
				\node at (-6,0) {\#};
				\node at (-5,0) {1};
				\node at (-4,0) {1};
				\node at (-3,0) {0};
				\node at (-2,0) {0};
				\node at (-1,0) {0};
				\node at (0,0) {0};
				\node at (1,0) {0};
				\node at (2,0) {1};
				\node at (3,0) {1};
				\node at (4,0) {0};
				\node at (5,0) {?};
				
				\node at (-6,-0.5) {$\models\tilde{\gamma}_j$};
				\node at (-5,-0.5) {\xmark};
				\node at (-4,-0.5) {\xmark};
				\node at (-3,-0.5) {\cmark};
				\node at (-2,-0.5) {\cmark};
				\node at (-1,-0.5) {\cmark};
				\node at (0,-0.5) {\cmark};
				\node at (1,-0.5) {\cmark};
				\node at (2,-0.5) {\xmark};
				\node at (3,-0.5) {\xmark};
				\node at (4,-0.5) {\cmark};
				\node at (5,-0.5) {?};
				
				\node at (-5,-1.5) {$\delta$};
				\node at (-4,-1.5) {$\lnot\delta$};
				\node at (-3,-1.5) {$\delta$};
				\node at (-2,-1.5) {$\lnot\delta$};
				\node at (-1,-1.5) {$\delta$};
				\node at (0,-1.5) {$\delta$};
				\node at (1,-1.5) {$\lnot\delta$};
				\node at (2,-1.5) {$\delta$};
				\node at (3,-1.5) {$\lnot\delta$};
				\node at (4,-1.5) {$\delta$};
				\node at (5,-1.5) {$\delta$};
				\node at (6,-1.5) {\dots};
				
				\node at (-5,-2) {$\delta_j$};
				\node at (-4,-2) {};
				\node at (-3,-2) {$\lnot\delta_j$};
				\node at (-2,-2) {};
				\node at (-1,-2) {$\delta_j$};
				\node at (0,-2) {$\delta_j$};
				\node at (1,-2) {};
				\node at (2,-2) {$\delta_j$};
				\node at (3,-2) {};
				\node at (4,-2) {$\lnot\delta_j$};
				\node at (5,-2) {$\delta_j$};
				\node at (6,-2) {\dots};
			\end{tikzpicture}
		%}
		\caption{Valuation of $\gamma_j$ and $\tilde{\gamma}_j$ on trace with infinitely many $\delta$-positions.
		The numbers in the line labeled \# indicate the number of relevant positions for each position as described in 1) and 2).}
		\label{fig:intuition2}
	\end{figure}

	As a consequence of 1) and 2), either $\gamma_j$ or $\tilde{\gamma}_j$ changes its value on all $\delta$-positions if there are infinitely many $\delta$-positions where $\delta_j$ holds and infinitely many $\delta$-positions where $\lnot \delta_j$ holds, i.e. the valuation of $\delta_j$ on $\delta$-positions changes infinitely often.
	If this is not the case, i.e. if the valuation of $\delta_j$ is constant for all $j \in \{1,\dots,m\}$ on $\delta$-positions from some point onward, $\gamma_j$ or $\tilde{\gamma}_j$ change value on all $\delta$-positions up to that point.
	Thus, $\Gamma$ advances a trace exactly like $\Delta$ except in situations where there are infinitely many $\delta$-positions and the valuation of all tests $\delta_j$ is constant on $\delta$ positions on the suffix of the trace.
	However, in this case we can use the fact that the valuation for all tests is constant and perform future tests on arbitrary $\delta$-positions.
	This is done by replacing tests $[\delta_j]_\pi$ by $[(\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)]_\pi$.
	The disjunct $(\lnot \delta \mathcal{U} (\delta \land \delta_j))$ is equivalent to $\delta_j$ if the stuttering assignment has correctly advanced to a $\delta$-position and tests at the next $\delta$-position if the stuttering assignment has not correctly advanced.
	Additionally, $(\delta_j \land \lnot \mathcal{F} \delta)$ accounts for the tests that are performed on the suffix where $\delta$ does not hold in the case with finitely many $\delta$-positions.
	
	We formalise these intuitions in additional claims, which we show separately.
	For these claims, we classify positions on traces bound by $\Pi$ into three categories.
	For a trace variable $\pi$ with $\Pi(\pi) = \tr$, $\Delta(\pi) = \delta$ and $\Gamma(\pi) = \gamma$ (as defined above) and a position $i$, we say that $i$ is a position of Type a), b) or c) on $\pi$ based on the following conditions:
	\begin{itemize}
		\item \textit{Type a):} There are only finitely many $k$ such that $\tr[k] \models \delta$.
		\item \textit{Type b):} There are infinitely many $k$ such that $\tr[k] \models \delta$ and there are $j \in \{1,\dots,m\}$, $k > i$ and $l > i$ such that $\tr[k] \models \delta \land \delta_j$ and $\tr[l] \models \delta \land \lnot \delta_j$.
		\item \textit{Type c):} Neither of the previous conditions applies.
		This is equivalent to the condition that there are infinitely many $k$ with $\tr[k] \models \delta$ and for all $j \in \{1,\dots,m\}$ and $k,k' > i$ with $\tr[k] \models \delta$ and $\tr[k'] \models \delta$, $\tr[k] \models \delta_j$ iff $\tr[k'] \models \delta_j$.
	\end{itemize}
	
	\textbf{Claim A:}
	Let $\pi$ be a path variable with $\Pi(\pi) = \tr$, $\Delta(\pi) = \delta$ and $\Gamma(\pi) = \gamma$ as well as $i$ be a position of type a) or b) on $\pi$.
	Then $\Succ_\delta(\tr,i) = \Succ_\gamma(\tr,i)$.
	
	\textbf{Proof of Claim A:} If $i$ is a position of type a) on $\pi$, we distinguish two cases based on how many positions $k > i$ with $\tr[k] \models \delta$ there are.
	If there are no such positions, then clearly $\Succ_\delta(\tr,i) = i + 1$.
	Since the valuation of $\gamma_0$ is false on all positions after $i$, we have $\Succ_\gamma(\tr,i) = i + 1$ as well in this case.
	If there are such positions, then $\Succ_\delta(\tr,i) = \textit{min}\{ k > i \mid \tr[k] \models \delta \}$ by definition.
	We argue that $\Succ_\gamma(\tr,i) = \textit{min}\{ k > i \mid \tr[k] \models \delta \}$ as well in this case:
	If $\tr[i] \models \gamma_0$, then there are an odd number of $\delta$-positions after position $i$.
	For all $i < l < \textit{min}\{ k > i \mid \tr[k] \models \delta \}$, there are also an odd number of $\delta$-positions after $l$, thus $\tr[l] \models \gamma_0$ as well.
	For $\textit{min}\{ k > i \mid \tr[k] \models \delta \}$ on the other hand, there are an even number of $\delta$-positions and thus $\tr[\textit{min}\{ k > i \mid \tr[k] \models \delta \}] \not\models \gamma_0$.
	Analogously, if $\tr[i] \not\models \gamma_0$ then $\tr[l] \not\models \gamma_0$ for all $i < l < \textit{min}\{ k > i \mid \tr[k] \models \delta \}$ and $\tr[\textit{min}\{ k > i \mid \tr[k] \models \delta \}] \models \gamma_0$.
	Thus, $\Succ_\gamma(\tr,i) = \textit{min}\{ k > i \mid \tr[k] \models \delta \}$.
	
	If $i$ is a position of type b) on $\pi$, we again have $\Succ_\delta(\tr,i) = \textit{min}\{ k > i \mid \tr[k] \models \delta \}$.
	We choose $k$ and $l$ as the minimal positions greater than $i$ such that $\tr[k] \models \delta \land \delta_j$ and $\tr[l] \models \delta \land \lnot \delta_j$.
	Since $k = l$ is impossible, we distinguish two cases, $k < l$ and $k > l$.
	We start with the case $k < l$ where there is a positive number of $\delta \land \delta_j$ positions between $i$ and $l$.
	If $\tr[i] \models \gamma_j$, then this number is even.
	For all $i < k' < \textit{min}\{ k > i \mid \tr[k] \models \delta \}$, the number of $\delta \land \delta_j$ positions between $k'$ and $l$ is even as well since $\tr[k'] \not\models \delta$ for all such $k'$.
	Thus $\tr[k'] \models \gamma_j$.
	On the other hand, the number of $\delta \land \delta_j$ positions between $\textit{min}\{ k > i \mid \tr[k] \models \delta \}$ and $l$ is odd since $\tr[\textit{min}\{ k > i \mid \tr[k] \models \delta \}] \models \delta \land \delta_j$.
	Thus $\tr[\textit{min}\{ k > i \mid \tr[k] \models \delta \}] \not\models \gamma_j$.
	Analogously, if $\tr[i] \not\models \gamma_j$, then $\tr[m] \not\models \gamma_j$ for all $i < m < \textit{min}\{ k > i \mid \tr[k] \models \delta \}$ and $\tr[\textit{min}\{ k > i \mid \tr[k] \models \delta \}] \models \gamma_j$.
	We conclude $\Succ_\gamma(\tr,i) = \textit{min}\{ k > i \mid \tr[k] \models \delta \}$
	The other case, $k > l$, is analogous to the case $k < l$ with the roles of $\gamma_j$ and $\tilde{\gamma}_j$ switched.
	This concludes the proof of Claim A. \hfill$\square$
	
	\textbf{Claim B:}
	Let $\pi$ be a path variable with $\Pi(\pi) = \tr$ and $\Gamma(\pi) = \gamma$ as well as $i$ be a position of type c) on $\pi$.
	Then $\Succ_\gamma(\tr,i) = i + 1$.
	
	\textbf{Proof of Claim B:}
	The valuation of $\gamma_0$ is false on all positions of a trace with positions of type c).
	We show that the valuation of $\gamma_j$ and $\tilde{\gamma}_j$ is also constant for all $j \in \{1,\dots,m\}$ and positions $k \geq i$.
	Fix an arbitrary $j \in \{1,\dots,m\}$.
	We distinguish two cases based on whether all positions $k' > i$ with $\tr[k'] \models \delta$ satisfy $\gamma_j$ or all positions $k' > i$ with $\tr[k'] \models \delta$ satisfy $\lnot \gamma_j$.
	Consider the case where for all $k' > i$ with $\tr[k'] \models \delta$, we have $\tr[k'] \models \delta_j$.
	We argue that $\tr[k] \not\models \gamma_j$ and $\tr[k] \models \tilde{\gamma}_j$ for all $k \geq i$.
	For $\gamma_j$, this is due to the fact that the base case of the fixpoint formula is not satisfied for any position on the subtrace $\tr[k]$.
	For $\tilde{\gamma}_j$, this is due to the fact that $k$ is $0$ positions (i.e. an even number of positions) satisfying $\lnot\delta_j \land \delta$ away from the next position satisfying $\delta_j \land \delta$ since there are no such positions on $\tr[k]$. 
	The other case is analogous with the roles of $\gamma_j$ and $\tilde{\gamma}_j$ switched.
	\hfill$\square$

	For the next claim and the proof of the main claim, we introduce additional notations.
	The first notations are $v_\pi$ and $v[\pi:k]$ for vectors $v \in \mathbb{N}_0^n$, path variables $\pi$ and indices $k$.
	$v_\pi$ represents the entry belonging to $\pi$ in $v$ and
	$v[\pi:k]$ is obtained from the vector $v$ by substituting the entry belonging to $\pi$ by $k$.
	Formally, if $\pi = \pi_m$ and $v = (v_1,\dots,v_n)$, then $v_\pi = v_m$ and $v[\pi:k] = (v_1,\dots,v_{m-1},k,v_{m+1},\dots,v_n)$.
	Next, for a set $S \subseteq \mathbb{N}_0^n$ of vectors, we say that \textit{$S$ is invariant under type c) substitutions} if and only if for for all vectors $v \in \mathbb{N}_0^n$, trace variables $\pi$ and non minimal type c) positions $k,k'$ on $\pi$, if they exist, we have $v[\pi:k] \in S$ iff $v[\pi:k'] \in S$.
	Additionally, for three sets $S,S',S'' \subseteq \mathbb{N}_0^n$ of vectors, we say that \textit{$S$ and $S'$ are equivalent on $S''$} if and only if for all $v \in S''$, $v \in S$ iff $v \in S'$ (or in other words $S \cap S'' = S' \cap S''$).

	\textbf{Claim C:}
	Let $\mathcal{W}$ be a fixpoint variable assignment such that for all fixpoint variables $X$, $\mathcal{W}(X)$ is invariant under type c) substitutions.
	Then, $\llbracket \hat{\psi} \rrbracket^\Pi_\mathcal{W}$ is invariant under type c) substitutions.
	
	\textbf{Proof of Claim C:}
	The proof of this claim is by induction on the structure of $\psi$.
	
	\textit{Case} $\psi = [\delta_j]_{\pi'}$: 
	Let $v \in \mathbb{N}_0^n$ be a vector, $\pi$ be a trace variable with $\delta = \Delta(\pi)$ and $k,k'$ be non minimal positions of type c) on $\pi$.
	For $\pi' \neq \pi$, the claim is trivial, we thus assume $\pi' = \pi$ from here.
	Since the evaluation of the test is independent of all positions other than $v_\pi$, we need to show that $\Pi(\pi)[k] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$ iff $\Pi(\pi)[k'] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$.
	For this, let $k'' \geq k$ and $k''' \geq k'$ be the minimal positions such that $\Pi(\pi)[k''] \models \delta$ and $\Pi(\pi)[k'''] \models \delta$.
	Then $\Pi(\pi)[k] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$ iff $\Pi(\pi)(k'') \models \delta_j$ iff $\Pi(\pi)(k''') \models \delta_j$ iff $\Pi(\pi)[k'] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$.
	Here, the first and third equivalence are due the semantics of the until formula (and the fact that $\lnot \mathcal{F} \delta$ is false in type c) positions) and the second equivalence is due to the fact that $k''$ and $k'''$ are both $\delta$-positions that are greater than the minimal position of type c) on $\pi$ and thus have the same valuation on $\delta_j$.

	\textit{Case} $\psi = \lnot [\delta_j]_{\pi'}$:
	Analogous to the previous case.
	
	\textit{Case} $\psi = X$:
	Follows immediately from the assumption on $\mathcal{W}$.
	
	\textit{Case} $\psi = \psi_1 \lor \psi_2$:
	Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \psi_1 \land \psi_2$:
	Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \bigcirc^\Delta \psi_1$:
	Let $v \in \mathbb{N}_0^n$ be a vector, $\pi$ be a trace variable and $k,k'$ be non minimal positions of type c) on $\pi$.
	
	On the one hand, let $v[\pi : k] \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	By the definition of the semantics, we get $\Succ_\Gamma(\Pi,v[\pi : k]) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	By Claim B, we know that $(\Succ_\Gamma(\Pi,v[\pi : k]))_\pi = k + 1$ and thus $\Succ_\Gamma(\Pi,v)[\pi : k + 1] = \Succ_\Gamma(\Pi,v[\pi : k]) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	Since successors of type c) positions are also type c) positions, $k + 1$ is a non minimal position of type c) on $\pi$ as well.
	By the same argument, $k' + 1$ is a non minimal position of type c) on $\pi$ and the induction hypothesis yields $\Succ_\Gamma(\Pi,v)[\pi : k' + 1] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	Again, by Claim B, we have $(\Succ_\Gamma(\Pi,v)[\pi : k' + 1])_\pi = k' + 1 = (\Succ_\Gamma(\Pi,v[\pi : k']))_\pi$, thus $\Succ_\Gamma(\Pi,v[\pi : k']) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	Finally, using the semantics definition, we get $v[\pi:k'] \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	The other direction is analogous.
		
	\textit{Case} $\psi = \mu X. \psi_1$: 
	For least fixpoints, the approximant characterisation from \cref{app:fixpoints} is used, i.e. $\llbracket \mu X. \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W} = \bigcup_{\kappa \geq 0} \alpha^\kappa(\emptyset)$ for $\alpha$ defined as $\alpha(V) = \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}[X \mapsto V]}$.
	We show by transfinite induction, that for all ordinals $\kappa \geq 0$, $\alpha^\kappa(\emptyset)$ is invariant under type c) substitutions.
	In this induction's base case, $\alpha^0(\emptyset)$ is empty and thus satisfies the claim.
	In the case for successors, the induction hypothesis from the transfinite induction yields that $\alpha^\kappa(\emptyset)$ is invariant under type c) substitutions which, together with the fact that $\mathcal{W}(Y)$ is invariant under type c) substitutions for all fixpoint variables $Y$, means that $\mathcal{W}[X \mapsto \alpha^\kappa(\emptyset)]$ is invariant under type c) substitutions.
	Thus, the induction hypothesis from the structural induction is applicable and yields the claim for $\alpha^{\kappa + 1}(\emptyset)$.
	The case for limit ordinals is a straightforward application of the induction hypothesis of the transfinite induction.
	
	\textit{Case} $\psi = \nu X. \psi_1$: Analogous to the previous case.
	\hfill$\square$
		
	We now proceed with the \textbf{proof of the Main Claim}.
	
	In the \textbf{base case of the main proof}, let $\mathcal{T}$ be an arbitrary set of traces and $\Pi$ be an arbitrary trace assignment over $\mathcal{T}$.
	We prove a result implying $(0,\dots,0) \in \llbracket \psi \rrbracket^\Pi$ iff $(0,\dots,0) \in \llbracket \hat{\psi} \rrbracket^\Pi$ and thus $\Pi \models_\mathcal{T} \varphi_0$ iff $\Pi \models_{\mathcal{T}} \hat{\varphi}_0$.
	We formulate this result so that we can show it by induction on the structure of $\psi$.
	
	\textbf{Inductive claim:}
	Let $S = \{ \Succ_\Delta^k(\Pi,(0,\dots,0)) \mid k \in \mathbb{N}_0 \}$.
	Let $\mathcal{W}$, $\mathcal{W}'$ be fixpoint variable assignments such that for all fixpoint variables $X$
	\begin{itemize}
		\item $\mathcal{W}'(X)$ is invariant under type c) substitutions and
		\item $\mathcal{W}(X)$ and $\mathcal{W}'(X)$ are equivalent on $S$.
	\end{itemize}
	Then, $\llbracket \psi \rrbracket^\Pi_\mathcal{W}$ and $\llbracket \hat{\psi} \rrbracket^\Pi_{\mathcal{W}'}$ are equivalent on $S$.
	
	\textbf{Proof of the inductive claim:}
	
	\textit{Case} $\psi = [\delta_j]_\pi$: 
	Let $v \in \{ \Succ_\Delta^k(\Pi,(0,\dots,0)) \mid k \in \mathbb{N}_0 \}$.
	If $v = (0,\dots,0)$, we just need to focus on tests applied to the initial tests.
	As $\hat{\psi} = \psi$ for these positions, this case is trivial.
	
	If $v = \Succ_\Delta^k(\Pi,(0,\dots,0))$ for some $k > 0$, we need to show that $\Pi(\pi)[v_\pi] \models \delta_j$ iff $\Pi(\pi)[v_\pi] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$ since the evaluation of the test is independent of all positions other than $v_\pi$.
	If $\Pi(\pi)[v_\pi] \models \delta$, then the test in $\hat{\psi}$ is equivalent to $(\lnot \delta \mathcal{U} (\delta \land \delta_j))$ which is equivalent to $\delta_j$ and the case is established.
	If $\Pi(\pi)[v_\pi] \not\models \delta$, then we know that there are no future positions on $\pi$ that satisfy $\Delta(\pi)$, i.e. $\delta$, (since $v = \Succ_\Delta^k(\Pi,(0,\dots,0))$) and the test in $\hat{\psi}$ is equivalent to $(\delta_j \land \lnot \mathcal{F} \delta)$ which is equivalent to $\delta_j$ and the case is established as well.
	
	\textit{Case} $\psi = \lnot [\delta_j]_\pi$: Analogous to the previous case.
	
	\textit{Case} $\psi = X$: Follows immediately from the assumptions on $\mathcal{W}$ and $\mathcal{W}'$.
	
	\textit{Case} $\psi = \psi_1 \lor \psi_2$: Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \psi_1 \land \psi_2$: Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \bigcirc^\Delta \psi_1$:
	Let $v \in \{ \Succ_\Delta^k(\Pi,(0,\dots,0)) \mid k \in \mathbb{N}_0 \}$.
	Since $\mathcal{W}'(X)$ is invariant under type c) substitutions for all fixpoint variables $X$, we can apply Claim C and obtain that $\llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ is invariant under type c) substitutions.
	
	On the one hand, assume that $v \in \llbracket \bigcirc^\Delta \psi_1 \rrbracket^\Pi_\mathcal{W}$.
	By the definition of the semantics, we know that $\Succ_\Delta(\Pi,v) \in \llbracket \psi_1 \rrbracket^\Pi_\mathcal{W}$.
	From the induction hypothesis, we know that $\Succ_\Delta(\Pi,v) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ as well.
	For all $\pi$ where $v_\pi$ is a position of type a) or b), we can apply Claim A to obtain $(\Succ_\Delta(\Pi,v))_\pi = (\Succ_\Gamma(\Pi,v))_\pi$.
	For all $\pi$ where $v_\pi$ is a position of type c), $(\Succ_\Delta(\Pi,v))_\pi$ and $(\Succ_\Gamma(\Pi,v))_\pi$ are non minimal positions of type c) on $\pi$.
	Since $\llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ is invariant under type c) substitutions, we obtain that $\Succ_\Gamma(\Pi,v) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ in both cases.	
	Using the semantics definition, we conclude $v \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$.
	
	On the other hand, assume that $v \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$.
	By the definition of the semantics, we know that $\Succ_\Gamma(\Pi,v) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$.
	For all $\pi$ where $v_\pi$ is a position of type a) or b), we can apply Claim A to obtain $(\Succ_\Gamma(\Pi,v))_\pi = (\Succ_\Delta(\Pi,v))_\pi$.
	For all $\pi$ where $v_\pi$ is a position of type c), $(\Succ_\Gamma(\Pi,v))_\pi$ and $(\Succ_\Delta(\Pi,v))_\pi$ are non minimal positions of type c) on $\pi$.
	Since $\llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ is invariant under type c) substitutions, we again obtain that $\Succ_\Delta(\Pi,v) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ in both cases.
	From the induction hypothesis, we thus know $\Succ_\Delta(\Pi,v) \in \llbracket \psi_1 \rrbracket^\Pi_\mathcal{W}$ and therefore $v \in \llbracket \bigcirc^\Delta \psi_1 \rrbracket^\Pi_\mathcal{W}$ using the semantics definition.
	
	\textit{Case} $\psi = \mu X. \psi_1$: 
	For least fixpoints, we use the approximant characterisation from \cref{app:fixpoints} where $\llbracket \mu X. \psi_1 \rrbracket^\Pi_\mathcal{W} = \bigcup_{\kappa \geq 0} \alpha^\kappa(\emptyset)$ for $\alpha$ defined as $\alpha(V) = \llbracket \psi_1 \rrbracket^\Pi_{\mathcal{W}[X \mapsto V]}$ and $\llbracket \mu X. \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'} = \bigcup_{\kappa \geq 0} \hat{\alpha}^\kappa(\emptyset)$ for $\hat{\alpha}$ defined as $\hat{\alpha}(V) = \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W'}[X \mapsto V]}$
	We show by transfinite induction, that for all ordinals $\kappa \geq 0$, (i) $\hat{\alpha}(\emptyset)$ is invariant under type c) substitutions and (ii) $\alpha^\kappa(\emptyset)$ and $\hat{\alpha}^\kappa(\emptyset)$ are equivalent on $S$.
	In this induction's base case, $\alpha^0(\emptyset)$ and $\hat{\alpha}^0(\emptyset)$ are both empty and thus satisfy both claims.
	
	In the case for successors, the induction hypothesis from the transfinite induction yields that (1) $\hat{\alpha}^\kappa(\emptyset)$ is invariant under type c) substitutions and (2) $\alpha^\kappa(\emptyset)$ and $\hat{\alpha}^\kappa(\emptyset)$ are equivalent on $S$.
	(1) together with the fact that $\mathcal{W}'(Y)$ is invariant under type c) substitutions for all fixpoint variables $Y$ means that $\mathcal{W}'[X \mapsto \hat{\alpha}^\kappa(\emptyset)](Y)$ is invariant under type c) substitutions for all fixpoint variables $Y$.
	Claim C then establishes that $\llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'[X \mapsto \hat{\alpha}^\kappa(\emptyset)]} = \hat{\alpha}^{\kappa + 1}(\emptyset)$ is invariant under type c) substitutions.
	(2) together with the fact that $\mathcal{W}(Y)$ and $\mathcal{W}'(Y)$ are equivalent on $S$ for all fixpoint variables $Y$ yield that $\mathcal{W}[X \mapsto \alpha^\kappa(\emptyset)](Y)$ and $\mathcal{W}'[X \mapsto \hat{\alpha}^\kappa(\emptyset)](Y)$ are equivalent on $S$ for all fixpoint variables $Y$.
	Since both requirements on $\mathcal{W}[X \mapsto \alpha^\kappa(\emptyset)]$ and $\mathcal{W}'[X \mapsto \hat{\alpha}^\kappa(\emptyset)]$ are fulfilled, the induction hypothesis from the structural induction is applicable and yields that $\llbracket \psi_1 \rrbracket^\Pi_{\mathcal{W}[X \mapsto \alpha^\kappa(\emptyset)]} = \alpha^{\kappa + 1}(\emptyset)$ and $\llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'[X \mapsto \hat{\alpha}^\kappa(\emptyset)]} = \hat{\alpha}^{\kappa + 1}(\emptyset)$ are equivalent on $S$.
	
	The case for limit ordinals is a straightforward application of the induction hypothesis of the transfinite induction.
	
	\textit{Case} $\psi = \nu X. \psi_1$:
	Analogous to the previous case.\hfill$\square$
	
	The \textbf{inductive step of the main proof} is trivial.
\end{proof}


\begin{comment}
	
	For the next claim, we introduce notations $v_\pi$ and $v[\pi:k]$ for vectors $v \in \mathbb{N}_0^n$, path variables $\pi$ and indices $k$.
	$v_\pi$ represents the entry belonging to $\pi$ in $v$ and
	$v[\pi:k]$ is obtained from the vector $v$ by substituting the entry belonging to $\pi$ by $k$.
	Formally, if $\pi = \pi_m$ and $v = (v_1,\dots,v_n)$, then $v_\pi = v_m$ and $v[\pi:k] = (v_1,\dots,v_{m-1},k,v_{m+1},\dots,v_n)$.
	
	\textbf{Claim C:}
	Let $\mathcal{W}$ be a fixpoint assignment such that for all fixpoint variables $X$, all trace variables $\pi$ and all vectors $v \in \mathbb{N}_0^n$, if $v_\pi$ is a non minimal position of type c) on $\pi$,
	\begin{itemize}
		\item $v \in \mathcal{W}(X)$ iff $v[\pi:k] \in \mathcal{W}(X)$ for all $k \geq v_\pi$.
	\end{itemize}
	Then for all trace variables $\pi$ and vectors $v \in \mathbb{N}_0^n$, if $v_\pi$ is a non minimal position of type c) on $\pi$,
	\begin{itemize}
		\item $v \in \llbracket \hat{\psi} \rrbracket^\Pi_\mathcal{W}$ iff $v[\pi:k] \in \llbracket \hat{\psi} \rrbracket^\Pi_\mathcal{W}$ for all $k \geq v_\pi$.
	\end{itemize}
	
	\textbf{Proof of Claim C:}
	The proof of this claim is by induction on the structure of $\psi$.
	
	\textit{Case} $\psi = [\delta_j]_{\pi'}$: 
	Let $\pi$ be a trace variable with $\delta = \Delta(\pi)$ and $v \in \mathbb{N}_0^n$ be a vector such that $v_\pi$ is a non minimal position of type c) on $\pi$.
	For $\pi' \neq \pi$, the claim is trivial, we thus assume $\pi' = \pi$ from here.
	Since the evaluation of the test is independent of all positions other than $v_\pi$, we need to show that $\Pi(\pi)[v_\pi] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$ iff $\Pi(\pi)[k] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$ for all $k \geq v_\pi$.
	For this, let $k \geq v_\pi$ be an arbitrary index and let $k' \geq k$ be the minimal position such that $\Pi(\pi)[k'] \models \delta$.
	Additionally, let $k'' \geq v_\pi$ be the minimal position such that $\Pi(\pi)[k''] \models \delta$.
	Then $\Pi(\pi)[v_\pi] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$ iff $\Pi(\pi)(k'') \models \delta_j$ iff $\Pi(\pi)(k') \models \delta_j$ iff $\Pi(\pi)[k] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$.
	Here, the first and third equivalence are due the semantics of the until formula (and the fact that $\lnot \mathcal{F} \delta$ is false in type c) positions) and the second equivalence is due to the fact that $k'$ and $k''$ are both $\delta$-positions that are greater than the minimal position of type c) on $\pi$ and thus have the same valuation on $\delta_j$.
	
	\textit{Case} $\psi = \lnot [\delta_j]_{\pi'}$:
	Analogous to the previous case.
	
	\textit{Case} $\psi = X$:
	Follows immediately from the assumption on $\mathcal{W}$.
	
	\textit{Case} $\psi = \psi_1 \lor \psi_2$:
	Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \psi_1 \land \psi_2$:
	Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \bigcirc^\Delta \psi_1$:
	Let $\pi$ be a trace variable and $v \in \mathbb{N}_0^n$ be a vector such that $v_\pi$ is a non minimal position of type c) on $\pi$.
	
	On the one hand, let $v \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	By the definition of the semantics, we get $\Succ_\Gamma(\Pi,v) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	Since successors of type c) positions are also type c) positions, we know that $(\Succ_\Gamma(\Pi,v))_\pi$ is a non minimal position of type c) on $\pi$ and the induction hypothesis is applicable, yielding $\Succ_\Gamma(\Pi,v)[\pi:k] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$ for all $k \geq (\Succ_\Gamma(\Pi,v))_\pi$.
	By Claim B, we know that $(\Succ_\Gamma(\Pi,v))_\pi = v_\pi + 1$ and thus $\Succ_\Gamma(\Pi,v)[\pi:k] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$ for all $k \geq v_\pi + 1$.
	Again using Claim B yields the following equivalence:
	\begin{align*}
		&\{ \Succ_\Gamma(\Pi,v)[\pi:k] \mid k \geq v_\pi + 1 \} \\
		= &\{ \Succ_\Gamma(\Pi,v)[\pi:k'+1] \mid k' \geq v_\pi \} \\
		= &\{ \Succ_\Gamma(\Pi,v[\pi:k']) \mid k' \geq v_\pi \},
	\end{align*}
	which lets us deduce $\Succ_\Gamma(\Pi,v[\pi:k]) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$ for all $k \geq v_\pi$.
	Finally, using the semantics definition, we get $v[\pi:k] \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$ for all $k \geq v_\pi$.
	
	On the other hand, let $v[\pi:k] \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$ for all $k \geq v_\pi$.
	By choosing $k = v_\pi$, we immediately obtain $v[\pi:v_\pi] = v \in \llbracket \bigcirc^\Gamma \hat{\psi}_1 \rrbracket^\Pi_\mathcal{W}$.
	
	\textit{Case} $\psi = \mu X. \psi_1$: 
	\tbd{Explicit definition of alpha}
	For least fixpoints, the approximant characterisation from \cref{app:fixpoints} is used and we show by transfinite induction, that for all ordinals $\kappa \geq 0$, $v \in \alpha^\kappa(\emptyset)$ iff $v[\pi:k] \in \alpha^\kappa(\emptyset)$ for all $k \geq v_\pi$.
	In this induction's base case, $\alpha^0(\emptyset)$ is empty and thus satisfies the claim.
	In the case for successors, the induction hypothesis from the transfinite induction yields a set $\alpha^\kappa(\emptyset)$ satisfying the equivalence which means that $\mathcal{W}[X \mapsto \alpha^\kappa(\emptyset)]$ satisfies the assumption on fixpoint variable assignments.
	Thus, the induction hypothesis from the structural induction is applicable and yields the claim for $\alpha^{\kappa + 1}(\emptyset)$.
	The case for limit ordinals is a straightforward application of the induction hypothesis of the transfinite induction.
	
	\textit{Case} $\psi = \nu X. \psi_1$: Analogous to the previous case.
	\hfill$\square$
	
	\tbd{
		Use this Claim or characterisation of type c) positions directly?
		
		\textbf{Claim X:}
		Let $\pi$ be a path variable with $\Pi(\pi) = \tr$, $\Delta(\pi) = \delta$ and $\Gamma(\pi) = \gamma$ as well as $i_\pi$ be a minimal position of type c) on $\pi$.
		Additionally, let $k,k' > i_\pi$ be positions with $\tr[k] \models \delta$ and $\tr[k'] \models \delta$.
		Then $\tr[k] \models \delta_j$ iff $\tr[k'] \models \delta_j$ for all $j \in \{1,\dots,m\}$.
		
		\textbf{Proof of Claim X:}
		Follows directly from the characterisation of positions of type c). \hfill$\square$
	}
	
	
	We now proceed with the \textbf{proof of the Main Claim}.
	
	In the \textbf{base case of the main proof}, let $\mathcal{T}$ be an arbitrary set of traces and $\Pi$ be an arbitrary trace assignment over $\mathcal{T}$.
	We prove a result implying $(0,\dots,0) \in \llbracket \psi \rrbracket^\Pi$ iff $(0,\dots,0) \in \llbracket \hat{\psi} \rrbracket^\Pi$ and thus $\Pi \models_\mathcal{T} \varphi_0$ iff $\Pi \models_{\mathcal{T}} \hat{\varphi}_0$.
	We formulate this result so that we can show it by induction on the structure of $\psi$.
	
	For This claim, we introduce some additional notation.
	We use $i_\pi$ for the minimal type c) position on $\pi$, if it exists.
	Furthermore, we group the trace variables $\{\pi_1,\dots,\pi_n\}$ into three categories with respect to $v$.
	We write $\mathit{TypeAB}(v) \subseteq \{\pi_1,\dots,\pi_n\}$ for the set of trace variables $\pi$ such that $v_\pi$ is a position of type a) or b) on $\pi$.
	Next, we write $\mathit{TypeC}(v) \subseteq \{\pi_1,\dots,\pi_n\}$ for the set of trace variables $\pi$ such that $v_\pi$ is a position of type c) on $\pi$ and $v_\pi > i_\pi$.
	Finally, we write $\mathit{FirstTypeC}(v) \subseteq \{\pi_1,\dots,\pi_n\}$ for the set of trace variables $\pi$ such that $v_\pi$ is a position of type c) on $\pi$ and $v_\pi = i_\pi$.
	
	\textbf{Inductive claim:}
	Let $\mathcal{W}$, $\mathcal{W}'$ be fixpoint variable assignments such that for all fixpoint variables $X$ and vectors $v \in \{ \Succ_\Delta^k(\Pi,(0,\dots,0)) \mid k \in \mathbb{N}_0 \}$  with $\mathit{TypeC}(v) = \{\pi_c^1,\dots,\pi_c^l\}$:
	\begin{itemize}
		\item $v \in \mathcal{W}(X)$ iff $v[\pi_c^1:k_1]\dots[\pi_c^l:k_l] \in \mathcal{W}'(X)$ for all $k_1 \geq v_{\pi_c^1},\dots,k_l \geq v_{\pi_c^l}$.
	\end{itemize}
	Then, for all vectors $v \in \{ \Succ_\Delta^k(\Pi,(0,\dots,0)) \mid k \in \mathbb{N}_0 \}$  with $\mathit{TypeC}(v) = \{\pi_c^1,\dots,\pi_c^l\}$:
	\begin{itemize}
		\item $v \in \llbracket \psi \rrbracket^\Pi_\mathcal{W}$ iff $v[\pi_c^1:k_1]\dots[\pi_c^l:k_l] \in \llbracket \hat{\psi} \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_l \geq v_{\pi_c^l}$.
	\end{itemize}
	
	As mentioned, the proof is by induction on the structure of $\psi$.
	
	\textit{Case} $\psi = [\delta_j]_\pi$: 
	If $v = (0,\dots,0)$, we just need to focus on tests applied to the initial tests.
	As $\hat{\psi} = \psi$ for these positions and $\mathit{TypeC}((0,\dots,0)) = \emptyset$, this case is trivial.
	If $v = \Succ_\Delta^k(\Pi,(0,\dots,0))$ for some $k > 0$, we discriminate whether $\pi \in \mathit{TypeC}(v)$ or not.
	In case $\pi \in \mathit{TypeC}(v)$, the claim is established by applying Claim C to $\pi$ and for the rest of the trace variables, the semantics is independent of the entries belonging to those trace variables.
	Next, we consider the case where $\pi \not\in \mathit{TypeC}(v)$.
	Since the evaluation of the test is independent of all positions other than $v_\pi$, we just need to show that $\Pi(\pi)[v_\pi] \models \delta_j$ iff $\Pi(\pi)[v_\pi] \models (\lnot \delta \mathcal{U} (\delta \land \delta_j)) \lor (\delta_j \land \lnot \mathcal{F} \delta)$.
	If $\Pi(\pi)[v_\pi] \models \Delta(\pi)$, then the test in $\hat{\psi}$ is equivalent to $(\lnot \delta \mathcal{U} (\delta \land \delta_j))$ which is equivalent to $\delta_j$ and the case is established.
	If $\Pi(\pi)[v_\pi] \not\models \Delta(\pi)$, then we know that there are no future positions on $\pi$ that satisfy $\Delta(\pi)$ (since $v = \Succ_\Delta^k(\Pi,(0,\dots,0))$) and the test in $\hat{\psi}$ is equivalent to $(\delta_j \land \lnot \mathcal{F} \delta)$ which is equivalent to $\delta_j$ and the case is established as well.
	
	\textit{Case} $\psi = \lnot [\delta_j]_\pi$: Analogous to the previous case.
	
	\textit{Case} $\psi = X$: Follows immediately from the assumption on $\mathcal{W}$ and $\mathcal{W}'$.
	
	\textit{Case} $\psi = \psi_1 \lor \psi_2$: Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \psi_1 \land \psi_2$: Follows immediately from the induction hypothesis.
	
	\textit{Case} $\psi = \bigcirc^\Delta \psi_1$:
	By the definition of type c) positions, we know that $\mathit{TypeC}(\Succ_\Delta(\Pi,v)) = \mathit{TypeC}(v) \cup \mathit{FirstTypeC}(v)$.
	W.l.o.g., we assume that $\mathit{TypeC}(v) = \{\pi_c^1,\dots,\pi_c^l\}$ and $\mathit{TypeC}(\Succ_\Delta(\Pi,v)) = \{\pi_c^1,\dots,\pi_c^{l'}\}$ for $l' \geq l$.
	
	For the first direction, assume that $v \in \llbracket \bigcirc^\Delta \psi_1 \rrbracket^\Pi_\mathcal{W}$.
	By the definition of the semantics, we know that $\Succ_\Delta(\Pi,v) \in \llbracket \psi_1 \rrbracket^\Pi_\mathcal{W}$.
	Applying the induction hypothesis, we obtain $\Succ_\Delta(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l'}:k_{l'}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq (\Succ_\Delta(\Pi,v))_{\pi_c^1},\dots,k_{l'} \geq (\Succ_\Delta(\Pi,v))_{\pi_c^{l'}}$.
	Using Claim B, this can be reformulated as $\Succ_\Delta(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l'}:k_{l'}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1} + 1,\dots,k_{l'} \geq v_{\pi_c^{l'}} + 1$.
	On the one hand, for all $\pi \in \mathit{TypeAB}(v)$, we know that $(\Succ_\Delta(\pi,v))_\pi = (\Succ_\Gamma(\Pi,v))_\pi$ by using Claim A.
	On the other hand, for all $\pi \in \mathit{TypeC}(v) \cup \mathit{FirstTypeC}(v)$, we know that $(\Succ_\Delta(\Pi,v))_\pi \geq v_\pi + 1$, meaning that these entries are exchangeable.
	We thus know $\Succ_\Gamma(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l'}:k_{l'}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1} + 1,\dots,k_{l'} \geq v_{\pi_c^{l'}} + 1$.
	In particular, we have $\Succ_\Gamma(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1} + 1,\dots,k_{l} \geq v_{\pi_c^{l}} + 1$ by instantiating $k_{l+1}, \dots,k_{l'}$ with $v_{\pi_c^{l+1}} + 1,\dots,v_{\pi_c^{l'}} + 1$, respectively.
	From the equivalence
	\begin{align*}
		&\{ \Succ_\Gamma(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}] \mid k_1 \geq v_{\pi_c^1} + 1,\dots,k_{l} \geq v_{\pi_c^{l}} + 1 \} \\
		= &\{ \Succ_\Gamma(\Pi,v)[\pi_c^1:k_1' + 1]\dots[\pi_c^{l}:k_{l}' + 1] \mid k_1' \geq v_{\pi_c^1},\dots,k_{l}' \geq v_{\pi_c^{l}} \} \\
		= &\{ \Succ_\Gamma(\Pi,v[\pi_c^1:k_1']\dots[\pi_c^{l}:k_{l}']) \mid k' \mid k_1' \geq v_{\pi_c^1},\dots,k_{l}' \geq v_{\pi_c^{l}} \},
	\end{align*}
	we further deduce $\Succ_\Gamma(\Pi,v[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}]) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_{l} \geq v_{\pi_c^{l}}$.
	Using the semantics definition, we conclude $v[\pi_c^1:k_1]\dots[\pi_c^l:k_l] \in \llbracket \hat{\psi} \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_l \geq v_{\pi_c^l}$.
	
	For the other direction, assume that $v[\pi_c^1:k_1]\dots[\pi_c^l:k_l] \in \llbracket \hat{\psi} \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_l \geq v_{\pi_c^l}$.
	By the semantics definition, we know that $\Succ_\Gamma(\Pi,v[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}]) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq (\Succ_\Gamma(\Pi,v[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}]))_{\pi_c^1},\dots,k_{l} \geq (\Succ_\Gamma(\Pi,v[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}]))_{\pi_c^{l}}$.
	We reformulate this by using Claim B:
	$\Succ_\Gamma(\Pi,v[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}]) \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1} + 1,\dots,k_{l} \geq v_{\pi_c^{l}} + 1$.
	Using the equivalence
	\begin{align*}
		&\{ \Succ_\Gamma(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}] \mid k_1 \geq v_{\pi_c^1} + 1,\dots,k_{l} \geq v_{\pi_c^{l}} + 1 \} \\
		= &\{ \Succ_\Gamma(\Pi,v)[\pi_c^1:k_1' + 1]\dots[\pi_c^{l}:k_{l}' + 1] \mid k_1' \geq v_{\pi_c^1},\dots,k_{l}' \geq v_{\pi_c^{l}} \} \\
		= &\{ \Succ_\Gamma(\Pi,v[\pi_c^1:k_1']\dots[\pi_c^{l}:k_{l}']) \mid k' \mid k_1' \geq v_{\pi_c^1},\dots,k_{l}' \geq v_{\pi_c^{l}} \},
	\end{align*}
	from the previous direction the other way around, we can deduce that $\Succ_\Gamma(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l}:k_{l}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_{l} \geq v_{\pi_c^{l}}$.
	We can now use Claim C for all trace variables $\pi \in \mathit{FirstTypeC}(v)$ to obtain $\Succ_\Gamma(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l'}:k_{l'}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_{l'} \geq v_{\pi_c^{l'}}$.
	Again, as in the previous direction, we know that on the one hand, for all $\pi \in \mathit{TypeAB}(v)$, we have $(\Succ_\Delta(\pi,v))_\pi = (\Succ_\Gamma(\Pi,v))_\pi$ by using Claim A.
	On the other hand, for all $\pi \in \mathit{TypeC}(v) \cup \mathit{FirstTypeC}(v)$, we know that $(\Succ_\Delta(\pi,v))_\pi \geq v_\pi + 1$, meaning that these entries are exchangeable.
	Thus, $\Succ_\Delta(\Pi,v)[\pi_c^1:k_1]\dots[\pi_c^{l'}:k_{l'}] \in \llbracket \hat{\psi}_1 \rrbracket^\Pi_{\mathcal{W}'}$ for all $k_1 \geq v_{\pi_c^1},\dots,k_{l'} \geq v_{\pi_c^{l'}}$.
	Applying the induction hypothesis, we know that $\Succ_\Delta(\Pi,v) \in \llbracket \psi_1 \rrbracket^\Pi_\mathcal{W}$.
	Using the semantics definition, we conclude $v \in \llbracket \bigcirc^\Delta \psi_1 \rrbracket^\Pi_\mathcal{W}$.
	
	\textit{Case} $\psi = \mu X. \psi_1$: 
	The case for least fixpoints is analogous to the least fixpoint case in the proof of Claim C.
	
	\textit{Case} $\psi = \nu X. \psi_1$:
	Analogous to the previous case.
	
	The \textbf{inductive step of the main proof} is trivial.
\end{comment}

==> math/proofs/synchronousconnection.tex <==
\begin{proof}(of \cref{lem:synchronousconnection})
	The proof is by induction on the structure of $\psi$.
	
	\textbf{Case 1:} $\psi = [\delta]_{\pi}$.
	Follows straightforwardly from the definition of $\Pi^\Delta$.
	
	\textbf{Case 2:} $\psi = \lnot [\delta]_{\pi}$.
	Analogous to case 1.
	
	\textbf{Case 3:} $\psi = [X]_{\pi}$.
	Follows from the assumption on $\mathcal{W}$ and $\mathcal{W}'$.
	
	\textbf{Case 4:} $\psi = \psi_1 \lor \psi_2$.
	Follows directly from the induction hypothesis.
	
	\textbf{Case 5:} $\psi = \psi_1 \land \psi_2$.
	Analogous to case 4.
	
	\textbf{Case 6:} $\psi = \bigcirc^\Delta \psi_1$.
	For arbitrary $i$, the claim follows from the fact that the induction hypothesis establishes the claim for $i+1$.
	
	\textbf{Case 7:} $\psi = \mu X. \psi_1$.
	We use the fixpoint approximant characterisation of $\psi^s$ and $\psi$ and write $\llbracket \psi^s \rrbracket_{\mathcal{W}}^{\Pi^\Delta}$ as $\bigcup_{\kappa \geq 0} \alpha_s^\kappa(\emptyset)$ for $\alpha_s$ with $\alpha_s(V) = \llbracket \psi_1^s \rrbracket_{\mathcal{W}[X \mapsto V]}^{\Pi^\Delta}$ and $\llbracket \psi \rrbracket_{\mathcal{W}'}^{\Pi}$ as $\bigcup_{\kappa \geq 0} \alpha^\kappa(\emptyset)$ for $\alpha$ with $\alpha(V) = \llbracket \psi_1 \rrbracket_{\mathcal{W}'[X \mapsto V]}^\Pi$.
	We then show by transfinite induction over $\kappa$, that $(i,\dots,i) \in \alpha_s^\kappa(\emptyset)$ iff $\Succ_{\Delta}^i(\Pi,(0,\dots,0)) \in \alpha^\kappa(\emptyset)$.
	To avoid confusion, we will write (SIH) for the induction hypothesis of the structural induction and (TIH) for the induction hypothesis of the transfinite induction.
	The \textit{base case} $\kappa = 0$ follows directly from (SIH) if we can establish that the assumption from the lemma holds for $\mathcal{W}[X \mapsto \emptyset]$ and $\mathcal{W}'[X \mapsto \emptyset]$.
	For all $X' \neq X$, the assumption follows from the fact that it holds for $\mathcal{W}$ and $\mathcal{W}'$.
	For $X' = X$, the assumption follows from the fact that $X$ is mapped to $\emptyset$ in both vector fixpoint variable assignments.
	In the inductive step $\kappa \mapsto \kappa + 1$, we use (TIH) to establish that the claim holds for $\kappa$.
	Thus, the lemma's assumption holds for $\mathcal{W}[X \mapsto \alpha_s^\kappa(\emptyset)]$ and $\mathcal{W}'[X \mapsto \alpha^\kappa(\emptyset)]$ and we can use (SIH) to establish the claim for $\kappa + 1$.
	Finally, the \textit{limit case} $\kappa < \lambda \mapsto \lambda$ follows directly from (TIH).
	
	\textbf{Case 8:} $\psi = \nu X. \psi_1$.
	Analogous to case 7.
\end{proof}
\begin{comment}
\tbd{Maybe for this to be proven easily, we need to change the semantics from $\llbracket \psi \rrbracket^{\Pi}_{\mathcal{W}} = \dots$ to $\llbracket \psi \rrbracket_{\mathcal{W}} : \Pi \mapsto \dots$.
Then, a restriction of the lemma to restricted predicate valuations could be used to prove the claim for $\psi = X$.
We need $\llbracket X \rrbracket_\mathcal{W}(\Pi) = \llbracket X \rrbracket_{\mathcal{W}'}(\Pi^\Delta)$, so maybe something like $\Delta$ and $\Pi$-respecting valuations $\mathcal{W}$, $\mathcal{W}'$ where $\Succ_{\Delta}^i((0,\dots,0)) \in \mathcal{W}(\Pi)$ iff $(i,\dots,i) \in \mathcal{W'}(\Pi^\Delta)$.
Do all valuations occuring in fixpoinbt evaluations have this property?}
\end{comment}

==> math/proofs/undecidability.tex <==
\begin{proof}%(of \cref{thm:undecidability})
	Since HyperLTL$_S$ is a subset of stuttering $H_\mu$, we can use \cref{thm:deltagammareduction} to obtain a reduction from HyperLTL$_S$ model checking which was shown to be undecidable in \cite{Bozzelli2021}.
\end{proof}

\begin{comment}
	The proof of this claim is by a reduction from the Post Correspondence Problem.
	Let $I = \{(u_1,v_1),...,(u_n,v_n)\}$ with $u_i,v_i \in \Sigma^*$ be a PCP instance.
	We construct a formula $\varphi_I$ and a Kripke Structure $\mathcal{K}_I$ such that $\mathcal{K}_I \models \varphi_I$ iff $I$ has a solution.
	
	The labelling alphabet of the Kripke Structure contains $\Sigma$, the letters $\{1,...,n\}$, a fresh atomic proposition $p$ and a dummy symbol $\bot$.
	The main idea is to encode a solution of $I$ in two traces $\pi_1$ and $\pi_2$, each being a concatenation of two parts.
	In the first part, we have exactly one letter from $\Sigma$ in each position.
	Additionally, some positions are labelled with $p$ and a symbol $i$ from $\{1,...,n\}$ indicating that a new domino stone starts at this position and the number of that stone is $i$.
	In the second part, we have that all positions are labelled with $\bot$ and $p$.
	We choose the Kripke Structure that generates traces of this structure as $\mathcal{K}_I$.
	
	The formula $\varphi_I$ is given as $\exists \pi_1 . \exists \pi_2 . \psi_{domino} \land \psi_{same}$.
	Intuitively, $\psi_{domino}$ states that the first part of the traces $\pi_1$ and $\pi_2$ encode words in accordance with some concatenation of domino stones and $\psi_{same}$ encodes that the letters in each position are the same.
	The formula $\psi_{domino}$ uses the successor assignment $\Delta$ with $\Delta(\pi_1) = \Delta(\pi_2) = p$ to move from domino stone to domino stone.
	It is given by $\psi_{domino} := \mu X. ([\bot]_{\pi_1} \land [\bot]_{\pi_2}) \lor ((\bigvee_{i = 1}^n [i]_{\pi_1} \land [i]_{\pi_2} \land [\delta_i^1]_{\pi_1} \land [\delta_i^2]_{\pi_2}) \land \bigcirc^{\Delta} X)$.
	Here $\delta_i^1$ (resp. $\delta_i^2$) are trace formulae that state that the next symbols on the traces concatenated form $u_i$ (resp. $v_i$) and are immediately followed by a position labelled $p$.
	For example, if $v_i = v_i^1 ... v_i^m$, then $\delta_i^1 = (v_i^1 \land \lnot p \land \bigcirc (v_i^2 \land \lnot p \land ... \land \bigcirc  (v_i^m \land \lnot p \land \bigcirc p)...))$.
	The second part of the formula, $\psi_{same}$, uses a successor assignment $\Delta'$ with $\Delta'(\pi_1) = \Delta'(\pi_2) = \true$ to synchronously advance the traces.
	It is given as $\psi_{same} := \nu X. (\bigwedge_{a \in \Sigma \cup \{\bot\}} [a]_{\pi_1} \leftrightarrow [a]_{\pi_2} \land \bigcirc^{\Delta'}X)$.
	
	It is straightforward to see that $\mathcal{K}_I \models \varphi_I$ iff $I$ has a solution.
\end{comment}

==> math/proofs/vpmodelcheckinglemma.tex <==
\begin{proof}%(of \cref{lem:vpmodelcheckinglemma})
	The first claim is shown by a straightforward structural induction on the formulae $\delta \in \cl(B)$ and is very similar to the proof of \cref{thm:synchronousautomaton} which was conducted in \cite{GutsfeldMO21}.
	In the fixpoint case, use the fact that states for least fixpoints and their fixpoint variables can only be visited finitely many times while greatest fixpoints and their fixpoint variables have to be visited infinitely often.
	Thus the language of the automaton starting from these states can be expressed as a least or greatest fixpoint of a function $f \colon \mathcal{L} \mapsto \mathcal{L}(\mathcal{A}_{X:\mathcal{L}})$ where $\mathcal{A}_{X:\mathcal{L}}$ is a variant of the automaton $\mathcal{A}$ that recognizes the language $\mathcal{L}$ when starting from state $X$ instead of having the normal transition behavior in $X$.
	This fixpoint can then be compared to the semantics of the formula using the approximant characterisations.
	
	The second claim can be shown constructively.
	Given a trace $tr$, $w$ is obtained by amending every position $i$ of $tr$ with the set of atomic propositions $\{ at(\delta) \mid i \in \llbracket \delta \rrbracket^{tr}\}$.
\end{proof}

==> math/proofs/vpmodelcheckingreduction.tex <==
\tbd{Size of construction}
\begin{proof}
	Transform a general formula $\varphi$ with successor assignment $\Delta$ and a fair Visibly Pushdown System $(\mathcal{VP},F)$ into $\varphi'$ and $(\mathcal{VP}',F')$ as described before.
	$\varphi'$ has size $\mathcal{O}(|\varphi|)$ and $(\mathcal{VP}',F')$ has size $\mathcal{O}(|\mathcal{VP}| \cdot 2^{|\varphi| \cdot \log(|\varphi|)})$.
	By construction, we have $(\mathcal{VP},F) \models \varphi$ iff $(\mathcal{VP}',F') \models \varphi'$.\qed
\end{proof}

==> math/proofs/vpundecidability.tex <==
\begin{proof}
	It is straightforward to see that with the standard successor operator and the synchronous successor assignment $\Delta_\true$, the logic subsumes HyperLTL.
	Thus, the claim can be shown by a reduction from HyperLTL model checking against pushdown systems which was shown to be undecidable in \cite{Pommellet2018}.
\end{proof}

==> math/shortproofs/alignedprefixlemma.tex <==
\begin{proof}(Sketch)
	By induction on $l$ using the inductive definition of $\psi^j$.
\end{proof}

==> math/shortproofs/alignedsynchronousautomaton.tex <==
\begin{proof}(Sketch)
	The size of the automaton $\mathcal{A}_\psi$ is linear.
	To show the required equivalence for all trace assignments $\Pi$, we discriminate two cases based on $\wapref(\Pi,\Delta)$.
	The first one, where $\wapref(\Pi,\Delta) = \infty$ and $w_{\Pi}^{\Delta}$ does not contain $\top$ symbols, is done by a structural induction on $\psi$.
	In the second one, where $\wapref(\Pi,\Delta) < \infty$ and $w_{\Pi}^{\Delta}$ ends in a $\top$ suffix, we first show the claim for formulae $\psi$ that do not contain fixpoints.
	We then establish a lemma that shows that if $\wapref(\Pi,\Delta) < \infty$, then the semantics of a formula $\psi$ containing fixpoints on $\Pi$ can be characterised by a variant of $\psi$ that unrolls the fixpoints up to $\wapref(\Pi,\Delta)$ times and then removes them.
	The claim for fixpoint-free formulae and the lemma are then used to also show the claim for $\psi$ containing fixpoints.
\end{proof}

==> math/shortproofs/deltaexpressiveness.tex <==
\begin{IEEEproof}(Sketch)
	The main idea is to extend the translation of the formula from the proof of \cref{thm:deltagammareduction}.
	When only one stuttering assignment is used in $\varphi$, the problem with the first position can be addressed directly in the formula $\varphi'$ without changing the structure.
	First, tests to the initial position are not shifted like the other tests.
	A subtle problem arises, if $\Gamma$ advances a trace onto the second position of that trace: In this case, outermost $\bigcirc^{\Delta}$ operators move too far.
	To compensate, such next operators are omitted and tests on traces without this problem are shifted by one $\Delta$-step using a corresponding fixpoint formula in the test.
	%Potential mismatches in progress due to this problem can be identified with tests for the jump criterion and shifting of next operators.
\end{IEEEproof}




\begin{comment}
\tbd{Problem: mismatch if $\Gamma$ advances to the second position
\begin{itemize}
\item Scenario: $\Gamma(\pi)$ changes from the first position on $\pi$ to the second
\item In this scenario $\bigcirc^{\Delta}$ should stand still on $\pi$ for the $[\bigcirc \gamma]_\pi$ test to work properly
\item However, $\bigcirc^{\Delta}$ always advances at least one step and thus skips the first $\bigcirc^{\Gamma}$ position
\item Possible solution: identify this case with $\delta_{\Gamma,\pi}$ and remove the outermost $\bigcirc^{\Delta}$ operator
\item Problem with this solution: the scenario can apply to some paths $\pi$ but not others
\item Possible workarbound: identify exactly the set of paths where this is the case with a combination of $\delta_{\Gamma,\pi}$ formulas, remove the outermost $\bigcirc^{\Delta}$ operator and shift the tests for all paths $\pi$ where $\delta_{\Gamma,\pi}$ does not initially hold by one $\Gamma$ position (replace $[\bigcirc \delta]_\pi$ with $[\bigcirc \mu X. ((\delta_{\Gamma,\pi} \land \bigcirc \delta) \lor (\lnot \delta_{\Gamma,\pi} \land \bigcirc X))]$)
\item Problem with this workaround: exponential blowup
\item Workaround works for formulas from the decidable fragment, i.e. formulas with only a single stuttering assignment, and stays in the decidable fragment, i.e. the translation also only has a single successor assignment
\item Workaround for formulas with different stuttering assignments: replace outermost $\bigcirc^{\Delta}$ with $\bigcirc^{\Delta'}$ where $\Delta'(\pi) = \true$ for all $\pi$ for which $\delta_{\Gamma,\pi}$ holds on the first position
\end{itemize}}
\end{comment}


==> math/shortproofs/deltagammareduction.tex <==
\begin{IEEEproof}(Sketch)
	The main idea of the reduction is to replace stuttering assignments $\Gamma$ by successor assignments $\Delta$ in which each formula $\Delta(\pi)$ expresses that the valuation of some formula $\delta \in \Gamma(\pi)$ changes from this point on the trace $\pi$ to the next, i.e.  $\Delta(\pi) = \bigvee_{\delta \in \Gamma(\pi)} \lnot (\delta \leftrightarrow \bigcirc^g \delta)$.
	Then, tests $[\delta]_{\pi}$ are replaced by $[\bigcirc^g \delta]_{\pi}$ to compensate for the fact that we jump to the positions directly in front of the positions that $\Gamma$ would jump to.
	In order to ensure that we start directly in front of the first position, the system receives a fresh initial state transitioning to the old initial state.
\end{IEEEproof}

==> math/shortproofs/deltastrictexpressiveness.tex <==
\begin{proof}(Sketch)
	The hyperproperty $\mathcal{H}$ is given by the set of all $\mathcal{T} \subseteq (2^\AP)^\omega$ such that for all $tr \in \mathcal{T}$ we have $p \in tr(0)$ and all $tr \in \mathcal{T}$ have the same finite number of positions $i$ with  $p \in tr(i)$.
	In $\Delta$-stuttering $H_\mu$, this can be expressed as $\forall \pi_1 . \forall \pi_2 . [p]_{\pi_1} \land [p]_{\pi_2} \land (([p]_{\pi_1} \land [p]_{\pi_2}) \mathcal{U}^{\Delta} (\lnot[p]_{\pi_1} \land \lnot[p]_{\pi_2}))$ where $\Delta(\pi_1) = \Delta(\pi_2) = p$.
	In order to show that $\Gamma$-stuttering $H_\mu$ with basis $LTL$ cannot express this property, we first inductively define $nd(\delta)$ as the nesting depth of $\bigcirc$ modalities in $\delta$.
	Furthermore, for $n \geq 1$ let $tr_n$ be the trace $\{p\}^n\emptyset^\omega$.
	We then	show by structural induction on $\delta$ that for formulae $\delta \in LTL$ with $nd(\delta) = n$, we have $0 \in \llbracket \delta \rrbracket^{tr_i}$ iff $0 \in \llbracket \delta \rrbracket^{tr_j}$ for all $i,j > n$.
	This can then be used to show by a structural induction, that ($\ast$) for all trace assignments $\Pi$, we have $(0,\dots,0) \in \llbracket \psi \rrbracket^{\Pi[\pi \mapsto tr_i]}$ iff $(0,\dots,0) \in \llbracket \psi \rrbracket^{\Pi[\pi \mapsto tr_j]}$ for all $i,j > \max\{nd(\delta) \mid \delta \in \sub(\psi)\}$.
	Assume now that $\varphi = Q_1 \pi_1  \dots Q_m \pi_m . \psi$ is a formula that expresses the above hyperproperty $\mathcal{H}$.
	Let $n = \max\{nd(\delta) \mid \delta \in \sub(\psi)\}$.
	Then, let $\mathcal{T}_1 = \{t_{n+1}\}$ and $\mathcal{T}_2 = \{t_{n+1},t_{n+2}\}$.
	Clearly, $\mathcal{T}_1 \in \mathcal{H}$ whereas $\mathcal{T}_2 \not\in \mathcal{H}$.
	Hence $\mathcal{T}_1 \models \varphi$ and $\mathcal{T}_2 \not\models \varphi$.
	However, using ($\ast$), it is easy to see that $\mathcal{T}_1 \models \varphi$ implies $\mathcal{T}_2 \models \varphi$, a contradiction.
\end{proof}

==> math/shortproofs/deltastrictexpressivenesslemma1.tex <==
\begin{IEEEproof}(Sketch)
	Let $\Delta$ be the successor assignment with $\Delta(\pi_1) = \Delta(\pi_2) = p$.
	The formula expressing the hyperproperty universally quantifies $\pi_1$ and $\pi_2$ and then uses this successor assignment to synchronously progress over matching $p$ positions.
	We have a disjunction over four cases based on whether $p$ holds in the initial positions of $\pi_1$ and $\pi_2$.
\end{IEEEproof}

==> math/shortproofs/deltatequivalencecorollary.tex <==
\begin{proof}(Sketch)
	The proof uses the following claim which is established by induction:
	
	\textbf{Claim:} For all multitrace formulae $\psi$, indices $i \in \mathbb{N}_0$, trace assignments $\Pi$ and fixpoint variable assignments $\mathcal{W}, \mathcal{W}'$ with $(i,\dots,i) \in \mathcal{W}(X)$ iff $\prog(\Pi,\Delta,i) \in \mathcal{W}'(X)$ for all $X \in \chi_v$, we have
	$(i,\dots,i) \in \llbracket \psi^{s} \rrbracket_{\mathcal{W}}^{\Pi^\Delta}$ iff $\prog(\Pi,\Delta,i) \in \llbracket \psi \rrbracket_{\mathcal{W}'}^{\Pi}$.
	
	With the claim established, we can easily show that $\mathcal{A}_\psi$ is $(\Delta,\mathcal{T})$-equivalent to $\psi$:
	Let $\mathcal{T}$ be an arbitrary set of traces and let $\Pi$ be an arbitrary trace assignment over $\mathcal{T}$.
	Also, let $i \in \mathbb{N}_0$ be an arbitrary index.
	For the first direction, assume that $\prog(\Pi,\Delta,i) \in \llbracket \psi \rrbracket^\Pi$.
	From the claim, we then get $(i,\dots,i) \in \llbracket \psi^s \rrbracket^{\Pi^\Delta}$ since $\mathcal{W}_0$ satisfies the requirement of the claim.
	Then, the $\Img(\Pi^\Delta)$-equivalence of $\mathcal{A}_{\psi^s}$ and $\psi^s$ gives us $w_{\Pi^\Delta}[i] \in \mathcal{L}(\mathcal{A}_{\psi^s})$.
	The other direction is analogous.	
\end{proof}

==> math/shortproofs/gniundecidability.tex <==
\begin{proof}(Sketch)
	The property generalised non-interference is given by the HyperLTL formula
	\begin{align*}
		\varphi_{\mathit{GNI}} := \forall \pi_1 . \forall \pi_2 . \exists \pi_3 . (\mathcal{G} \bigwedge\nolimits_{\ap \in L} \ap_{\pi_1} \leftrightarrow \ap_{\pi_3} )\land (\mathcal{G} \bigwedge\nolimits_{\ap \in H} \ap_{\pi_2} \leftrightarrow \ap_{\pi_3} )
	\end{align*}
	where $L$ encodes a set of low security variables and $H$ encodes a set of high-security variables.
	It states that for all pairs of traces $\pi_1,\pi_2$, there is a third trace $\pi_3$ agreeing with $\pi_1$ on the low-security variables from $L$ and agreeing with $\pi_2$ on the high-security variables from $H$.
	We show that it is undecidable to check $\mathcal{PD} \models \varphi_{\mathit{GNI}}$ for pushdown systems $\mathcal{PD}$ via a reduction from the equivalence problem for pushdown automata.
	
	Let $\mathcal{A}_1$ and $\mathcal{A}_2$ be pushdown automata recognizing languages $\mathcal{L}_1$ and $\mathcal{L}_2$ respectively. 
	We construct a system $\mathcal{PD}$ such that $\mathcal{PD} \models \varphi_{\mathit{GNI}}$ iff $\mathcal{L}_1 = \mathcal{L}_2$.
	Specifically, $\mathcal{PD}$ contains a copy of $\mathcal{A}_1$ and $\mathcal{A}_2$ with a nondeterministic choice to move to either automaton at the start.
	Transition symbols of the automata are encoded in low-security variables $L$ while a high-security bit $b$ (with $H = \{b\}$) indicates whether $\mathcal{PD}$ follows a trace from $\mathcal{A}_1$ or from $\mathcal{A}_2$.
	Both directions of the required equivalence can easily be shown.
\end{proof}


==> math/shortproofs/quantifierkequivalence.tex <==
\begin{proof}(Sketch)
	The part of the claim about the size of $\mathcal{A}_\varphi$ can be seen by inspecting the construction.
	For the inner formula $\psi$, we know that $|\mathcal{A}_\psi|$ is linear in $|\psi|$ for the APA $\mathcal{A}_\psi$ from \cref{thm:deltatequivalence}.
	An alternation removal construction to transform it into an NBA increases the size to exponential in $|\psi|$ by \cref{prop:paritydealternation}.
	Complementation constructions are performed corresponding to every quantifier alternation, each further increasing the size exponentially due to \cref{prop:paritydealternation}.
	%For this, we can interpret an NBA as an APA, complement it without an increase in size, and then transform it into an NBA again with \cref{thm:paritydealternation}.
	Finally, the size measured in $|\mathcal{K}|$ is one exponent smaller since the structure is first introduced into the automaton after the first alternation removal construction.
	
	The part of the claim about $(\Delta,\Traces(\mathcal{K},F))$-equivalence is shown as follows.
	Using the notation $\varphi_i$ with special cases $\varphi_0 = \psi$ and $\varphi_n = \varphi$ from above, we show that $\mathcal{A}_{\varphi_i}$ is $(\Delta,\Traces(\mathcal{K},F))$-equivalent to $\varphi_i$ by induction on $i$.
	The base case follows from \cref{thm:deltatequivalence}.
	In the inductive step, the more interesting case is that where $Q_i$ is an existential quantifier.
	For one direction of the required equivalence, we can simulate the trace witnessing the satisfaction of the quantifier in the state space of the automaton to construct an accepting run.
	For the other direction, we can extract a trace from an accepting run and show that it witnesses the satisfaction of the quantifier.
\end{proof}

==> math/shortproofs/undecidability.tex <==
\begin{proof}(Sketch)
	The proof of this claim is by a reduction from the Post Correspondence Problem.
	The main idea is to have two subformulae $\psi_{\mathit{domino}}$ and $\psi_{\mathit{same}}$ that express that two words encoded in traces $\pi_1$ and $\pi_2$ can be constructed from the PCP domino stones and form the same words respectively.
	$\psi_{\mathit{domino}}$ uses a successor assignment $\Delta$ with $\Delta(\pi_1) = \Delta(\pi_2) = p$ where $p$ marks the start of every domino stone to move from stone to stone.
	$\psi_{\mathit{same}}$ on the other hand uses a successor assignment $\Delta'$ with $\Delta'(\pi_1) = \Delta'(\pi_2) = \true$ to synchronously check if the traces encode the same words.
\end{proof}

==> math/theorems/alignmentlemma.tex <==
\begin{lemma}\label{lem:alignmentlemma}
	Let $\tr_1[v_1,v_1'],...,\tr_n[v_n,v_n']$ be well-aligned subtraces that start on the same stack level. 
	Then there are natural numbers $k,l \in \mathbb{N}_0$ such that for all traces $\tr_i$, the subtrace $\tr_i[v_i,v_i']$ can be progressed as $(\abs^*\ret)^k(\abs^*\call)^l \abs^*$ where $\abs$ stands for an abstract succesor move.
\end{lemma}

==> math/theorems/deltaexpressivenesscor.tex <==
\begin{corollary}
	The decidable fragment of mumbling $H_\mu$ is at least as expressive as the decidable fragment of stuttering $H_\mu$.
\end{corollary}

==> math/theorems/deltaexpressivenesscorollary.tex <==
\begin{corollary}
	$\Delta$-stuttering $H_\mu$ is strictly more expressive than asynchronous HyperLTL from Bozzelli et al.
\end{corollary}

==> math/theorems/gammaexpressiveness.tex <==
\begin{theorem}
	The Model Checking and Satisfiability problem for $\Delta$-stuttering $H_\mu$ can be reduced in linear time to the Model Checking and Satisfiability problem for $\Gamma$-stuttering $H_\mu$.
\end{theorem}

==> math/theorems/ltlclaim.tex <==
\begin{lemma}\label{lem:ltlclaim}
	For all trace formulae $\delta \in LTL$ with $\mathit{nd}(\delta) = n$ and traces $\tr$, we have $\tr[i] \models \delta$ iff $tr[i+1] \models \delta$ if there is a set $P \subseteq \AP$ such that $tr(j) = P$ for all $i \leq j \leq i + n + 1$.
\end{lemma}

==> math/theorems/modelcheckingreduction.tex <==
\begin{corollary}\label{cor:modelcheckingreduction}
	The fair Finite State and fair pushdown model checking problem for mumbling $H_\mu$ can be reduced in exponential time to the fair finite state and fair pushdown model checking problem for mumbling $H_\mu$ with basis $\AP'$ respectively, where $\AP' \supseteq \AP$ is an extended set of atomic propositions.
	%\begin{itemize}
	%	\item The fair Finite State Model Checking Problem for stuttering $H_\mu$ can be reduced in exponential time to the fair Finite State Model Checking Problem for $H_\mu$ with basis $\AP'$ for an extended set of atomic propositions $\AP' \supseteq \AP$.
	%	\item The fair Visibly Pushdown Model Checking Problem for stuttering $H_\mu$ can be reduced in exponential time to the fair Visibly Pushdown Model Checking Problem for $H_\mu$ with basis $\AP'$ for an extended set of atomic propositions $\AP' \supseteq \AP$.
	%\end{itemize}
\end{corollary}

==> math/theorems/mumblingstrictexpressivenesslemma2.tex <==
\begin{lemma}\label{lem:mumblingstrictexpressivenesslemma2}
	$\mathcal{H}$ cannot be expressed in the decidable fragment of stuttering $H_\mu$.
\end{lemma}

==> math/theorems/synchronousconnection.tex <==
\begin{lemma}\label{lem:synchronousconnection}
	For all formulae $\psi$, $i \in \mathbb{N}_0$, trace assignments $\Pi$ and fixpoint variable assignments $\mathcal{W}, \mathcal{W}'$ with $(i,\dots,i) \in \mathcal{W}(X)$ iff $\Succ_{\Delta}^i(\Pi,(0,\dotsm,0)) \in \mathcal{W}'(X)$ for all $X \in \chi_v$, we have
	$(i,\dots,i) \in \llbracket \psi^{s} \rrbracket_{\mathcal{W}}^{\Pi^\Delta}$ iff $\Succ_{\Delta}^i(\Pi,(0,\dotsm,0)) \in \llbracket \psi \rrbracket_{\mathcal{W}'}^{\Pi}$.
\end{lemma}

==> math/theorems/vpmodelcheckinglemma.tex <==
\begin{lemma}\label{lem:vpmodelcheckinglemma}
	Given a set of $VP-\mu TL$ formulae $B$ over $\AP$, one can construct a VPA $\mathcal{A}_{B}$ over the alphabet $2^{\AP_B} \times \{\intern,\call,\ret\}$ with a number of states exponential in $|\AP_{B}|$ satisfying the following conditions:
	\begin{itemize}
		\item[1)] let $w \in \mathcal{L}(\mathcal{A}_B)$: then for all $i \geq 0$ and $\delta \in \cl(B)$, $at(\delta) \in w(i)$ iff $i \in \llbracket \delta \rrbracket^{(w)_\AP}$.
		\item[2)] for each trace $\mathit{tr}$, there exists $w \in \mathcal{L}(\mathcal{A}_B)$ such that $\mathit{tr} = (w)_\AP$
	\end{itemize}
\end{lemma}

==> math/theorems/vpmodelcheckingreduction.tex <==
\begin{lemma}\label{lem:vpmodelcheckingreduction}
	The fair Visibly Pushdown Model Checking Problem for stuttering $H_\mu$ with unique successor assignments can be reduced in exponential time to the fair Visibly Pushdown Model Checking Problem for atomic restricted $H_\mu$ with unique successor assignments.
\end{lemma}

==> sections/introduction/preliminariesold.tex <==
\section{Preliminaries}\label{section:preliminaries}

\tbd{Different notation and letters for different systems and automata?}
\tbd{Idea: Define (infinite) Kripke Structure induced by a VPA, then define satisfaction only on Kripke Structures throughtout the paper}
\tbd{Idea: Define Kripke Structure as VPA with only internal moves, then define satisfaction only on VPA throughtout the paper}
\tbd{Shortest possible definition of all models: System Models are VPS, Kripke Structure is a VPS that only has internal moves;\\
Langauage acceptors are 2-AJA and VPA, APA are 2-AJA with only global successors}

\subsection{System Models}

Let $\AP$ be a finite set of atomic propositions.
A \textit{Kripke Structure} is a tuple $\mathcal{K} := (S, s^0, R, L)$ where $S$ is a finite set of states, $s^0 \in S$ is an initial state, $R \subseteq S \times S$ is a transition relation and $L : S \to 2^{\AP}$ is a labeling function.
We assume that Kripke Structures are total, i.e. there are no states without outgoing edges which means that for each $s \in S$, there is an $s' \in S$ with $(s,s') \in R$.
A \textit{relaxed path} of $\mathcal{K}$ is an infinite sequence $s_0 s_1 \dots \in S^{\omega}$.
A \textit{path} in a Kripke Structure $\mathcal{K}$ is a relaxed path where $s_0 = s^0$ is the initial state of $\mathcal{K}$ and $(s_{i}, s_{i+1})\in R$ holds for all $i \geq 0$.
We denote by $\RelPaths(\mathcal{K})$ the set of relaxed paths of $\mathcal{K}$ and by $\Paths(\mathcal{K})$ the set of paths in $\mathcal{K}$ starting in $s^0$. 
% and by $Paths^{*}(\mathcal{K},s)$ the set of corresponding path suffixes $\{p[i,\infty] | p \in Paths(\mathcal{K},s), i \in \mathbb{N}_0\}$ where $p[i,\infty]$ is the path suffix of $p$ starting at index $i$.
%As a slight variation, we use $Paths(\mathcal{K},p,i)$ to denote the set of paths in $\mathcal{K}$ that agree with path $p$ up to index $i$.
A \textit{trace} is an infinite sequence from the set $(2^{\AP})^{\omega}$.
For a path $s_0 s_1 \dots$, the induced trace is given by $L(s_0) L(s_1) \dots \in (2^\AP)^\omega$. 
%For a Kripke Structure $\mathcal{K}$ and a state $s \in S$, 
We write $\Traces(\mathcal{K})$ to denote the traces induced by paths of a Kripke Structure $\mathcal{K}$ starting in $s^0$.
A \textit{fair Kripke Structure} is a pair $(\mathcal{K},F)$ where $\mathcal{K} = (S,s^0,R,L)$ is a Kripke Structure and $F \subseteq S$ is a set of target states.
The set of paths $\Paths((\mathcal{K},F))$ is the set of fair paths of $\mathcal{K}$, i.e. the set of paths $p \in \Paths(\mathcal{K})$ that visit states in $F$ infinitely often.

\tbd{Use same notation for visibly pushdown systems and visibly pushdown automata? Does notion of configuration only apply to systems or automata? If yes, which one?}
\tbd{Add $\Gamma$ to VPS tuple?}
\tbd{Labelling function for configuration heads or just states?}

Let $\Gamma$ be a finite set of stack symbols and $\bot$ be a special bottom of stack symbol with $\bot \not\in \Gamma$.
A \textit{Visibly Pushdown System} is a tuple $\mathcal{VP} = (S,s^0,R,L)$ where $S$ is a finite set of control locations, $s^0$ is an initial control location and $L : S \to 2^{\AP}$ is a labeling function.
The transition relation $R \subseteq (S \times \{int\} \times S) \dot\cup (S \times \{call\} \times \Gamma \times S) \dot\cup (S \times \{ret\} \times \Gamma \times S)$ is a union of three kinds of transitions: internal moves from $(S \times \{int\} \times S)$, push moves from $(S \times \{call\} \times \Gamma \times S)$ and return moves from $(S \times \{ret\} \times \Gamma \times S)$.
A \textit{configuration} of a Visibly Pushdown System $\mathcal{VP} = (S,s^0,R,L)$ is a pair $c = (s,u)$ where $s \in S$ is a control location and $u \in \Gamma^* \bot$ is a stack content ending in $\bot$.
The set of all configurations of $\mathcal{VP}$ is denoted by $\conf(\mathcal{VP})$.
Let $c = (s,u)$ and $c' = (s',u')$ be configurations.
We call $c'$ an internal successor of $c$, denoted by $c \xrightarrow{int} c'$, if there is a transition $(s,int,s') \in R$ and $u = u'$.
We call $c'$ a call successor of $c$, denoted by $c \xrightarrow{call} c'$, if there is a transition $(s,call,\gamma,s') \in R$ and $u' = \gamma u$.
We call $c'$ a return successor of $c$, denoted by $c \xrightarrow{ret} c'$, if there is a transition $(s,ret,\gamma,s') \in R$ and $u = \gamma u'$.
A \textit{relaxed path} of $\mathcal{VP}$ is an infinite alternating sequence $p = (c_0,m_0) (c_1,m_1) \dots \in (\conf(\mathcal{VP}) \times \{int,call,ret\})^\omega$.
A \textit{path} of $\mathcal{VP}$ is a relaxed path such that $c_0 = (s^0,\bot)$ and for all $i \geq 0$ we have $c_i \xrightarrow{m_i} c_{i+1}$.
The visibly pushdown trace induced by $p$ is given by $(L(s_0),m_0) (L(s_1),m_1) \dots \in (2^\AP \times \{int,call,ret\})^\omega$.
We use $\RelPaths(\mathcal{VP})$ to denote the set of relaxed paths of $\mathcal{VP}$, $\Paths(\mathcal{VP})$ to denote the set of paths of $\mathcal{VP}$ and $\Traces(\mathcal{VP})$ to denote the set of traces induced by paths in $\Paths(\mathcal{VP})$.

For infinite sequences $w = w_0 w_1 \dots \in \Sigma^\omega$ for some alphabet $\Sigma$ like paths and traces, we introduce some additional notation.
We use $w(i) = w_i$ to denote the letter at position $i$ of $w$ and $w[i] = w_i w_{i+1} \dots$ to denote the suffix of $w$ starting at position $i$. 
For Visibly Pushdown Traces from $\VPTraces := (2^\AP \times \{int,call,ret\})^\omega$, we also introduce three successor functions as in \cite{Alur2004}.
\tbd{Adapt definitions to work on traces or switch back to definition on paths? Do we need definition on traces? If so, how to handle semantics?}
The function $\Succ_g \colon \VPTraces \times \mathbb{N}_0 \to \mathbb{N}_0$ with $\Succ_g(p,i) = i+1$ is called the global successor function.
The abstract successor function $\Succ_a \colon \VPTraces \times \mathbb{N}_0 \rightsquigarrow \mathbb{N}_0$ for a visibly pushdown path $p = c_0 m_0 c_1 m_1 \dots$ with $c_i = (s_i,u_i)$ is given by
\begin{align*}
	\Succ_a(p,i) = \begin{cases}
		\mathit{inf}\{j \mid j > i \land |u_i| = |u_j|\}, &\text{if } m_i \in \{int,call\},\\
		\mathit{undefined}, &\text{otherwise.}
	\end{cases}
\end{align*}
Finally, the caller function $\Succ_- \colon \VPTraces \times \mathbb{N}_0 \rightsquigarrow \mathbb{N}_0$ for a path $p = c_0 m_0 c_1 m_1 \dots$ with $c_i = (s_i,u_i)$ is given by
\begin{align*}
	\Succ_-(p,i) = \begin{cases}
		\mathit{sup}\{j \mid j < i \land |u_j| < |u_i|\}, &\text{if } \exists j<i:|u_j| < |u_i|,\\
		\mathit{undefined}, &\text{otherwise.}
	\end{cases}
\end{align*}

\subsection{Language Acceptors}

\tbd{Do we still need notion of holes?}

Let $\Sigma$ be a finite input alphabet.
An \textit{Alternating Parity Automaton} (APA) over $\Sigma$ is a tuple 
$\mathcal{A} = (Q, q_0, \rho, \Omega)$
such that $Q$ is a finite, non-empty set of control locations, $q_0 \in Q$ is an initial control location, $\rho: Q \times \Sigma \rightarrow \mathcal{B}^+(Q)$ is a function that maps control locations and input symbols	to positive boolean formulas over control locations and $\Omega: Q  \rightarrow \{0, 1, \dots k\}$ is a function that maps control locations to priorities.
We assume that every APA has two distinct states $\true$ with priority 0 and $\false$ with priority 1 such that $\rho(\true,\sigma) = \textit{true}$ and $\rho(\false,\sigma) = \textit{false}$ for all $\sigma \in \Sigma$.
If $\rho(q,\sigma)$ only consists of disjunctions for every $q$ and $\sigma$, we call an APA a Nondeterministic Parity Automaton (NPA) and denote $\rho(q,\sigma)$ as a set of control locations.
Additionally, we allow states $X$ with $\rho(X,\sigma) = \bot$ and $\Omega(X) = \bot$, which we call \textit{holes} \cite{Lange2005}.
Intuitively, a hole is a state where the construction of an APA is not yet finished.
By $\mathcal{A}[X:\mathcal{A}']$, we denote the APA $\mathcal{A}$ where the hole $X$ is replaced by the automaton $\mathcal{A}'$.

A \textit{tree} $T$ is a subset of $\mathbb{N}^{*}$ such that for every node $t \in \mathbb{N}^{*}$ and every positive integer $n \in \mathbb{N}$: $t \cdot n \in T$ implies (i) $t \in T$ (we then call $t \cdot n$ a child of $t$), and (ii) for every $0 < m < n$, $t \cdot m \in T$. 
We assume every node has at least one child.
A path in a tree $T$ is a sequence of nodes $t_0 t_1 \dots$ such that $t_0 = \varepsilon$ and $t_{i+1}$ is a child of $t_i$ for all $i \in \mathbb{N}_{0}$.
A \textit{run} of an APA $\mathcal{A}$ on an infinite word $w \in \Sigma^{\omega}$ is defined as a $Q$-labeled tree $(T,r)$ where $r: T \to Q$ is a labelling function such that $r(\varepsilon) = q_{0}$ and for every node $t \in T$ with children $t_1,\dots,t_k$, we have $1 \leq k \leq |Q|$ and the valuation assigning true to the control locations $r(t_1),\dots,r(t_k)$ and false to all other control locations satisfies $\rho(r(t),w(|t|))$.
A run $(T,r)$ is an \textit{accepting run} iff for every path $t_1 t_2 \dots$ in $T$, the lowest priority occuring infinitely often is even.
A word $w$ is \textit{accepted} by $\mathcal{A}$ iff there is an accepting run of $\mathcal{A}$ on $w$.
The set of infinite words accepted by $\mathcal{A}$ is denoted by $\mathcal{L}(\mathcal{A})$.
Extending the notion of holes, we write $\mathcal{A}[X:\mathcal{L}]$ for a language $\mathcal{L} \subseteq \Sigma^{\omega}$ to denote $\mathcal{A}[X:\mathcal{A}']$ for some automaton $\mathcal{A}'$ with $\mathcal{L}(\mathcal{A}') = \mathcal{L}$.
We call an APA (resp. NPA) an Alternating Büchi Automaton (resp. Nondeterministic Büchi Automaton) iff its priorities are $0$ and $1$.
We abbreviate these automata as ABA and NBA.
%We manipulate known theorems about alternation removal and complementation to work with APA with holes:
In the remainder of this paper, we use known theorems about parity and Büchi automata (without holes):

\input{math/theorems/paritydealternation}

%\autoref{thm:paritycomplement} and 
\autoref{thm:parityemptiness} can be found e.g.\ in \cite{Demri2016}.

\tbd{Define VPA from VPS or vice versa to reduce space needed for definitions?}
\tbd{Adapt Defintions of VPS and VPA such that stacks are treated the same way: should transitions be able to look at the top of stack or not?}
\tbd{Adapt VPA or VPS such that either both have a transition relation or a transition function; make function/relation total}
\tbd{single initial state or set?}

Let $\Sigma = \Sigma_i \dot\cup \Sigma_c \dot\cup \Sigma_r$ be a finite visibly pushdown alphabet and $\Gamma$ be a finite stack alphabet.
A (nondeterministic) \textit{Visibly Pushdown Automaton} (VPA) over $\Sigma$ and $\Gamma$ is a tuple $\mathcal{A} = (Q,Q_0,\rho,F)$ where $Q$ is a finite set of states, $Q_0 \subseteq Q$ is an initial state and $F \subseteq Q$ is a set of final states.
The transition relation $\rho \colon Q \times \Gamma \times \Sigma \to 2^{Q \times \Gamma^*}$ satisfies the following conditions for all $q \in Q$ and $\gamma \in \Gamma$: (i) for $\sigma_i \in \Sigma_i$, we have $\rho(q,\gamma,\sigma_i) \subseteq 2^{Q \times \Gamma}$, (ii) for $\sigma_c \in \Sigma_c$, we have $\rho(q,\gamma,\sigma_c) \subseteq 2^{Q \times \Gamma^2}$, and (iii) for $\sigma_r \in \Sigma_r$, we have $\rho(q,\gamma,\sigma_r) \subseteq 2^{Q \times \{\varepsilon\}}$.

\tbd{Letter for stack content?}
\tbd{only use $w$ without $w_0 w_1 \dots$ for words since we have notation $w(i)$?}

A \textit{run} of a VPA $\mathcal{A}$ over an infinite word $w = w_0 w_1 \dots \in \Sigma^\omega$ is an infinite sequence $(q_0,u_0)(q_1,u_1)\dots \in (Q \times \Gamma^*)^\omega$ such that $q_0 \in Q_0$, $u_0 = \bot$ for all $i \geq 0$ (i) if $w_i \in \Sigma_i$, then $u_i = \gamma u'$, $u_{i+1} = \gamma'u'$ and $(q_{i+1},\gamma') \in \rho(q_i,\gamma,w_i)$ for some $\gamma,\gamma' \in \Gamma$ and $u' \in \Gamma^*$, (ii) if $w_i \in \Sigma_c$, then $u_i = \gamma u'$, $u_{i+1} = \gamma'\gamma''u'$ and $(q_{i+1},\gamma'\gamma'') \in \rho(q_i,\gamma,w_i)$ for some $\gamma,\gamma',\gamma'' \in \Gamma$ and $u' \in \Gamma^*$, and (iii)  if $w_i \in \Sigma_r$, then $u_i = \gamma u'$, $u_{i+1} = u'$ and $(q_{i+1},\varepsilon) \in \rho(q_i,\gamma,w_i)$ for some $\gamma \in \Gamma$ and $u' \in \Gamma^*$.
A run $(q_0,u_0)(q_1,u_1)\dots \in (Q \times \Gamma^*)^\omega$ is accepting iff $q_i \in F$ for infinitely many $i$.
$\mathcal{A}$ accepts a word $w$ iff there is an accepting run of $\mathcal{A}$ over $w$.
We use $\mathcal{L}(\mathcal{A})$ to denote the set of words accepted by $\mathcal{A}$.

\input{math/theorems/vpacomplementation}

Let $\mathit{DIR} = \{g,a,b,c\}$.
A \textit{2-way Alternating Jump Automaton} (2-AJA) is a tuple $\mathcal{A} = (Q,q_0,\rho,\Omega)$ where $Q$, $q_0$ and $\Omega$ are defined the same way as in an APA and $\rho \colon Q \times \Sigma \to \mathcal{B}^+(\mathit{DIR} \times Q \times Q)$ is a transition funtion.
Instead of only moving to global successors ($g$) like in an APA, a 2-AJA can move to abstract successors ($a$), make backward steps ($b$) and moving to the caller ($c$).
A target $(dir,q,q')$ means that if the $dir$-successor exists in the current position $i$, the automaton starts a copy in state $q$ at this successor and else starts a copy in state $q$ at position $i+1$.

A \textit{run} of a 2-AJA over an infitie word $w = w_0 w_1 \dots \in \Sigma^\omega$ is a $\mathbb{N} \times Q$-labelled tree $(T,r)$ with labelling function $r \colon T \to \mathbb{N} \times Q$ that satisfies $r(\varepsilon) = (0,q)$ and for all $t \in T$ labelled $r(t) = (i,q)$ we have a set $\{(dir_0,q_0',q_0''),\dots,(dir_k,q_k',q_k'')\}$ satisfying $\rho(q,w_i)$ and children $t_1,\dots,t_k$ that are labelled in the following way: if $\Succ_{dir_h}(w,i)$ is undefined, then $r(t_h) = (i+1,q_h'')$, else $r(t_h) = (\Succ_{dir_h}(w,i),q_h')$.
Just like an APA, a run of an AJA is accepting iff for every path in the run, the lowest priority occuring infinitely often on that path is even.
$\mathcal{A}$ accepts a word $w$ iff there is an accepting run of $\mathcal{A}$ over $w$.
We use $\mathcal{L}(\mathcal{A})$ to denote the set of words accepted by $\mathcal{A}$.

\input{math/theorems/ajadealternation}

On multiple occasions in this paper, we use a function for nested exponentials.
Specifically, we define $g_{c,p}(0,n) := p(n)$ and $g_{c,p}(d+1,n) := c^{g_{c,p}(d,n)}$ for a constant $c > 1$ and a polynomial $p$.
For $c = 2$ and $p = id$, i.e. the identity function, we omit the subscripts in order to improve readability.
By slight abuse of notation, we say that a function $f$ is in $\mathcal{O}(g(d,n))$ if $f$ is in $\mathcal{O}(g_{c,p}(d,n))$ for some constant $c > 1$ and polynomial $p$.
We straightforwardly extend this notion to multiple $g$ functions, where different constants $c > 1$ and polynomials $p$ can be used for the various $g$ functions.
Also, we write $\SPACE(g(d,n))$ as an abbreviation for $\bigcup_{c,p}\SPACE(g_{c,p}(d,n))$ and $\TIME(g(d,n))$ as an abbreviation for $\bigcup_{c,p}\TIME(g_{c,p}(d,n))$.

==> sections/main/modelchecking.tex <==
\section{Model Checking Stuttering $H_\mu$}\label{sec:modelchecking}

\tbd{Structure of the section}

In this section, we consider variants of the Model Checking problem for stuttering $H_\mu$.
The structure is as follows: We first establish two undecidability results in \cref{subsec:undecidability} that motivate us to consider restrictions of the logic in further subsections.
Then, in \cref{subsec:basis}, we show that the fair Finite State and fair Visibly Pushdown Model Checking problems for stuttering $H_\mu$ with full basis can be reduced to the respective Model Checking problems for stuttering $H_\mu$ with basis $\AP$, enabling us to consider another restriction of the logic in the two subsections thereafter.
\cref{subsec:finitestate} and \cref{subsec:visiblypushdown} present algorithms that solve the respective fair Model Checking problems for stuttering $H_\mu$ with the previously established restrictions.
Finally, in \cref{subsec:lowerbounds}, we show that some of the presented algorithms are optimal by establishing lower bounds for the considered problems.

\subsection{Sources of Undecidability}\label{subsec:undecidability}

We start by considering the Finite State Model Checking problem.
It turns out, this problem is already undecidable for stuttering $H_\mu$:

\tbd{Reduce from the HyperLTL$_S$ Model Checking problem instead}

\input{math/theorems/undecidability}
%\input{math/shortproofs/undecidability}
\input{math/proofs/undecidability}

This proof heavily relies on the fact that two different successor assignments are allowed in a formula in gerneral.
It turns out, this is the reason for undecidability in this case.
Thus, we consider the restriction to stuttering $H_\mu$ with unique stuttering in the remainder of the section.

When it comes to Visibly Pushdown Model Checking however, this restriction is still not enough to obtain a decidable Model Checking problem:

\input{math/theorems/vpundecidability}
\input{math/proofs/vpundecidability}

The source of undecidability here is that even though we are considering traces from a visibly pushdown system, these traces are not aligned on $\intern$, $\call$ and $\ret$ moves, allowing to encode the intersection of contextfree languages.
This motivates us to consider another restriction when dealing with Visibly Pushdown Model Checking.
In particular, we will introduce a \textit{well-aligned} successor operator that poses some restrictions on how the stack operations on the traces to be considered in tandem may behave in \cref{subsec:visiblypushdown}.

\subsection{Restriction of the basis}\label{subsec:basis}

In this section, we show how the fair Model Checking problem for stuttering $H_\mu$ with full basis can be reduced to the fair Model Checking problem for stuttering $H_\mu$ with basis $\AP'$ for an amplified set of atomic propositions $\AP' \supseteq \AP$.
This is not only an interesting result in itself that works for the full logic.
It also has the nice property that it keeps the number of successor assignments the same, which is crucial for decidability.
The reduction thus motivates us to focus our efforts in developing a model checking procedure on stuttering $H_\mu$ with basis $\AP$ since such a procedure can be combined with the reduction to obtain a procedure for stuttering $H_\mu$ with full basis.
Generally, we use and expand on the ideas of \cite{Bozzelli2021} to perform a similar reduction for the logic HyperLTL$_S$ introduced in that paper.

Let $\varphi$ be a stuttering $H_\mu$ formula and $(\mathcal{VP},F)$ be a fair Visibly Pushdown System.
We show how to transform $\varphi$ into a formula $\varphi'$ with basis $\AP'$ and $(\mathcal{VP},F)$ into a fair Visibly Pushdown System $(\mathcal{VP}',F')$ such that $(\mathcal{VP},F) \models \varphi$ iff $(\mathcal{VP}',F') \models \varphi'$.
The main idea is to track the satisfaction of general single-trace formulae $\delta$ in $\varphi$ by atomic propositions $at(\delta)$ in the translation.
This is done by first constructing an automaton $\mathcal{A}_B$ that tracks for the set $B$ of formulae $\delta$ occuring in a test $[\delta]_\pi$ or a successor assignment $\Delta(\pi)$ of $\varphi$, that $at(\delta)$ is encountered if and only if $\delta$ indeed holds in this position of the input word of $\mathcal{A}_B$.
We then add this automaton to the fair Visibly Pushdown System $(\mathcal{VP},F)$ to arrive at the system $(\mathcal{VP}',F')$ that is properly labelled with $at(\delta)$ labels.
Then, we can replace tests $[\delta]_\pi$ or stuttering criteria $\Delta(\pi)$ in $\varphi$ with $[at(\delta)]_\pi$ or $at(\Delta(\pi))$ to obtain formula $\varphi'$ with basis $\AP'$ that we can check against $(\mathcal{VP}',F')$.

Let $B$ be the set of formulae occuring in a test $[\delta]_\pi$ or a successor assignment $\Delta(\pi)$ of $\varphi$.
Let $\cl(B)$ be the least set $C$ of formulae such that (i) $B \subseteq C$, (ii) $C$ is closed under semantic negation, that is if $\delta \in C$ then $\lnot\delta \in C$, where we mean the positive normal form of $\lnot \delta$ whenever we write $\lnot \delta$ in this construction, and (iii) if $\delta \in \sub(\delta')$ and $\delta' \in C$ then $\delta \in C$.
We will use atomic propositions $at(\delta)$ to track satisfaction of all formulae $\delta \in cl(B)$ on traces.
That is, we expand the set of atomic propositions $\AP$ by $\AP_\delta := \{at(\delta) \mid \delta \in \cl(B)\}$ to obtain $\AP_{B} := \AP \dot\cup \AP_\delta$ and expand traces from $2^{\AP} \times \{\intern,\call,\ret\}$ to $2^{\AP_{B}} \times \{\intern,\call,\ret\}$.

In this construction and the associated lemmas, we need a notion of fixpoint alternation depth for $\delta$ formulae.
In a formula $\delta$, we say that the variable $Y'$ depends on the variable $Y$, written $Y \prec_\delta Y'$ if $Y$ is a free variable in $\fp(Y')$.
We use $<_\delta$ to denote the transitive closure of $\prec_\delta$.
Then the alternation depth $\ad(\delta)$ is the length of a maximal chain $Y_1 <_\delta \dots <_\delta Y_n$ such that adjacent variables have a different fixpoint type.
We extend this notion to sets of $\delta$ formulae: $\ad(B) = \max\{\ad(\delta) \mid \delta \in B\}$.
For a formula $\varphi$, we define $\ad(\varphi) = \ad(B)$ for the set $B$ defined above.

%\input{math/constructions/modelcheckinglemma}

\tbd{This construction has to altered so always two symbols are read. Also the lemma should be slightly altered since we are not interested in all words over $2^\AP \cup \{\intern,\call,\ret\}$ but only those from $(2^\AP \cdot \{\intern,\call,\ret\})^\omega$.}

Given a set of $VP-\mu TL$ formulae $B$, we construct the 2-AJA $\mathcal{A}_{B}$ that ensures that for all $\delta \in B$, $at(\delta)$ holds in a position on a trace if and only if $\delta$ holds on this position on the trace's restriction by conjunctively moving to a module checking $\delta$ for every atomic proposition $at(\delta)$ encountered.
These modules are constructed in a standard manner.
We introduce a state $q_\delta$ for every $\delta \in \cl(B)$.
Their transition function can either check $\delta$ directly if it is an atomic formula, or move to states for the subformulae of $\delta$ using suitable transitions if it is not.
Fixpoints introduce loops with even or odd priorities depending on the type of the fixpoint.
The details of this construction is given in \cref{app:modelcheckinglemma}.

In our construction, $\mathcal{A}_B$ only makes non global moves if subformulae $\bigcirc^a \delta$ or $\bigcirc^c \delta$ occur in $B$.
Also notice that when considering the fair Finite State Model Checking problem, we can restrict the basis to the linear time $\mu$-calculus where $\bigcirc^a \delta$ or $\bigcirc^c \delta$ do not occur due to \cref{rem:fsbasisformulae}.
Thus, we can assume $\mathcal{A}_B$ to be an APA over $2^{\AP_{B}} \times \{\intern\}$ in this situation.
For combining $\mathcal{A}_B$ with a Visibly Pushdown System or Kripke Structure, we transform it into a nondeterministic automaton.
Given $w \in (2^{\AP_{B}} \times \{\intern,\call,\ret\})^\omega$ let $(w)_\AP$ be the restriction of $w$ to $(2^\AP \times \{\intern,\call,\ret\})^\omega$.
Applying \cref{thm:ajadealternation}  or \cref{thm:paritydealternation} to $\mathcal{A}_B$ gives us the following Lemma:

%Applying \cref{thm:ajadealternation} to the 2-AJA $\mathcal{A}_B$ gives us:

%\input{math/theorems/vpmodelcheckinglemma}
%\input{math/proofs/vpmodelcheckinglemma}

\input{math/theorems/modelcheckinglemma}
\input{math/proofs/modelcheckinglemma}

Now we can use this automaton to enrich the fair Visibly Pushdown System to be checked.
$(\mathcal{VP}',F')$ is constructed as a product structure of $(\mathcal{VP},F)$ and $\mathcal{A}_B$ that extends the labeling from one assigning $\AP$ labels to one assigning $\AP_{B}$ labels in a consistent manner.
Intuitively, $\Traces(\mathcal{VP}',F')$ is the set of traces $\tr$ over $\AP_{B}$ such that $(\tr)_\AP$ is a trace from $\Traces(\mathcal{VP},F)$ and propositions $at(\delta)$ occur in those positions where $\delta$ holds on $(\tr)_\AP$, i.e. for all $i \geq 0$ and $\delta \in \cl(B)$, $at(\delta) \in \tr(i)$ iff $i \in \llbracket \delta \rrbracket^{(\tr)_\AP}$.
The details of this construction are described in \cref{app:productstructure}.

%\input{math/constructions/productstructure}

\input{math/constructions/formulatranslation}

Overall, we obtain the following result:

\input{math/theorems/modelcheckingtranslation}

On a conceptual level, we have:

\input{math/theorems/modelcheckingreduction}
%\input{math/proofs/modelcheckingreduction}

\subsection{Fair Finite State Model Checking}\label{subsec:finitestate}

\tbd{Explain better what ideas we take from \cite{Bozzelli2021} and why we still have this section}

Let $(\mathcal{K},F)$ with $\mathcal{K} = (S,S_0,R,L)$ be a fair Kripke Structure and $\varphi := Q_1 \pi_1 \dots Q_n \pi_n. \psi$ be a closed formula with basis $\AP$ where $\psi$ uses a unique successor assignment $\Delta$.
In this subsection we show how to decide $(\mathcal{K},F) \models \varphi$.
Like in the previous subsection, we expand on ideas from \cite{Bozzelli2021} that were used to establish decidability for a fragment of HyperLTL$_S$.
Let $\psi^s$ be the variant of $\psi$ where $\Delta$ is replaced with the synchronous successor assignment $\Delta_{\true} = \lambda \pi . \true$.
Note that since we only have atomic tests, $\psi^s$ is a formula belonging to the synchronous fragment of $H_\mu$ from \cite{GutsfeldMO21}.
We establish a connection between $\psi$ and $\psi^s$ that will allow us to reuse an automaton construction for synchronous $H_\mu$ from \cite{GutsfeldMO21} for model checking $\varphi$.
We have:

\input{math/theorems/synchronousconnection}
%\input{math/proofs/synchronousconnection}

In order to formalise the connection between formulae and the automata we construct from them, we need a notion of equivalence that respects trace assignments over a set of traces $\mathcal{T}$.
Such a relation is called $\mathcal{K}$-equivalence in the literature \cite{Finkbeiner2015} where instead of trace assignments, path assignments over paths of a Kripke Structure $\mathcal{K}$ are considered as the basis for semantics.
Here we adapt this notion to our setting where the semantics is based on trace assignments.
\tbd{Also change $w_\Pi$ to match changes in traces?}
Given a trace assignment $\Pi$ over $\mathcal{T}$ with $\Pi(\pi_i) = P_0^i m_0^i P_1^i m_1^i \dots \in \Traces = (2^{\AP} \cdot \{\intern,\call,\ret\})^\omega$, we define $w_\Pi \in ((2^{\AP} \times \{\intern,\call,\ret\})^n)^\omega$ such that $w_\Pi (i) = ((P_i^1,m_i^1),\dots,(P_i^n,m_i^n))$.
We define:

\tbd{Maybe change this to $(\Delta,\mathcal{T})$-equivalence to match the section after this:
$v \in \llbracket \psi \rrbracket^\Pi$ iff $w_{\Pi^\Delta}[v] \in \mathcal{L}(\mathcal{A})$.
Then we have that  $\mathcal{A}_\psi$ is $(\Delta,\mathcal{T})$-equivalent to $\psi$, not only to $\psi^s$.
Also, $\mathcal{A}_\varphi$ is $(\Delta,\mathcal{T})$-equivalent to $\varphi$ for all subformulae, not only the full formula.}

\input{math/defs/kequivalence}

For quantified formulae $\varphi$ with $n$ free variables, this notion is extended such that $\mathcal{A}$ is $\mathcal{T}$-equivalent to $\varphi$ iff for all trace assignments $\Pi$ of size $n$ over $\mathcal{T}$, we have that $\Pi \models_{\mathcal{T}} \varphi$ and $w_{\Pi} \in \mathcal{L}(\mathcal{A})$ are equivalent.
In the special case where all trace variables are quantified in $\varphi$, this condition reduces to $\mathcal{T} \models \varphi$ iff $w \in \mathcal{L}(\mathcal{A})$ for the unique word $w$ over the single letter alphabet of empty tuples.
Thus, model checking a fair Kripke Structure $(\mathcal{K},F)$ against a formula $\varphi$ can be reduced to an emptiness test on an automaton $\mathcal{A}$ that is $\Traces(\mathcal{K},F)$-equivalent to $\varphi$.

A combination of Theorem 5.2 and 6.1 from \cite{GutsfeldMO21} gives us the following theorem:

\input{math/theorems/synchronousautomaton}

Note that in \cite{GutsfeldMO21}, $\mathcal{K}$-equivalence is defined with respect to free predicates in formulae and holes in automata.
Since we are only concerned with closed formulae, we can use a simpler definition here.
Another difference is that their definition uses Kripke Structures $\mathcal{K}$ rather than trace sets $\mathcal{T}$.
However, the results of \cref{thm:synchronousautomaton} still carry over: a slight variation of the constructions there also works for the input alphabet $(2^{\AP} \times \{\intern,\call,\ret\})^n$ instead of $S^n$ and for quantified formulae, $\mathcal{K}$-equivalence and $\mathcal{T}$-equivalence have the same requirements.

%\input{math/constructions/restrictedfinitestatemodelchecking}

Using \cref{lem:synchronousconnection} and this automaton, we construct another automaton $\mathcal{A}_{\varphi}$ that is $\Traces(\mathcal{K},F)$-equivalent to $\varphi$ by adding a technique to handle the quantifiers.
When adressing the quantifier $Q_i \pi_i. \varphi'$, we know that $\Delta(\pi_i) = \ap$ for some $\ap \in \AP$ since $\varphi$ has basis $\AP$.
The main idea is to transform $(\mathcal{K},F)$ into a fair Kripke Structure $(\mathcal{K}_\ap,F_\ap)$ such that $\Traces(\mathcal{K}_\ap,F_\ap) = \strf_\ap(\Traces(\mathcal{K},F))$.
Then, we can use a standard construction for handling quantifiers as used e.g. for HyperLTL in \cite{Finkbeiner2015}, HyperPDL-$\Delta$ in \cite{Gutsfeld2020a} or $H_\mu$ in \cite{GutsfeldMO21} with the difference that we use $(\mathcal{K}_\ap,F_\ap)$ instead of $(\mathcal{K},F)$ in the product construction.
A detailed construction of $\mathcal{A}_\varphi$ as well as the proof of the following theorem can be found in \cref{app:finitestate}.
%For this automaton, it holds:

\input{math/theorems/quantifierkequivalence}
%\input{math/proofs/quantifierkequivalence}

Overall we obtain the following result:

\input{math/theorems/restrictedfinitestatemodelchecking}
\input{math/proofs/restrictedfinitestatemodelchecking}

In combination with the results of the previous section, we obtain:

\input{math/theorems/finstatemodelchecking}
\input{math/proofs/finstatemodelchecking}

\subsection{Fair Visibly Pushdown Model Checking}\label{subsec:visiblypushdown}

\tbd{Explain this section better}

In this subsection, we tackle the fair Model Checking problem for Visibly Pushdown Systems.
As seen in \cref{thm:vpundecidability}, this problem is even harder than the fair Finite State Model Checking problem as a restriction to unique stuttering does not suffice to obtain decidability.
Thus, we introduce another restriction by defining what we call a \textit{well-aligned} successor operator.
Recall that for a trace $\tr = P_1 m_1 P_2 m_2 \dots \in \Traces$, we use the  $\calls_{i,j}^{\tr} = |\{k \mid i \leq k \leq j \text{ and } m_k = \call \}|$ to denote the number of calls between positions $i$ and $j$ and use $\rets_{i,j}^{\tr} = |\{k \mid i \leq k \leq j \text{ and } m_k = \ret \}|$ to denote the number of returns between positions $i$ and $j$.
\tbd{Change notation here? Maybe we dont even need this anmore due to new well-alignedness definition.}
We call subtraces $\tr_1[v_1,v_1'],...,\tr_n[v_n,v_n'] \in (2^{\AP} \times \{\intern,\call,\ret\})^*$ well-aligned iff there are integers $e,l \in \mathbb{Z}$ such that for all $1 \leq i \leq n$, we have (i) $e = \calls_{v_i,v_i'}^{\tr_i} - \rets_{v_i,v_i'}^{\tr_i}$ and (ii) $l = \min \{ \calls_{v_i,j}^{\tr_i} - \rets_{v_i,j}^{\tr_i} \mid v_i \leq j \leq v_i' \}$.
\tbd{First say this informally, then formally}
Intuitively, (i) means that the subtraces add or remove the same number of stack levels and (ii) means that if they remove stack levels, then they remove the same amount.
For subtraces starting on the same stack level, this means that they end on the same stack level and the lowest stack level they encounter is the same.

\tbd{New definition of well-alignedness:\\
Let $\tr$ be a finite trace and $\tr_{|\mathit{cr}}$ its restriction to the transition symbols, i.e. if $\tr = P_0 m_0 P_1 m_1 \dots m_{n-1} P_n$ then $\tr_{|\mathit{cr}} = m_0 m_1 \dots m_{n-1}$.
Also let $\tr_\abs$ be the version of $\tr$ where every $\intern$ symbol is replaced with $\abs$.
We call words $\mathit{absstrf}$ over $\{\abs,\call,\ret \}$ \textit{abstract stratifications}.
We say that $\mathit{absstrf}$ is an abstract stratification of a trace $\tr$ iff there is a maximal sequence $\tr_0,\tr_1,\dots,\tr_l$ with $\tr_\abs = \tr_0$ and $\mathit{absstrf} = \tr_{l|cr}$ such that for all $i<l$, $\tr_{i+1}$ is obtained from $\tr_i$ in the following way:
if $\tr_i = P_0,m_0,\dots,P_{n}$, let $j_1 < n$ be the minimal index such that there is $j_2 > j_1$ such that $m_{j_1} = \call$ and $\Succ_a(\tr_i,j_1) = j_2$.
Then $\tr_{i+1} = P_0 m_0 \dots m_{j_1-1} P_{j_1} \abs P_{j_2} m_{j_2} \dots P_{n}$.

It is easy to see that (i) every trace has an abstract stratification and (ii) the  abstract stratification of a trace is unique.
We thus use $\mathit{absstrf}(\tr)$ to denote the unique abstract stratification of $\tr$.
From the definition of abstract successors, it is also easy to see that $\mathit{absstrf}(\tr)$ is contained in the regular language $(\abs^*\ret)^r (\abs^*\call)^c \abs^*$ for some $r,c \in \mathbb{N}_0$.
We then call $(r,c)$ the $\ret-\call$ profile of $\tr$.
Now we define well-alignedness:
\begin{definition}
	We call traces $\tr_1,\dots,\tr_n$ \textit{well-aligned} iff they have the same $\ret-\call$ profile.
\end{definition}
}

We now define a well-aligned variant of the successor operator $\Succ_\Delta(\Pi,v)$ for trace assignments $\Pi$ and vectors $v = (v_1,...,v_n)$.
Let $\tr_i = \Pi(\pi_i)$ and $v_i' := \Succ_{\Delta(\pi_i)}(\tr_i,v_i)$ for all $i$.
We define
\begin{align*}
	\Succ_\Delta^w(\Pi,v) := \begin{cases}
		\Succ_\Delta(\Pi,v) &\text{if } \tr_1[v_1,v_1'],...,\tr_n[v_n,v_n'] \text{ are well-aligned}\\ 
		\mathit{undefined} &\text{else}
	\end{cases} 
\end{align*}
From now on, we use this successor operator in the semantics of $\bigcirc^\Delta \psi$:
\begin{align*}
	\llbracket \bigcirc^\Delta \psi \rrbracket_{\mathcal{W}}^\Pi := \{ v \in \mathbb{N}_0^n \mid \Succ_\Delta^w(\Pi,v) \text{ is defined and }\Succ_\Delta^w(\Pi,v) \in \llbracket \psi \rrbracket_{\mathcal{W}}^{\Pi} \}.
\end{align*}
Notice that this operator is not dual to itself.
We do, however, need a dual version of the next operator in order to ensure a positive form of $\psi$ formulae.
For this purpose, we define
\begin{align*}
	\llbracket \bigcirc_d^\Delta \psi \rrbracket_{\mathcal{W}}^\Pi := \{ v \in \mathbb{N}_0^n \mid \Succ_\Delta^w(\Pi,v) \text{ is undefined or }\Succ_\Delta^w(\Pi,v) \in \llbracket \psi \rrbracket_{\mathcal{W}}^{\Pi} \}.
\end{align*}
On traces generated from Kripke Structures, both well-aligned next operators coincide with the previous definition.

%While the restriction to well-aligned successors might seem like a drastic restriction at first sight, we believe that it is natural in many circumstances. 
We believe that the restriction to well-aligned successors is natural in many circumstances. Often hyperproperties are used to specify that different executions of a system satisfying certain conditions are sufficiently similar. In such situations, a deviation from well-alignedness often already indicates that the executions differ from each other too much. Examples from the realm of security include non-interference and observational determinism, where non-aligned visits to program points observed by an attacker in itself hint at a security risk. Note also that the formula $\psi_{wa} = \nu X. \true \land \bigcirc^\Delta X$ expresses explicitly that the traces under considerations are indeed well-aligned with respect to $\Delta$. 
This formula can then be used either to require certain properties captured by a subformula $\psi_{\textit{prop}}$ for well-aligned evolutions only by using $\psi_{wa}$ as a pre-condition like in $\psi_{wa} \rightarrow \psi_{\textit{prop}}$ or to require well-alignedness in addition to the property as in $\psi_{wa} \land \psi_{\textit{prop}}$. 
Notice that the addition of the formula $\psi_{wa}$ as precondition or conjunct of sub-formulae preserves unique stuttering such that the resulting formulae still belong to the fragment for which model checking for VPS is decidable.
\begin{comment}
Note that due to the fact that we require well-alignedness in the semantics of the next operator instead of in the semantics of trace quantifiers, we have flexibility on how much well-alignedness we have to require from the system.
For this, notice that the formula $\psi_{wa} = \nu X. \true \land \bigcirc^\Delta X$ expresses that the traces under considerations are well-aligned with respect to $\Delta$.
Then, the formula $\forall \pi_1 . \forall \pi_2 . \psi_{wa} \rightarrow \psi$ expresses that all well-aligned pairs of traces satisfy $\psi$ whereas the formula $\forall \pi_1 . \forall \pi_2 . \psi_{wa} \land \psi$ expresses that all pairs of traces are well-aligned and satisfy $\psi$.

We argue that the notion of well-alignedness is adequate for many scenarios.
Especially in information security applications prominent in the hyperlogics literature, observation points on the executions that are compared have to be similar in order for the comparison to make sense.
Hyperproperties like observational determinism or non-interference state that a low security user cannot deduce values of high security variables from low security outputs.
However, such a deduction can only be made if a difference in low security outputs is only due to a difference in the high security variables and not due to the fact that one of the two executions under comparison is in a completely different part of the program.
Additionally, such a system behavior would have its own security consequences.
\end{comment}
\begin{comment}
We argue that the well-aligned next operator induces a natural requirement for many scenarios.
Especially in information security applications prominent in the hyperlogics literature, observation points on the executions that are compared have to be similar in order for the comparison to make sense.
Hyperproperties like observational determinism or non-interference state that a low security user cannot deduce values of high security variables from low security outputs.
However, such a deduction can only be made if a difference in low security outputs is only due to a difference in the high security variables and not due to the fact that one of the two executions under comparison is in a completely different part of the program.
Additionally, such a system behavior would have its own security consequences.
\end{comment}
\tbd{If we keep the old definition and this lemma, then we have to adapt the notation for traces.}
\tbd{
Let $\tr$ be a finite trace and $\tr_{|\mathit{cr}}$ its restriction to the second component, i.e. if $\tr = (P_0,m_0)(P_1,m_1)\dots(P_n,m_n)$ then $\tr_{|\mathit{cr}} = m_0 m_1 \dots m_n$.
Also let $\tr_\abs$ be the version of $\tr$ where every $\intern$ symbol is replaced with $\abs$.
We call words $\mathit{absstrf}$ over $\{\abs,\call,\ret \}$ \textit{abstract stratifications}.
We say that a trace $\tr$ is \textit{compatible} with an abstract stratification $\mathit{absstrf}$ iff there is a sequence $\tr_0,\tr_1,\dots,\tr_l$ with $\tr_\abs = \tr_0$ and $\mathit{absstrf} = \tr_{l|cr}$ such that for all $i<l$, $\tr_{i+1}$ is obtained from $\tr_i$ in the following way:
if $\tr_i = (P_0,m_0),\dots,(P_{n},m_{n})$ and there are indices $j_1<j_2 \leq n$ such that $m_{j_1} = \call$ and $\Succ_a(\tr_i,j_1) = j_2$, then $\tr_{i+1} = (P_0,m_0),\dots,(P_{j_1-1},m_{j_1-1}),(P_{j_1},\abs),(P_{j_2},m_{j_2}),\dots,(P_{n},m_{n})$.

Comment: 
This way, if one step moves from position $i_1$ to $i_2$ and the next step moves from $i_2$ to $i_3$, then $m_{i_2}$ is included in the subtrace $\tr[i_1,i_2]$ and in the subtrace $\tr[i_2,i_3]$.
This can be a problem when $m_{i_2}$ is either a $\call$ or a $\ret$ symbol that is then not replaced in one subtrace and treated as part of an abstract step in the other.
Maybe grouping traces as $P_0 \cdot m_0 \cdot P_1 \cdot m_1 \dots$ instead of $(P_0,m_0)\cdot(P_1,m_1)\dots$ may help. Then we can define finite traces from start to end state, i.e. $P_0 \cdot m_0\cdot P_1 \cdot m_1\dots P_{n-1} \cdot m_{n-1}\cdot P_n$.

Lemma:\\
Let $\tr_1,\dots,\tr_n$ be well-aligned finite traces.
Then there are natural numbers $r,c \in \mathbb{N}_0$ such that for all $1\leq i\leq n$ there is an abstract stratification $\mathit{absstrf}_i$ from the regular language $(\abs^*\ret)^r (\abs^*\call)^c \abs^*$ compatible with $\tr_i$.
}

The next lemma helps us to see why well-alignedness helps us obtain a decidable Model Checking problem:

\input{math/theorems/alignmentlemma}
%\input{math/proofs/alignmentlemma}

Intuitively, this lemma tells us that despite the fact that well-aligned subtraces may have different $\call$ and $\ret$ behavior, they still can be progressed in tandem using a single stack.
For this, successions of $\abs$ moves can be turned into internal steps and the different traces can synchronise their stack actions on the $k$ common $\ret$ and $l$ common $\call$ moves.

In the remainder of this section, we sometimes need the number of steps for which the well-aligned next operator is defined on a trace assignment $\Pi$.
For this, we call $l := \sup\{i \in \mathbb{N}_0 \mid (\Succ_{\Delta}^w)^i(\Pi,(0,\dots,0)) \text{ is defined}\}$ the length of the $\Delta$-well-aligned prefix of $\Pi$.

%Let $\llbracket \psi \rrbracket^\Pi_0 := \llbracket \psi \rrbracket^\Pi \cap \{(0,...,0)\}$ and 
Let $\psi^j$ for $j \in \mathbb{N}_0$ be recursively defined as follows:
$\psi^0$ replaces all $\bigcirc^\Delta \psi'$ subformulae in $\psi$ with $\false$ as well as $\bigcirc_d^\Delta \psi'$ subformulae with $\true$ and $\psi^{j+1}$ is obtained from $\psi$ by replacing every subformula $\psi'$ of $\psi$ which is directly in scope of an outermost $\bigcirc^\Delta$ or $\bigcirc_d^\Delta$ operator by $\psi'^{j}$.
For this, fixpoints are unrolled $j$ times for $\psi^j$.
We will need the following lemma which is easily established by induction:

\input{math/theorems/alignedprefixlemma}
%\input{math/shortproofs/alignedprefixlemma}
%\input{math/proofs/alignedprefixlemma}

We now proceed with the Model Checking procedure.
For this purpose, let $(\mathcal{VP},F)$ be a fair visibly pushdown system with $\mathcal{VP} = (S,S_{0},R,L)$ over the stack alphabet $\Gamma$ and $\varphi := Q_1 \pi_1 \dots Q_n \pi_n . \psi$ be a formula with basis $\AP$ that uses a single successor assignment $\Delta$ and well-aligned next operators.
Similar to the previous section, we build an automaton $\mathcal{A}_\varphi$ that is equivalent to $\varphi$ with respect to a certain equivalence relation in order to reduce the fair Model Checking problem to an emptiness test of an automaton.
Here, we need a slightly different notion of equivalence compared to \cref{def:kequivalence}.

Let $\Pi$ be a trace assignment over $\mathcal{T}$ with $\Pi(\pi_i) = P_0^i m_0^i P_1^i m_1^i \dots \in \Traces = (2^{\AP} \cdot \{\intern,\call,\ret\})^\omega$ and $l \in \mathbb{N} \cup \{\infty\}$ be the length of the $\Delta$-well-aligned prefix of $\Pi$.
For $i \leq l$, let $r_i$ and $c_i$ be the number of returns and calls in well-aligned step $i$ according to \cref{lem:alignmentlemma} respectively.
We define $w_\Pi^{wa}$ as $\mathcal{P}_0 \cdot \{\ret\}^{r_0} \cdot \{\call\}^{c_0} \cdot \mathcal{P}_1 \cdot \{\ret\}^{r_1} \cdot \{\call\}^{c_1} \cdot ... \in ((2^\AP)^n \cdot \{ret\}^* \cdot \{\call\}^*)^\omega$ if $l = \infty$ and as $\mathcal{P}_0 \cdot \{\ret\}^{r_0} \cdot \{\call\}^{c_0} \cdot ... \cdot \mathcal{P}_l \cdot \{\top\}^\omega \in ((2^\AP)^n \cdot \{\ret\}^* \cdot \{\call\}^*)^* \cdot \{\top\}^\omega$ if $l \in \mathbb{N}$ where $\mathcal{P}_i = (P_i^1,\dots,P_i^n)$.
Since single traces $\tr$ are always well-aligned with themselves, this definition already induces a natural encoding $w_{\tr}^{wa} = w_{\Pi}^{wa}$ where $|\Pi| = 1$ and $\Pi(\pi) = \tr$.
For the empty trace assignment $\{\}$, $c_i$ and $r_i$ are not given by \cref{lem:alignmentlemma} since there are no traces in $\{\}$.
Here, we have a special case and say that $w_{\{\}}^{wa}$ is a well-aligned encoding of $\{\}$ if it is of the form $(() \cdot \{\ret\}^* \cdot \{\call\}^*)^\omega$ where $()$ is the empty tuple.
In order to simplify notation in the next definition, we define offsets in $w_{\Pi}^{wa}$ in a slightly different manner than usual.
For $i \leq l$, we have $w_{\Pi}^{wa}[i] = \mathcal{P}_i \cdot \{\ret\}^{r_i} \cdot \{\call\}^{c_i} \cdot ...$ and for $i > l$, we have $w_{\Pi}^{wa}[i] = \{\top\}^\omega$.
Based on this encoding, we adapt our notion of equivalence between formulae and automata:

\input{math/defs/alignedkequivalence}

We again extend this notion to quantified formulae $\varphi$ with $n$ free variables.
An automaton $\mathcal{A}$ is $\Delta$-aligned $\mathcal{T}$-equivalent to $\varphi$ iff for all trace assignments $\Pi$ of size $n$ over $\mathcal{T}$, we have that $\Pi \models_{\mathcal{T}} \varphi$ and $w_{\Pi}^{wa} \in \mathcal{L}(\mathcal{A})$ are equivalent.
In the special case where all trace variables are quantified in $\varphi$, this condition reduces to $\mathcal{T} \models \varphi$ iff $w \in \mathcal{L}(\mathcal{A})$ for some word $w \in (() \cdot \{\ret\}^* \cdot \{\call\}^*)^\omega$ due to our special definition of $w_{\{\}}^{wa}$.
Thus, model checking a fair Visibly Pushdown System $(\mathcal{VP},F)$ against a formula $\varphi$ can be reduced to an emptiness test on an automaton $\mathcal{A}$ that is $\Delta$-aligned $\Traces(\mathcal{VP},F)$-equivalent to $\varphi$.

\input{math/constructions/alignedformulaautomaton}

With this construction, we obtain:

\input{math/theorems/alignedsynchronousautomaton}
\input{math/shortproofs/alignedsynchronousautomaton}
%\input{math/proofs/alignedsynchronousautomaton}

\input{math/constructions/restrictedvpmodelchecking}

\input{math/theorems/quantifieralignedkequivalence}
\input{math/shortproofs/quantifieralignedkequivalence}
%\input{math/proofs/quantifieralignedkequivalence}

Overall, we obtain the following result:

\input{math/theorems/restrictedvpmodelchecking}
\input{math/proofs/restrictedvpmodelchecking}

Together with the results from \cref{subsec:basis}, we have:

\input{math/theorems/vpmodelchecking}
\input{math/proofs/vpmodelchecking}

\subsection{Lower bounds}\label{subsec:lowerbounds}

In order to finish our section about the Model Checking Problem for stuttering $H_\mu$, we establish lower bounds for the complexity.
We start with the finite state case.
Here, they can easily be obtained from the lower bounds for HyperLTL.

\input{math/theorems/finitestatelowerbound}
\input{math/proofs/finitestatelowerbound}

For the visibly pushdown case, we obtain a precise bound for the alternation-free case by a reduction from the LTL Model Checking problem against Visibly Pushdown Systems.

\input{math/theorems/vplowerbound}
\input{math/proofs/vplowerbound}

Using results from the previous subsections, we obtain:
%Together with the complexity results from the previous two subsections, we obtain:

\input{math/theorems/modelcheckingcompleteness}
\input{math/proofs/modelcheckingcompleteness}

==> sections/main/tbd.tex <==
\section{Stuff for which the exact place is not determined yet}


\subsection{Sources of Undecidability}\label{subsec:undecidability}

We start by considering the Finite State Model Checking problem.
It turns out, this problem is already undecidable for stuttering $H_\mu$:

\tbd{Reduce from the HyperLTL$_S$ Model Checking problem instead}

\input{math/theorems/undecidability}
%\input{math/shortproofs/undecidability}
\input{math/proofs/undecidability}

This proof heavily relies on the fact that two different successor assignments are allowed in a formula in gerneral.
It turns out, this is the reason for undecidability in this case.
Thus, we consider the restriction to stuttering $H_\mu$ with unique stuttering in the remainder of the section.

When it comes to Visibly Pushdown Model Checking however, this restriction is still not enough to obtain a decidable Model Checking problem:

\input{math/theorems/vpundecidability}
\input{math/proofs/vpundecidability}

The source of undecidability here is that even though we are considering traces from a visibly pushdown system, these traces are not aligned on $\intern$, $\call$ and $\ret$ moves, allowing to encode the intersection of contextfree languages.
This motivates us to consider another restriction when dealing with Visibly Pushdown Model Checking.
In particular, we will introduce a \textit{well-aligned} successor operator that poses some restrictions on how the stack operations on the traces to be considered in tandem may behave in \cref{subsec:visiblypushdown}.


\subsection{Lower bounds}\label{subsec:lowerbounds}

In order to finish our section about the Model Checking Problem for stuttering $H_\mu$, we establish lower bounds for the complexity.
We start with the finite state case.
Here, they can easily be obtained from the lower bounds for HyperLTL.

\input{math/theorems/finitestatelowerbound}
\input{math/proofs/finitestatelowerbound}

For the visibly pushdown case, we obtain a precise bound for the alternation-free case by a reduction from the LTL Model Checking problem against Visibly Pushdown Systems.

\input{math/theorems/vplowerbound}
\input{math/proofs/vplowerbound}

Using results from the previous subsections, we obtain:
%Together with the complexity results from the previous two subsections, we obtain:

\input{math/theorems/modelcheckingcompleteness}
\input{math/proofs/modelcheckingcompleteness}
